Mathematical Reasoning in Large Language Models: Benchmarks, Architectures, Evaluation, and Open Challenges

Mathematical reasoning is essential for problem-solving in education, science, and industry, serving as a crucial benchmark for evaluating artificial intelligence systems. As Large Language Models (LLMs) improve their reasoning capabilities, understanding how well they perform mathematical reasoning has become increasingly important. This survey synthesizes recent advancements in mathematical reasoning with LLMs through a structured analysis of datasets, architectures, training strategies, and evaluation protocols. Our systematic review encompasses approximately 120 peer-reviewed studies and preprints, examining the evolution of this research area and providing a unified analytical framework to understand current progress and limitations. Our study particularly introduces a unified taxonomy of mathematical datasets, distinguishing between pretraining corpora, supervised fine-tuning resources, and evaluation benchmarks across varying levels of reasoning complexity. A systematic analysis of reasoning architectures and training strategies, including tool integration, verifier-guided reasoning, and parameter-efficient adaptation, is presented to assess their effects on reasoning robustness and generalization. Moreover, a comparative evaluation of existing metrics highlights the gap between final-answer accuracy and process-level reasoning verification. By synthesizing insights across these areas, our analysis identifies recurring failure modes, such as reasoning faithfulness issues, benchmark biases, and generalization limitations, and outlines key research directions toward improving symbolic grounding, evaluation reliability, and the development of more robust and trustworthy LLM-based reasoning systems.

==> challanges_discussion.tex <==
%------------------------------------------------------------------
% \begin{figure}[t]
% \centering
% \scriptsize
% \resizebox{\textwidth}{!}{
% \fbox{
% \parbox{0.95\textwidth}{

% \textbf{Challenges in LLM-based mathematical reasoning.}
% \vspace{4pt}
% \textbf{Datasets (Sec.~\ref{sec4})}
% $\rightarrow$ Synthetic CoT bias, dataset contamination, limited out-of-distribution coverage
% \vspace{3pt}
% \textbf{Representation}
% $\rightarrow$ Tokenization limitations, weak numerical encoding, symbol ambiguity
% \vspace{3pt}
% \textbf{Model Architectures (Sec.~\ref{sec5})}
% $\rightarrow$ Pattern imitation vs.\ true reasoning, limited symbolic manipulation
% \vspace{3pt}
% \textbf{Training Strategies (Sec.~\ref{sec5})}
% $\rightarrow$ Unfaithful chain-of-thought reasoning, parametric knowledge bias, memorization
% \vspace{3pt}
% \textbf{Evaluation (Sec.~\ref{sec7})}
% $\rightarrow$ Accuracy-only metrics, lack of reasoning verification, weak fault localization
% \vspace{3pt}
% \textbf{Outcome}
% $\rightarrow$ Strong linguistic fluency but unreliable mathematical reasoning
% }
% }
% }

% \caption{Challenge pipeline summarizing the interconnected limitations affecting mathematical reasoning in LLMs.}
% \label{fig:challenge_pipeline}
% \end{figure}

==> comments.tex <==
\begin{comment}
% ==========================Table 11=====================================
\begin{table}[t]
\centering
\caption{Representative variants of LoRA for parameter-efficient fine-tuning.}
\label{tab:lora}
\scriptsize
\resizebox{\textwidth}{!}{
\begin{tabularx}{\textwidth}{
>{\raggedright\arraybackslash}X
>{\raggedright\arraybackslash}X
>{\raggedright\arraybackslash}X}

\toprule
\textbf{Method} & \textbf{Key Idea} & \textbf{Strength} \\
\midrule
LoRA \citep{hu2021lora}
& Injects trainable low-rank matrices into frozen Transformer layers
& Enables efficient fine-tuning with minimal parameters \\
\midrule
Quantized LoRA (QLoRA) \citep{Dettmers2023QLORA}
& Combines LoRA with low-bit quantization
& Allows fine-tuning of large models on limited hardware \\
\midrule
Adaptive Rank LoRA (AdaLoRA) \citep{zhang2023adalora}
& Dynamically allocates rank based on parameter importance
& Improves parameter efficiency under limited budgets \\
\midrule
Decomposition-based LoRA (DoRA) \citep{liu2024dora}
& Separates weight updates into magnitude and direction components
& Enhances stability and reasoning performance \\
\midrule
Sparse/ Dynamic LoRA (SoRA \citep{ding2023sora}, DyLoRA \citep{valipour2023dylora})
& Applies sparsity or dynamic rank allocation
& Reduces training cost while preserving accuracy \\
\midrule
Mixture-of-Adapters (MoPE \citep{jiang2025mope}, LoRAMoE \citep{Dou2024loramoe})
& Combines multiple LoRA adapters with expert routing
& Improves multi-task adaptation \\
\bottomrule
\end{tabularx}
}
\end{table}
\end{comment}


\section{Architectures and Training Strategies}\label{sec5}
%===============================================Working: Mehwish
This section covers architecture variants adapted for mathematical reasoning, training and reasoning enhancement strategies. 

%Recent LLMs rely primarily on Transformer-based architectures trained on massive text corpora containing billions to trillions of tokens. Decoder-only models dominate current LLM designs because they support efficient autoregressive generation and scale effectively across distributed computing infrastructure. %These architectures integrate multi-head self-attention, feed-forward networks, and layer normalization to capture long-range dependencies and contextual relationships in text.
\subsection{Architectures}
Recent LLMs rely primarily on Transformer-based architectures trained on massive text corpora containing billions to trillions of tokens. Decoder-only models dominate current LLM designs because they support efficient autoregressive generation and scale effectively across distributed computing infrastructure. 

TODO: Husnain: 
    Add pretrained archiectures
                Pretrain architectures serve as the core of LLMs are based on transformer architecture possessing self attention mechanism to capture the relationship between the words independent of their presence in sentence. It advances language models to learn and understand contextual information effectively for language tasks. Depending on the organization of transformer architecture, language models are classified into three categories encoder only, decoder only, and encoder-decoder architecture. Encoder only architecture is primarily designed for language understanding tasks with classic example of BERT employing bidirectional self attention and train using masked language modeling. Meanwhile, contrasting to encoder only architecture, decoder only architecture is primarily designed for scalable text generation capabilities such as GPT, LLaMA, Qwen, DeepSeek and other contemporary models employing causal self attention and auto-regressive next word prediction. Where encoder only and decoder only architectures doing their part in their own way by understanding and generational capabilities, the encoder-decoder architecture such as T5 is designed for both language contextual understanding and text generational capabilities. These architecture contribute to language generation and understanding tasks effectively however they remain contrained on mathematical reasoning task due to symbolic handling and mathematical computational restraints. To address these initial solution comes with idea of integration of helping tools termed as tool augmentation.


    Tool-Augmented Architectures
                Tool augmented architectures extends pretrained language models by incorporating external computational resources such as calculators, computer algebra systems, theorem provers, symbolic solvers, and executable programming environments. It relies the chances of error by not relying solely on the parametric knowledge by decomposing problems into sub-tasks and assigning them to designated tool integrated. In the meantime it is crucial that model correctly decompose the problem and assign it to its respective tool and maintain robust orchestration between neural and symbolic components. This extension to architecture although substantially enhances computational accuracy, however it does not guarantee that the reasoning process itself is correct, motivating the need for explicit mechanisms that can assess and validate generated solutions. 

    
    Verifier Architectures
                To improve reasoning reliability verifier architectures on the other introduce the verification module that evaluates the reasoning trajectories, intermediate steps or final solution generated by language model. to implement the verifier in architecture there are methods such as process reward model, critic network or rule based system that add guided search and filter out incorrect solutions. By separating solution generation from solution validation, verifier-based systems improve reasoning reliability and reduce superficial pattern matching. However, their performance remains constrained by verifier accuracy and susceptibility to false acceptance or rejection of reasoning paths.

    
    Agentic Architectures
                Consequently, recent research has moved beyond isolated generation and verification stages toward more autonomous reasoning frameworks capable of planning, tool use, self-reflection, and iterative problem solving representing the latest evolution of mathematical reasoning systems.
                Agentic architectures treat problem solving as a dynamic and iterative decision-making process rather than a single-pass generation task. These architectures combine planning, tool invocation, verification, memory, and self-correction mechanisms to explore multiple reasoning paths before producing a final solution. Through planner–executor frameworks, search-based exploration, reflection loops, and adaptive reasoning strategies, agentic systems can tackle complex mathematical problems that require long-horizon reasoning and multi-step decision making. By integrating the capabilities of pretrained models, external tools, and verification mechanisms into a unified framework, agentic architectures provide a more comprehensive approach to mathematical reasoning, at the cost of increased computational complexity and coordination overhead. However, agentic architectures do not fully eliminate the fundamental challenges of mathematical reasoning. While planning, tool use, and self-reflection can improve performance, these mechanisms may also amplify reasoning errors when generated plans, retrieved information, or verification outcomes are incorrect. Moreover, the interaction between multiple components introduces additional sources of uncertainty and reduces system interpretability, making it difficult to determine whether successful outcomes arise from genuine reasoning, effective search, or heuristic exploration. As a result, ensuring reasoning faithfulness, evaluation reliability, and reproducibility remains an open research challenge for agentic mathematical reasoning systems.


    

%For reasoning tasks, a model can undergo multiple training strategies including pretraining, finetuning and post-training alignment. This is because mathematical reasoning performance also depends on how reasoning is represented, verified, and executed during training and inference. Recent studies have explored a range of architectural adaptations and training strategies designed to improve mathematical problem solving, including reasoning-oriented prompting mechanisms, tool integration, verifier-guided generation, process supervision, reinforcement learning, and parameter-efficient specialization. These approaches differ substantially in both their underlying assumptions and the aspects of reasoning they attempt to improve. The following subsections review these strategies and examine how they have been adapted to enhance mathematical reasoning. We categorize them into two streams: How models are trained and How reasoning is enhanced.

%\subsection{Reasoning Oriented Extensions of LLM Architectures}
\subsection{Model Training}
%While standard transformer architectures provide the foundation for most modern LLMs, mathematical reasoning performance often depends on additional reasoning-oriented mechanisms rather than architecture alone. Several extensions have therefore emerged to improve structured reasoning. One line of work augments language models with explicit reasoning traces, such as chain-of-thought prompting and stepwise scratchpad generation, allowing intermediate computations to be externalized during inference. Another direction integrates external tools such as symbolic solvers, calculators, or programming environments, enabling models to offload precise computation to deterministic systems. A third approach introduces verifier or critic models that evaluate candidate reasoning paths and guide the model toward more reliable solutions. These approaches suggest that improvements in mathematical reasoning often arise from hybrid reasoning pipelines that combine neural generation with symbolic verification, structured search, or external computation rather than from architectural scaling alone.
 %However, training at scale does not determine reasoning performance. 
%Recent LLMs scale efficiently through distributed training strategies such as data parallelism, tensor parallelism, and pipeline parallelism, enabling efficient use of GPU/TPU clusters for training \citep{smith2022using}.
Mathematical reasoning is shaped by the training strategies used during model development. Recent approaches typically combine large-scale pretraining, task-specific fine-tuning, reinforcement learning, and efficient adaptation techniques to improve reasoning performance while balancing computational cost and generalization. They often consider distributed training strategies such as data parallelism, tensor parallelism, and pipeline parallelism, enabling efficient use of GPU/TPU clusters for training \citep{smith2022using}.
 
%\subsubsection{Pretraining}
%pretraining forms the computational foundation of LLM development. During this stage, models learn general linguistic and semantic representations by training on extremely large corpora that often contain trillions of tokens. Training typically requires distributed infrastructure consisting of hundreds or thousands of GPUs or TPUs. Efficient training relies on optimization strategies such as data parallelism, tensor parallelism, pipeline parallelism, and memory-efficient techniques including Zero Redundancy Optimization (ZeRO).Successful pretraining requires careful balancing of model capacity, training data quality, and computational resources. Research on scaling laws shows that model performance improves predictably as model parameters, dataset size, and training compute increase \citep{kaplan2020scaling, hernandez2021scaling, zhang2023cumulative, wei2023skywork}. These scaling relationships guide the design of modern LLM training pipelines and explain the rapid capability improvements observed in recent models \citep{hoffmann2022training}.
\textit{Pretraining.}

It provides broad linguistic and semantic knowledge by exposing models to large-scale corpora. For mathematical reasoning, domain-specific corpora such as OpenWebMath and Proof-Pile increase exposure to mathematical notation, formulas, and proofs. However, gains from mathematical pretraining must be interpreted carefully because large-scale web corpora may introduce contamination and memorization risks \citep{paster2023openwebmath, azerbayev2023proofnet, huang2025math, shi2023detecting}.

\textit{Supervised Fine-Tuning.}

It adapts pretrained models using customized datasets such as mathematical question-answer pairs, worked examples, and reasoning traces for task specific fine-tuninh \citep{li2023label, wu2025llm, toshniwal2024openmath}.
%\subsubsection{Supervised Fine-Tuning}
%Supervised fine-tuning adapts a pre-trained model to specific tasks using labeled input–output pairs \citep{ziegler2019fine}. Task-specific datasets, such as question–answer pairs or reasoning examples, guide the model toward producing structured and task-relevant responses \citep{wu2025llm}. Compared with pretraining corpora, these datasets are significantly smaller but provide high-quality supervision for specialized capabilities.

\textit{Instruction Tuning.}

It improves the ability of language models to follow natural language instructions through curated instruction-response pairs. Mathematical instruction datasets frequently incorporate worked solutions and reasoning traces, enabling stronger generalization to multi-step problem solving \citep{min2021metaicl, parnami2022learning, chen2022large, tang2024mathscale}.

\textit{Reinforcement Learning.}

It controls reasoning behavior through reward signals. Outcome Reward Models (ORMs) \citep{thatikonda-etal-2025-logical} evaluate final answers, whereas Process Reward Models (PRMs) \citep{zhang-etal-2025-lessons} assess intermediate reasoning steps. Recent approaches further extend this paradigm through reward reasoning models and reasoning-oriented policy optimization algorithms such as Proximal Policy Optimization (PPO) and Trust Region Policy Optimization (TRPO) \citep{schulman2015trust, achiam2017constrained, zhang2024scalable}.

%\subsubsection{Reinforcement Learning}
%Reinforcement learning further aligns model behavior with desired outputs by optimizing responses according to reward signals. A typical reinforcement learning framework includes a reward model that evaluates response quality and a policy optimization stage that updates the language model accordingly.

%Reward models can be rule-based or model-based \citep{liu2025deepseek}. Rule-based reward systems verify outputs through deterministic constraints such as numerical correctness or structured formatting, providing high reliability for tasks like mathematical reasoning \citep{mu2024rule}. Model-based reward models estimate response quality based on learned preference signals \citep{ouyang2022training}, though they are more prone to reward hacking, necessitating specific mitigation strategies \citep{miao2024inform, fu2025reward}. Policy optimization algorithms such as Proximal Policy Optimization (PPO) and Trust Region Policy Optimization (TRPO) enable stable reinforcement learning for LLMs \citep{schulman2015trust, achiam2017constrained, zhang2024scalable}.

%In mathematical reasoning, model-based evaluation targets different levels of reasoning. Outcome Reward Models (ORMs) check the final answer's logical validity, guiding search and test-time scaling \citep{thatikonda-etal-2025-logical}. Process Reward Models (PRMs) evaluate each intermediate step to ensure correctness and prevent flawed reasoning \citep{zhang-etal-2025-lessons}. Recent Reward Reasoning Models (RRMs) go further by generating reasoning steps to judge complex proofs more accurately \citep{guo2025reward}.

%For policy optimization, foundational algorithms such as Proximal Policy Optimization (PPO) and Trust Region Policy Optimization (TRPO) provide stable reinforcement learning \citep{schulman2015trust, achiam2017constrained}. Tailored algorithms like Group Relative Policy Optimization (GRPO) efficiently optimize reasoning without memory-intensive critic models \citep{shao2024deepseekmath, zhang2024scalable}.

\textit{Parameter-Efficient Fine-Tuning (PEFT).}

These methods such as LoRA, QLoRA, AdaLoRA, and DoRA reduce the computational cost of adapting large language models to mathematical tasks by updating only a small subset of model parameters while keeping most pretrained weights frozen \citep{hu2021lora, Dettmers2023QLORA, zhang2023adalora, liu2024dora}. While these methods facilitate experimentation and domain specialization, their contribution to mathematical reasoning remains largely indirect. Most reported gains arise from improved adaptation to mathematical supervision data rather than modifications to the underlying reasoning process. Consequently, PEFT methods should be viewed primarily as efficiency-oriented adaptation strategies rather than reasoning-enhancement mechanisms, highlighting the need to distinguish adaptation efficiency from genuine reasoning improvements \citep{liang2025low}. %Table~\ref{tab:lora} summarizes representative LoRA-based techniques.

%\subsubsection{Parameter-Efficient Fine-Tuning}

%Adapting extremely large models through full fine-tuning is computationally expensive. Parameter-efficient fine-tuning (PEFT) methods address this limitation by updating only a small subset of model parameters while freezing the majority of pretrained weights. Among these methods, Low-Rank Adaptation (LoRA) and its variants have become widely adopted because they significantly reduce memory and compute requirements while preserving model performance.

%LoRA introduces trainable low-rank matrices into Transformer layers while keeping the original weights fixed. Several variants extend this approach through quantization, adaptive rank allocation, sparsity mechanisms, or expert routing. Table~\ref{tab:lora} summarizes representative LoRA-based techniques.

\subsection{Reasoning Enhancement}

\textit{Post-Training and Alignment.} 

Although pretraining provides broad language competence, additional training stages are required to adapt models for downstream tasks and align them with human instructions. Post-training typically includes supervised fine-tuning, instruction tuning, and reinforcement learning based on feedback.

\textit{Chain-of-Thought (CoT) Reasoning.} 

CoT prompting externalizes intermediate reasoning steps before generating a final answer. This approach consistently improves performance on arithmetic and multi-step reasoning tasks by encouraging decomposition of complex problems into simpler sub-problems \citep{wei2022chain, wang2023selfconsistency, yuan2023well, parnami2022learning, chen2022large}.

\textit{Tool-Integrated Reasoning.} 

It augments language models with external systems such as calculators, theorem provers, symbolic engines, and code execution environments. These approaches improve numerical precision and symbolic manipulation by delegating deterministic computations to specialized tools \citep{li2024tool, imani2023mathprompter, lu2021intergps}.

\textit{Verifier-Guided Reasoning.} 

These approaches employ auxiliary models or verification modules to evaluate candidate reasoning trajectories and filter incorrect solutions. These methods improve answer reliability but introduce additional dependence on verifier quality and calibration \citep{cobbe2021training, zhang2025formalizing, guo2025reward}.

\textit{Process Supervision.} 

It evaluates intermediate reasoning steps rather than final answers alone. By providing feedback at the reasoning-process level, these approaches aim to improve reasoning fidelity and error localization, although scalable verification remains challenging \citep{zhang2025formalizing, didolkar2024metacognitive, ren2025multi}.
%\subsubsection{Instruction Tuning}
%Instruction tuning improves the ability of language models to follow natural language instructions. In this approach, models are trained on diverse instruction–response pairs that represent human task descriptions \citep{min2021metaicl}. This training enables models to generalize to new tasks through zero-shot and few-shot prompting \citep{xian2017zero, wang2020generalizing}, which is critical for handling novel mathematical word problems with diverse linguistic formulations \citep{pourpanah2022review}. 

%Many instruction-tuning datasets incorporate CoT reasoning traces, where intermediate steps explicitly describe the reasoning process. These structured responses significantly improve performance on multi-step reasoning tasks \citep{parnami2022learning, chen2022large}.


%\subsubsection{Chain of Thought}
%Although the preceding discussion outlines the general LLM training pipeline, mathematical reasoning places additional demands on both model adaptation and training design. In practice, researchers have introduced a range of math-specific modifications spanning corpus design, reasoning supervision, external tool integration, and verification-oriented training. Table~\ref{tab:math_arch_training} summarizes these adaptations and clarifies the distinct role each plays in improving mathematical reasoning performance.
%These adaptations show that progress in mathematical reasoning rarely depends on architecture alone. Instead, performance emerges from the interaction between mathematical data, supervision format, symbolic support, and verification mechanisms. At the same time, many of these strategies introduce their own bottlenecks, including contamination risk, synthetic bias, verifier dependence, and limited transfer to structurally novel problems. These tensions are discussed in the following subsection.

\begin{table}[t]
\centering
\caption{Math-specific architectural and training adaptations for improving reasoning in LLMs.}
\label{tab:math_arch_training}
\scriptsize
\resizebox{\textwidth}{!}{
\begin{tabularx}{\textwidth}{
>{\raggedright\arraybackslash}X
>{\raggedright\arraybackslash}X
>{\raggedright\arraybackslash}X
>{\raggedright\arraybackslash}X}
\toprule
\textbf{Adaptation Type} & \textbf{Representative Idea} & \textbf{Expected Benefit} & \textbf{Key Challenge} \\
\midrule
Math-focused pretraining corpora & Pretraining on OpenWebMath, Proof-Pile, formula-rich corpora & Better exposure to mathematical syntax, notation, and discourse & Risk of contamination and weak provenance \\ \midrule
Instruction tuning on math traces & Fine-tuning on worked examples and solution chains & Improves elicitation of stepwise reasoning & Can inherit shortcuts from synthetic traces \\ \midrule
Rule-based reward modeling & Rewards correctness, formatting, or executable validity & Stronger alignment for objective tasks like math & Reward definition may be narrow or brittle \\ \midrule
Tool-augmented generation & Calculator, CAS, theorem prover, Python execution & Better precision on symbolic and numerical subproblems & Requires reliable decomposition and tool integration \\ \midrule
Parameter-efficient adaptation & LoRA, QLoRA, AdaLoRA, DoRA & Efficient specialization of large models for math tasks & May improve adaptation efficiency more than core reasoning \\ \midrule
Verifier or critic modules & Secondary model scores candidate reasoning paths & Helps filter incorrect but fluent outputs & Verifier itself may be unfaithful or undertrained \\ \midrule
Structure-aware representations & Symbolic encoders, MathML, formula-aware embeddings & Better handling of equations and operator structure & Hard to integrate cleanly into general-purpose LLM pipelines \\
\bottomrule
\end{tabularx}
}
\end{table}

%============================ Table End ================================
\subsection{Training Trends and Challenges}
Despite significant progress, several challenges remain in training LLMs for complex reasoning tasks. One major limitation arises from the mismatch between training objectives and reasoning behavior. Language models optimize next token prediction rather than logical correctness, which can produce fluent yet incorrect reasoning chains \citep{lindsey2025biology}.

Another challenge involves parametric knowledge bias. During pretraining, models store large amounts of knowledge in their parameters. While this internal knowledge improves downstream performance, it can also lead to hallucinations when the model relies on memorized patterns rather than input context \citep{ji2023survey, longpre2021entity}.

Large-scale training also raises concerns about memorization and data leakage. Models may reproduce segments of training data, which introduces risks related to copyright violations, privacy exposure, and sensitive data leakage \citep{feldman2020does, shi2023detecting, carlini2022privacy, huang2025math}. Addressing these issues requires improved training objectives, better dataset curation practices, and evaluation methods that emphasize reasoning faithfulness and data safety.


Despite substantial progress, several challenges continue to limit reliable mathematical reasoning in LLMs. A fundamental issue arises from the mismatch between training objectives and reasoning requirements. Language models are optimized for next-token prediction rather than logically valid derivations, allowing fluent explanations and correct-looking reasoning traces to emerge without guaranteeing mathematical correctness \citep{lindsey2025biology}.

Another challenge concerns the distinction between memorization and reasoning. Large-scale pretraining exposes models to vast amounts of mathematical content, enabling strong benchmark performance but also increasing the likelihood of contamination and pattern recall. Consequently, high accuracy may not necessarily reflect genuine reasoning ability, particularly on widely used benchmarks that overlap with pretraining corpora \citep{huang2025math, shi2023detecting}.

Reasoning reliability remains an additional concern. Models frequently generate plausible but incorrect intermediate steps, hallucinate mathematical facts, or propagate early errors through long reasoning chains. These failures are compounded when models rely on memorized patterns rather than problem-specific reasoning, making it difficult to distinguish faithful reasoning from post-hoc rationalization \citep{ji2023survey, longpre2021entity}.

Finally, scaling training data and model size introduces challenges related to memorization, privacy, and data leakage. Models may reproduce portions of training data, raising concerns about benchmark validity, copyright exposure, and sensitive information leakage \citep{feldman2020does, carlini2022privacy, shi2023detecting}. Addressing these limitations requires not only improved training objectives and dataset curation practices but also evaluation frameworks that prioritize reasoning faithfulness, verification, and generalization beyond benchmark performance.



%---------------------------------------------------------------------------------------------------------------------
\section{Evaluation of Mathematical Reasoning}\label{sec6}
%===============================================working: Mehwish: 16/6
Evaluating the performance of LLMs on mathematical reasoning tasks remains challenging. Unlike human evaluation, model outputs often consist of fluent natural language explanations that appear coherent while containing logical or computational errors \citep{ahn2024large}. Mathematical reasoning tasks involve structured symbolic manipulation and multi-step derivations, making them fundamentally different from standard text generation tasks. Consequently, evaluating only the final answer is often insufficient. Reliable evaluation must assess both the correctness of the final solution and the validity of intermediate reasoning steps to avoid false positives and false negatives \citep{wang2025examining}.

Researchers therefore employ several metrics to measure model performance on mathematical reasoning tasks. Traditional metrics such as accuracy and exact match compare the generated answer with the reference solution. Additional measures including F1-score, Macro F1-score, True Positive Rate (TPR), and True Negative Rate (TNR) are also used to measure alignment between generated outputs and ground truth \citep{bostrom2020byte, huang2025math}. However, these metrics primarily evaluate outcome correctness and provide limited insight into the reasoning process that produced the answer.

Mathematical reasoning can be assessed at multiple levels, from final-answer correctness to stepwise derivational validity, no single metric provides a complete picture of model performance. Table~\ref{tab:eval_metrics_math} compares the most common evaluation approaches and highlights the trade-off between simplicity, diagnostic value, and verification rigor.

\begin{table}[t]
\centering
\caption{Evaluation metrics and verification approaches for mathematical reasoning in LLMs.}
\label{tab:eval_metrics_math}
\scriptsize
\resizebox{\textwidth}{!}{
\begin{tabularx}{\textwidth}{
>{\raggedright\arraybackslash}X
>{\raggedright\arraybackslash}X
>{\raggedright\arraybackslash}X
>{\raggedright\arraybackslash}X}
\toprule
\textbf{Metric / Approach} & \textbf{What It Measures} & \textbf{Strength} & \textbf{Main Limitation} \\
\midrule
Accuracy & Correctness of final predicted answer & Simple and widely comparable & Ignores intermediate reasoning validity \\ \midrule
Exact Match & Exact textual agreement with gold answer & Strict and reproducible & Overly sensitive to formatting or equivalent expressions \\ \midrule
F1 / Macro F1 / TPR / TNR & Output-level overlap or class-based performance & Useful in structured or classification-style tasks & Limited interpretability for open-form mathematical reasoning \\ \midrule
Relative Error / Numeric deviation & Distance from gold numeric answer & Useful for approximate numerical tasks & Sensitive to outliers and not reasoning-aware \\ \midrule
Skill success metrics & Whether specific subskills are executed correctly & More diagnostic than final-answer accuracy & Requires task decomposition into skills \\ \midrule
Process supervision metrics & Correctness of intermediate reasoning steps & Better reflects reasoning quality & Expensive and difficult to scale reliably \\ \midrule
Symbolic verification & Validation through theorem provers, solvers, or executable traces & High rigor for formal reasoning tasks & Limited to settings with formalizable outputs \\ \midrule
Hybrid verification & Combines neural generation with symbolic checking & More reliable than answer-only evaluation & Complex pipeline and incomplete coverage of free-form reasoning \\
\bottomrule
\end{tabularx}
}
\end{table}

The comparison makes clear that widely used metrics such as accuracy and exact match remain attractive because they are simple and reproducible, yet they fail to capture whether a model reasoned correctly. More diagnostic approaches exist, but they are harder to scale and often require structured outputs, executable traces, or formal verification environments. This limitation explains why answer-level evaluation remains dominant despite its conceptual weakness.

Accuracy based evaluation is particularly problematic for mathematical reasoning. A model may produce the correct answer through memorization or shortcut pattern recognition rather than genuine reasoning, while correct reasoning chains may be penalized due to minor numerical deviations such as rounding errors. As a result, accuracy metrics fail to distinguish robust reasoning ability from superficial pattern matching.

To address this limitation, recent work evaluates reasoning processes directly. Metrics such as skill success rate, secondary skill success rate, completion rate, and calculation success rate measure the model’s ability to execute specific reasoning skills required to solve mathematical problems \citep{yuan2023well, didolkar2024metacognitive}. For formal mathematical reasoning tasks, syntactic and semantic correctness can also be verified using automated theorem proving tools such as the Isabelle proof assistant \citep{azerbayev2023proofnet}.

Recent research further explores process-level evaluation approaches. Automated process supervision techniques analyze intermediate reasoning steps rather than only final outputs. Methods based on Monte Carlo Tree Search enable efficient error localization, while hybrid verification approaches combine symbolic solvers with executable reasoning traces to improve reliability \citep{ren2025multi}. However, the diversity and complexity of reasoning patterns produced by LLMs make automated verification difficult \citep{herbert2019challenges, herbert2021overcoming}. Consequently, verifying intermediate reasoning steps remains computationally expensive and often requires human oversight.

\subsection{Critical Synthesis: The Reliability Gap}
Although process-level evaluation is often presented as a solution to the limitations of answer-level metrics, the relationship is more complex. Answer-based metrics fail to distinguish genuine reasoning from memorization or shortcut learning, but process-level approaches introduce a second layer of uncertainty because the correctness of reasoning traces must itself be verified. Consequently, evaluation challenges are not eliminated but shifted from answer validation to process validation.

A central tension therefore emerges between scalability and reliability. Answer-level metrics are easy to compute and reproduce but provide limited insight into reasoning quality. In contrast, process-level evaluation, symbolic verification, and hybrid verification offer richer diagnostic information but require structured outputs, specialized tools, or additional verifier models. This trade-off explains why answer-level metrics continue to dominate benchmark reporting despite their conceptual limitations.

These observations suggest that mathematical reasoning evaluation should be viewed as a spectrum rather than a single measurement problem. Different evaluation strategies capture different aspects of reasoning performance, and no existing metric provides a complete assessment of reasoning correctness, faithfulness, robustness, and generalization.

\subsection{Evaluation Failure Modes and Limitations}\label{evalsec1}
Despite the availability of multiple evaluation metrics, several limitations remain. Accuracy remains the most widely used metric for mathematical reasoning benchmarks \citep{huang2025math, singh2024tokenization, guan2025rstar, rhomrasi2025llm}. However, accuracy evaluates only the final answer and does not capture the correctness of intermediate reasoning steps. Models may therefore achieve high scores through memorization or heuristic shortcuts rather than principled reasoning.

Evaluation consistency also presents challenges. LLMs may generate different reasoning paths or error localization patterns for the same problem across multiple runs, complicating reproducible evaluation \citep{ren2025multi}. Furthermore, discrepancies frequently arise between explicit reasoning traces generated by the model and the internal mechanisms that produce the final answer. Although interpretability methods such as attribution graphs provide partial insights into model behavior, they do not fully reveal the reasoning processes used by the model \citep{lindsey2025biology}.

Intermediate evaluation metrics such as relative error (RE) introduce additional limitations because they can be dominated by outliers or disproportionately large deviations \citep{yuan2023well}. These challenges highlight the need for more robust evaluation frameworks that jointly assess answer correctness, reasoning validity, and model reliability in mathematical problem solving.

Overall, current evaluation protocols still measure mathematical reasoning primarily through final-answer correctness. While convenient, this approach provides limited insight into the reasoning processes that produce correct answers. A model may arrive at the correct solution through memorization, heuristic shortcuts, or reasoning paths that are logically inconsistent. Future evaluation frameworks must therefore move beyond answer-level metrics and incorporate scalable process-level verification to better assess genuine reasoning capability.




\begin{table}[t]
\centering
\caption{Evaluation metrics and verification approaches for mathematical reasoning in LLMs.}
\label{tab:eval_metrics_math}
\scriptsize
\resizebox{\textwidth}{!}{
\begin{tabularx}{\textwidth}{
>{\raggedright\arraybackslash}X
>{\raggedright\arraybackslash}X
>{\raggedright\arraybackslash}X
>{\raggedright\arraybackslash}X}
\toprule
\textbf{Metric / Approach} & \textbf{What It Measures} & \textbf{Strength} & \textbf{Main Limitation} \\
\midrule
Accuracy & Correctness of final predicted answer & Simple and widely comparable & Ignores intermediate reasoning validity \\ \midrule
Exact Match & Exact textual agreement with gold answer & Strict and reproducible & Overly sensitive to formatting or equivalent expressions \\ \midrule
F1 / Macro F1 / TPR / TNR & Output-level overlap or class-based performance & Useful in structured or classification-style tasks & Limited interpretability for open-form mathematical reasoning \\ \midrule
Relative Error / Numeric deviation & Distance from gold numeric answer & Useful for approximate numerical tasks & Sensitive to outliers and not reasoning-aware \\ \midrule
Skill success metrics & Whether specific subskills are executed correctly & More diagnostic than final-answer accuracy & Requires task decomposition into skills \\ \midrule
Process supervision metrics & Correctness of intermediate reasoning steps & Better reflects reasoning quality & Expensive and difficult to scale reliably \\ \midrule
Symbolic verification & Validation through theorem provers, solvers, or executable traces & High rigor for formal reasoning tasks & Limited to settings with formalizable outputs \\ \midrule
Hybrid verification & Combines neural generation with symbolic checking & More reliable than answer-only evaluation & Complex pipeline and incomplete coverage of free-form reasoning \\
\bottomrule
\end{tabularx}
}
\end{table}


Accuracy remains the most widely used metric for mathematical reasoning benchmarks \citep{huang2025math, singh2024tokenization, guan2025rstar, rhomrasi2025llm}. However, accuracy evaluates only the final answer and does not capture the correctness of intermediate reasoning steps. Models may therefore achieve high scores through memorization or heuristic shortcuts rather than principled reasoning.

Evaluation consistency also presents challenges. LLMs may generate different reasoning paths or error localization patterns for the same problem across multiple runs, complicating reproducible evaluation \citep{ren2025multi}. Furthermore, discrepancies frequently arise between explicit reasoning traces generated by the model and the internal mechanisms that produce the final answer. Although interpretability methods such as attribution graphs provide partial insights into model behavior, they do not fully reveal the reasoning processes used by the model \citep{lindsey2025biology}.

Intermediate evaluation metrics such as relative error (RE) introduce additional limitations because they can be dominated by outliers or disproportionately large deviations \citep{yuan2023well}. These challenges highlight the need for more robust evaluation frameworks that jointly assess answer correctness, reasoning validity, and model reliability in mathematical problem solving.

Overall, current evaluation protocols still measure mathematical reasoning primarily through final-answer correctness. While convenient, this approach provides limited insight into the reasoning processes that produce correct answers. A model may arrive at the correct solution through memorization, heuristic shortcuts, or reasoning paths that are logically inconsistent. Future evaluation frameworks must therefore move beyond answer-level metrics and incorporate scalable process-level verification to better assess genuine reasoning capability.


==> contamination.tex <==
% %%%%%%%%%%%%%% New Addition to the contamination analysis section
% \subsection{Contamination Analysis}
% \label{sec:contamination_analysis}

% \subsubsection{Multi-Dimensional Benchmark Contamination}
% \label{sec:multidimensional_contamination}

% Mathematical reasoning benchmarks, such as MATH and GSM8K, serve as the primary mechanisms for evaluating the reasoning capabilities of large language models (LLMs). Traditional contamination studies primarily investigate verbatim duplication between training and testing corpora. However, LLMs learn statistical regularities rather than memorize documents character-by-character. Consequently, benchmark problems frequently differ at the surface level while sharing identical mathematical templates, semantic reasoning patterns, or proof structures. 

% To capture these hidden relationships, this evaluation employs a multi-dimensional framework spanning four complementary metrics: lexical overlap, semantic similarity, structural topology, and procedural solution-path alignment. These dimensions integrate into a Composite Contamination Index (CCI), which quantifies the contamination severity of individual benchmark problems.

% \subsubsection{Contamination Across the Benchmark's Subject--Level Structure}
% \label{sec:contamination_distribution}

% The MATH benchmark is natively organized as a $7 \times 5$ grid of seven subjects and five difficulty levels, yielding 35 subject--level cohorts per model. Rather than treating this structure purely as a set of fixed effects to control away, we use it as a second axis of the contamination analysis alongside the four similarity dimensions. This allows the analysis to determine not only \emph{which} dimension of contamination is associated with accuracy, but \emph{where in the benchmark} contamination is concentrated, and whether that concentration coincides with where accuracy is highest.

% \paragraph{Contamination Declines With Difficulty}
% Examining the Contamination Index (CI) across difficulty levels within each subject (Table~\ref{tab:ci_by_subject_level}) reveals a consistent pattern: contamination is highest at Level 1 and declines toward Level 5 in every one of the seven subjects, though the magnitude of the decline varies substantially. Geometry and Precalculus show the steepest declines (Pearson $r = -0.91$ and $r = -0.91$ between CI and level, respectively, computed within-subject across the five levels), while Prealgebra and Algebra show comparatively flat profiles ($r = -0.47$ and $r = -0.52$). Precalculus moves from a Level-1 CI of 0.56---the highest value observed anywhere in the benchmark---to 0.45 at Level 5; Geometry moves from 0.52 to 0.44 over the same range.

% \begin{table}[ht]
% \centering
% \caption{Contamination Index by subject and difficulty level (Level 1 through Level 5), condensed from the full subject--level breakdown. The within-subject correlation column reports the Pearson correlation between CI and difficulty level (1--5) for that subject.}
% \label{tab:ci_by_subject_level}
% \begin{tabular}{lccccc c}
% \toprule
% \textbf{Subject} & \textbf{L1} & \textbf{L2} & \textbf{L3} & \textbf{L4} & \textbf{L5} & \textbf{$r$ (CI vs.\ level)} \\
% \midrule
% Precalculus               & 0.56 & 0.49 & 0.48 & 0.47 & 0.45 & $-0.91$ \\
% Geometry                  & 0.52 & 0.52 & 0.50 & 0.49 & 0.44 & $-0.91$ \\
% Algebra                   & 0.49 & 0.51 & 0.50 & 0.50 & 0.47 & $-0.52$ \\
% Number Theory             & 0.49 & 0.48 & 0.49 & 0.47 & 0.46 & $-0.85$ \\
% Prealgebra                & 0.49 & 0.48 & 0.47 & 0.49 & 0.47 & $-0.47$ \\
% Counting \& Probability   & 0.47 & 0.48 & 0.47 & 0.47 & 0.46 & $-0.67$ \\
% Intermediate Algebra      & 0.47 & 0.47 & 0.48 & 0.45 & 0.45 & $-0.71$ \\
% \bottomrule
% \end{tabular}
% \end{table}

% This decline coincides directly with the level effect observed for accuracy: accuracy falls sharply at higher levels relative to Level 1, after controlling for subject and model. Contamination and accuracy therefore co-move across the benchmark's difficulty structure. This indicates that the easier end of the MATH benchmark is also the end most exposed to train--test overlap. Consequently, reported gains on lower-difficulty problems are disproportionately likely to reflect benchmark familiarity rather than reasoning ability, while the harder end of the benchmark is comparatively under-contaminated and therefore a more trustworthy signal of reasoning ability.

% \subsubsection{The Influence of Contamination on Evaluation Accuracy}
% \label{sec:influence_on_accuracy}

% To formally isolate the impact of contamination on model performance, a two-way fixed-effects regression isolates subject-specific difficulty and model-specific capabilities. Table \ref{tab:regression_results} summarizes the estimated regression coefficients.

% \begin{table}[ht]
% \centering
% \caption{Two-way fixed-effects regression relating benchmark contamination to benchmark accuracy.}
% \label{tab:regression_results}
% \begin{tabular}{lccc}
% \toprule
% \textbf{Variable} & \textbf{Coefficient ($\beta$)} & \textbf{t-statistic} & \textbf{p-value} \\
% \midrule
% Severe Contamination Rate & 3.044 & 9.414 & $<0.001$ \\
% Qwen2.5-Math-7B-Instruct & +24.084 & 6.680 & $<0.001$ \\
% WizardMath-7B & -42.116 & -11.681 & $<0.001$ \\
% \bottomrule
% \end{tabular}
% \end{table}

% The regression yields a highly significant, positive coefficient ($\beta=3.044$, $p<0.001$) for contamination severity. This indicates that benchmark cohorts containing higher proportions of severely contaminated problems consistently produce higher evaluation accuracy across diverse models. Evaluation performance is therefore partially conditioned by characteristics already embedded within the benchmark itself, rather than reflecting completely independent mathematical reasoning ability.

% \paragraph{Dimensional Decomposition Within the Subject--Level Structure}
% The regression in Table~\ref{tab:regression_results} uses the severe-contamination rate the proportion of problems per cohort whose Composite Contamination Index exceeds the critical threshold (CCI $> 0.70$) as a single binary severity-derived predictor. The decomposition that follows instead uses the continuous, per-cohort mean of each individual similarity dimension (mean lexical, semantic, and structural similarity, prior to thresholding), in order to assess each dimension's independent contribution rather than its contribution to the composite severity classification alone. Holding the subject--level structure fixed, we decompose the composite contamination index into its constituent lexical, semantic, and structural dimensions to assess which type of overlap is most associated with accuracy. Entered individually, lexical ($\beta = 3.71$, $p < 0.001$) and semantic ($\beta = 4.00$, $p < 0.001$) similarity are each strongly associated with accuracy; structural similarity is not ($\beta = 0.46$, $p = 0.266$). Entered jointly, only lexical similarity remains significant ($\beta = 4.04$, $p < 0.001$); semantic ($\beta = -1.08$, $p = 0.208$) and structural ($\beta = -0.09$, $p = 0.781$) similarity do not. This is consistent with substantial shared variance between lexical and semantic similarity ($r = 0.75$ across the 35 cohorts): once lexical overlap is in the model, semantic overlap adds little independent explanatory power.

% A model-specific decomposition, estimating the composite-contamination slope separately within each model's 35 cohorts, shows this association holds for every evaluated model (Table~\ref{tab:composite_by_model}). This confirms that composite contamination is associated with higher accuracy across the full model population, not only the weakest models.

% \begin{table}[ht]
% \centering
% \caption{Model-specific association between composite contamination and accuracy, estimated independently within each model's 35 subject--level cohorts.}
% \label{tab:composite_by_model}
% \begin{tabular}{lcc}
% \toprule
% \textbf{Model} & \textbf{Slope ($\beta$)} & \textbf{p-value} \\
% \midrule
% Qwen2.5-Math-1.5B            & $+4.101$ & $<0.001$ \\
% DeepSeek-Math-7B-RL          & $+3.963$ & $<0.001$ \\
% NuminaMath-7B-CoT            & $+3.695$ & 0.001 \\
% Qwen2.5-Math-7B-Instruct     & $+2.928$ & 0.001 \\
% DeepSeek-Math-7B-Base        & $+2.382$ & $<0.001$ \\
% WizardMath-7B-V1.0           & $+1.197$ & 0.011 \\
% \bottomrule
% \end{tabular}
% \end{table}

% Decomposed by dimension instead of by model, structural contamination's weak aggregate association also masks model-level heterogeneity. Only Qwen2.5-Math-1.5B ($\beta = 1.05$, $p = 0.016$) and DeepSeek-Math-7B-Base ($\beta = 0.65$, $p = 0.034$) show a significant dependence on structural overlap specifically (Table~\ref{tab:structural_by_model}). Notably, these are the only two \emph{base} models in our evaluation --- neither has undergone instruction tuning or reinforcement-learning-based alignment, unlike the remaining four models (Qwen2.5-Math-7B-Instruct, DeepSeek-Math-7B-RL, NuminaMath-7B-CoT, and WizardMath-7B-V1.0, each of which is instruction-tuned, RL-aligned, or CoT-distilled). The four post-trained models show no significant structural dependency, suggesting that reliance on abstract template matching may be specifically associated with the absence of post-training alignment, rather than with model scale or overall capability alone --- a distinction the size gap between Qwen2.5-Math-1.5B (1.5B parameters) and DeepSeek-Math-7B-Base (7B parameters) helps to disentangle, since both show the effect despite differing substantially in size.

% \begin{table}[ht]
% \centering
% \caption{Model-specific slope of accuracy on structural contamination alone.}
% \label{tab:structural_by_model}
% \begin{tabular}{lcc}
% \toprule
% \textbf{Model} & \textbf{Slope ($\beta$)} & \textbf{p-value} \\
% \midrule
% Qwen2.5-Math-1.5B            & $+1.048$ & 0.016 \quad (significant) \\
% DeepSeek-Math-7B-Base        & $+0.649$ & 0.034 \quad (significant) \\
% DeepSeek-Math-7B-RL          & $+0.749$ & 0.121 \\
% Qwen2.5-Math-7B-Instruct     & $+1.006$ & 0.105 \\
% NuminaMath-7B-CoT            & $+0.485$ & 0.302 \\
% WizardMath-7B-V1.0           & $-0.103$ & 0.722 \\
% \bottomrule
% \end{tabular}
% \end{table}

% This dimensional decomposition also reconciles an apparent tension with Table~\ref{tab:regression_results}: the composite severity rate is strongly predictive of accuracy in aggregate even though structural similarity, one of its four constituent dimensions, shows little independent association once lexical and semantic similarity are accounted for. Because the composite index combines all four dimensions, its predictive power is driven predominantly by the lexical, semantic, and solution-path components; structural similarity contributes comparatively little to the composite's association with accuracy, but its inclusion does not weaken the composite measure, since the weighting scheme (Section~\ref{sec:multidimensional_contamination}) allows the stronger dimensions to dominate the aggregate signal.

% \begin{figure}[ht]
% \centering
% \begin{tikzpicture}
% \begin{axis}[
%     width=0.75\textwidth,
%     height=8cm,
%     xlabel={Contamination Exposure Rate (\%)},
%     ylabel={Predicted Benchmark Accuracy (\%)},
%     legend pos=outer north east,
%     legend style={font=\footnotesize, fill=white, fill opacity=0.8, draw opacity=1, text opacity=1},
%     grid=both,
%     grid style={dashed, gray!30},
%     xmin=0, xmax=10,
%     ymin=0, ymax=100,
%     thick,
%     tick label style={font=\small},
%     label style={font=\small\bfseries}
% ]

% % 1. Qwen2.5-Math-7B-Instruct (Baseline: 47.60 + 24.08 = 71.68)
% \addplot[color=blue, mark=*, mark repeat=2, domain=0:10, line width=1.2pt] {71.68 + 2.928*x};
% \addlegendentry{Qwen2.5-Instruct 7B}

% % 2. Qwen2.5-Math-1.5B (Baseline: 47.60 + 0.70 = 48.30)
% \addplot[color=cyan, mark=square*, mark repeat=2, domain=0:10, line width=1.2pt] {48.30 + 4.101*x};
% \addlegendentry{Qwen2.5 1.5B}

% % 3. NuminaMath-7B-CoT (Baseline: Reference Intercept = 47.60)
% \addplot[color=green!60!black, mark=triangle*, mark repeat=2, domain=0:10, line width=1.2pt] {47.60 + 3.695*x};
% \addlegendentry{NuminaMath-CoT 7B}

% % 4. DeepSeek-Math-7B-RL (Baseline: 47.60 - 3.38 = 44.22)
% \addplot[color=orange, mark=diamond*, mark repeat=2, domain=0:10, line width=1.2pt] {44.22 + 3.963*x};
% \addlegendentry{DeepSeek-RL 7B}

% % 5. DeepSeek-Math-7B-Base (Baseline: 47.60 - 32.02 = 15.58)
% \addplot[color=red, mark=x, mark size=3pt, mark repeat=2, domain=0:10, line width=1.2pt] {15.58 + 2.382*x};
% \addlegendentry{DeepSeek-Base 7B}

% % 6. WizardMath-7B-V1.0 (Baseline: 47.60 - 42.12 = 5.48)
% \addplot[color=purple, mark=+, mark size=3pt, mark repeat=2, domain=0:10, line width=1.2pt] {5.48 + 1.197*x};
% \addlegendentry{WizardMath V1.0}

% \end{axis}
% \end{tikzpicture}
% \caption{Predicted evaluation accuracy as a function of benchmark contamination exposure. Line origins represent the normalized fixed-effects baseline for each model, while the slopes correspond to the model-specific contamination sensitivity coefficient ($\beta$).}
% \label{fig:accuracy_vs_contamination}
% \end{figure}

% \paragraph{An Exploratory Fourth Dimension: Solution-Path Similarity}
% The three dimensions analyzed above are grounded in established, externally validated measures. We additionally constructed a fourth, exploratory dimension: solution-path similarity, intended to capture overlap in the \emph{procedure} used to solve a problem independent of its lexical or structural form. Extracted by parsing reference solutions for transition operators (e.g., \emph{Substitute}, \emph{Simplify}, \emph{Therefore}), this dimension serves as a strong individual predictor of accuracy ($\beta = 1.94$, $p < 0.001$). However, because this operator vocabulary was explicitly defined for this framework rather than adopted from a universally validated baseline, we present the solution-path finding as a motivating exploratory result rather than a definitive claim, identifying procedural similarity quantification as a key area for future methodology research.

% \begin{figure}[ht]
% \centering
% \begin{tikzpicture}
% \begin{axis}[
%     ybar,
%     bar width=20pt,
%     width=0.95\textwidth,
%     height=6.5cm,
%     ylabel={Contamination Sensitivity ($\beta$)},
%     symbolic x coords={Qwen-1.5B, DeepSeek-RL, Numina-CoT, Qwen-Instruct, DeepSeek-Base, WizardMath},
%     xtick=data,
%     xticklabel style={rotate=15, anchor=north, font=\footnotesize},
%     nodes near coords,
%     nodes near coords align={vertical},
%     every node near coord/.append style={font=\footnotesize},
%     ymin=0, ymax=4.8,
%     enlarge x limits=0.15,
%     axis lines*=left,
%     ymajorgrids=true,
%     grid style={dashed, gray!30}
% ]

% \addplot[fill=blue!60, draw=blue!80!black, thick] coordinates {
%     (Qwen-1.5B,4.101) 
%     (DeepSeek-RL,3.963) 
%     (Numina-CoT,3.695) 
%     (Qwen-Instruct,2.928) 
%     (DeepSeek-Base,2.382) 
%     (WizardMath,1.197)
% };

% \end{axis}
% \end{tikzpicture}
% \caption{Model-specific sensitivity to benchmark contamination. The slope ($\beta$) indicates the expected percentage-point increase in evaluation accuracy for every unit increase in severe contamination exposure. Higher values indicate that a model's accuracy tracks contamination more aggressively.}
% \label{fig:contamination_sensitivity}
% \end{figure}

% \subsubsection{Output Similarity and Semantic Mimicry (The ``Clever Hans'' Effect)}
% \label{sec:semantic_mimicry}

% A direct behavioural analysis comparing model-generated solutions against benchmark reference solutions reveals how LLMs exploit this contaminated knowledge. Across representative models evaluated on both the MATH and GSM8K datasets, exact verbatim memorization remains at exactly $0\%$.

% Despite the absence of literal copying, generated responses exhibit remarkably high semantic similarity to the reference solutions. Table \ref{tab:semantic_mimicry} demonstrates the ``Semantic Plateau'' effect: semantic similarity remains persistently high even when the generated mathematical conclusion is entirely incorrect.

% \begin{table}[ht]
% \centering
% \caption{Cross-benchmark behavioural comparison: GSM8K accuracy alongside MATH-benchmark semantic similarity between generated responses and reference solutions, split by mathematical correctness on MATH. Accuracy and semantic-similarity columns are computed on different benchmarks for the same models, illustrating that the semantic-mimicry pattern observed on MATH (Section~\ref{sec:semantic_mimicry}) co-occurs with widely varying absolute accuracy on an independent benchmark. Statistical significance (p-value) represents the Welch's t-test difference between MATH correct and incorrect semantic similarity distributions.}
% \label{tab:semantic_mimicry}
% \begin{tabular}{llm{2cm}m{2cm}l}
% \toprule
% \textbf{Model} & \textbf{Acc (\%)} & \textbf{Correct Semantic} & \textbf{Incorrect Semantic} & \textbf{p-value} \\
% \midrule
% Qwen2.5-Math-7B-Instruct & 89.0 & 81.58\% & 80.29\% & $0.0018$ \\
% NuminaMath-7B-CoT        & 57.0 & 80.73\% & 79.06\% & $0.0045$ \\
% DeepSeek-Math-7B-RL      & 72.0 & 83.57\% & 80.74\% & $0.0012$ \\
% WizardMath-7B-V1.0       & 21.0 & 53.96\% & 63.60\% & $0.0047$ \\
% \bottomrule
% \end{tabular}
% \end{table}

% As illustrated in Figure \ref{fig:semantic_plateau}, highly instruction-tuned models frequently exhibit only a negligible difference (e.g., $\sim 1-2\%$) in semantic alignment between their correct and incorrect responses. 

% \begin{figure}[ht]
% \centering
% \begin{tikzpicture}
% \begin{axis}[
%     ybar,
%     bar width=15pt,
%     width=0.9\textwidth,
%     height=6cm,
%     enlarge x limits=0.2,
%     legend style={at={(0.5,-0.25)}, anchor=north, legend columns=-1},
%     ylabel={Semantic Similarity (\%)},
%     symbolic x coords={Qwen2.5-Instruct, NuminaMath-CoT, DeepSeek-RL, WizardMath},
%     xtick=data,
%     xticklabel style={rotate=8, anchor=north, style={font=\footnotesize}}, 
%     nodes near coords,
%     nodes near coords align={vertical},
%     every node near coord/.append style={font=\tiny}, 
%     ymin=40, ymax=100,
%     ]
% \addplot coordinates {(Qwen2.5-Instruct,81.5) (NuminaMath-CoT,80.7) (DeepSeek-RL,83.5) (WizardMath,53.9)};
% \addplot coordinates {(Qwen2.5-Instruct,80.2) (NuminaMath-CoT,79.0) (DeepSeek-RL,80.7) (WizardMath,63.6)};
% \legend{Correct Generation, Incorrect Generation}
% \end{axis}
% \end{tikzpicture}
% \caption{Comparison of semantic similarity distributions. The minimal delta between successful and unsuccessful generations demonstrates the models' rigid adherence to learned linguistic framing, independent of logical execution.}
% \label{fig:semantic_plateau}
% \end{figure}

% This behaviour demonstrates that models rigidly adhere to the learned linguistic framing and conceptual organization of the training distribution. They successfully map the problem to a familiar semantic gradient but frequently fail to execute the underlying logic. These empirical findings indicate that current mathematical language models often reproduce the semantic style, reasoning vocabulary, and discourse patterns of benchmark solutions, acting as advanced pattern matchers rather than independent symbolic reasoners. 

% \subsubsection{Synthesis}
% \label{sec:contamination_synthesis}

% Three primary conclusions emerge from analyzing contamination jointly with the benchmark's subject--level structure and model output behaviour. First, contamination is not uniformly distributed across difficulty: within every subject, the Contamination Index is highest at Level 1 and declines toward Level 5, coinciding with a steep decline in accuracy across the same levels. Easier problems are therefore both more contaminated and more accurately solved, strengthening the claim that reported benchmark accuracy partially reflects benchmark exposure rather than reasoning ability. 

% Second, composite contamination is associated with higher accuracy for every evaluated model. The decomposition of this contamination into lexical, semantic, and structural dimensions is sensitive to model specification due to substantial shared variance among the dimensions, with structural overlap specifically concentrated in the smallest and least heavily post-trained models. 

% Third, output behaviour is consistent with a pronounced ``Clever Hans'' effect. By continuously matching the semantic distribution of the training data regardless of mathematical correctness, instruction-tuned models successfully exploit the contamination gradients identified in the earlier regressions. Consequently, benchmark accuracy functions as a composite metric---reflecting both genuine reasoning capability and prior statistical exposure to benchmark-specific distributions.



==> img/fig_1.tex <==
\begin{figure}[t]
    \centering
    \caption{\textbf{Top:} Math word problem. \textbf{Bottom:} Step-by-step erroneous solution.}
    \label{fig:fig_1}
    \scalebox{1}{
    \begin{tcolorbox}[colback=white, colframe=blue!30, colbacktitle=blue!20, coltitle=black, title=Input,width=\linewidth, fontupper=\scriptsize, fonttitle=\scriptsize]
    
    Question:\\
    Dane's two daughters need to plant a certain number of flowers each to grow a garden. As the days passed, the flowers grew into 20 more but 10 of them died. Dane's daughters harvested the flowers and split them between 5 different baskets, with 4 flowers in each basket. How many flowers did each daughter plant initially?\\
    
    Answer:\\
    
    \end{tcolorbox}
    }
    \scalebox{1}{
    \begin{tcolorbox}[colback=white, colframe=blue!30, colbacktitle=blue!20, coltitle=black, title=Step-by-Step Solution,width=\linewidth, fontupper=\scriptsize, fonttitle=\scriptsize,  before upper={
    \setlength{\abovedisplayskip}{4pt}
    \setlength{\belowdisplayskip}{4pt}
    \setlength{\abovedisplayshortskip}{2pt}
    \setlength{\belowdisplayshortskip}{2pt}
  }]
    
    Calculate the total number of flowers harvested: Dane's daughters split the flowers into 5 baskets, with 4 flowers in each basket. The total number of flowers harvested is: 
    \[5 \times 4 = 20 \ \text{flowers}\]
    Account for the flowers that grew and died: The problem states that 20 additional flowers grew, but 10 of them died. Let the initial number of flowers planted by the two daughters be \(x\). After accounting for the growth and death of flowers, the total number of flowers becomes: 
    \[x + 20 - 10 = x + 10\]
    Set up the equation for the total flowers harvested: The total number of flowers harvested is equal to the total number of flowers after growth and death:  
    \[x + 10 = 20\]
    Solve for \(x\): Subtract 10 from both sides:  
    \[x = 10\]
    Determine how many flowers each daughter planted: The two daughters together planted \(x = 10\) flowers. Since the flowers were planted equally between the two daughters, each daughter planted:  
    \[\frac{10}{2} = 5 \ \text{flowers}\]
    Final Answer:  
    6
    \end{tcolorbox}
    }

\end{figure}

==> img/fig_3.tex <==

% % \begin{figure}[htbp]
% % \centering
% % \footnotesize
% % \begin{tikzpicture}[
% %   node distance=2mm and 3mm,
% %   box/.style={
% %     rectangle,
% %     draw,
% %     align=center,
% %     rounded corners=4pt,
% %     minimum width=5cm,
% %     minimum height=1.5cm,
% %     font=\tiny,
% %     fill=white
% %   },
% %   labelbox/.style={
% %     rectangle,
% %     rounded corners=4pt,
% %     fill=blue!20,
% %     text width=1.7cm,
% %     align=center,
% %     font=\tiny\bfseries,
% %     minimum height=0.5cm
% %   },
% %   arrow/.style={-Latex, thick}
% % ]
% % \node[labelbox, rotate=90] (label1) at (-4,-0.4) {Identification};
% % \node[labelbox, rotate=90] (label2) at (-4,-3.15) {Screening};
% % \node[labelbox, rotate=90] (label3) at (-4,-6.2) {Included};


% % \node[box] (idleft) at (-0.3,-0.2) {Records identified from:\\Databases\\(n = 5)};
% % \node[box, right=9mm of idleft] (idright) {Articles removed before screening:\\Duplicate records\\(n = 132))};


% % \node[box, below=6mm of idleft] (screenleft) {Articles screened\\(n = 939)};
% % \node[box, right=9mm of screenleft] (screenright) {Articles excluded:\\Publishing Year\\(n = 180)\\Full-Text (n = 36)};
% % \node[box, below=4mm of screenleft] (assessleft) {Articles assessed for\\eligibility\\(n = 723)};
% % \node[box, right=9mm of assessleft] (assessright) {Articles excluded:\\Title (n = 282)\\Abstract (n = 112)\\Topic-Relevancy (n = 116)};

% % \node[box, below=6mm of assessleft] (includedleft) {Included Articles\\(n = 213)};

% % \draw[arrow] (idleft) -- (screenleft);
% % \draw[arrow] (screenleft) -- (assessleft);
% % \draw[arrow] (assessleft) -- (includedleft);

% % \draw[arrow] (idright.west) -- (idleft.east);
% % \draw[arrow] (screenright.west) -- (screenleft.east);
% % \draw[arrow] (assessright.west) -- (assessleft.east);

% % \end{tikzpicture}
% % \caption{SLR flow diagram of study selection}
% % \label{fig:prisma}
% % \end{figure}

% \begin{figure}[t]
% \centering

% \caption{PRISMA flow diagram of the systematic literature review selection process}
% \label{fig:fig_3}

% \footnotesize
% \begin{tikzpicture}[
%   node distance=8mm and 12mm, % Increased spacing for better arrow visibility
%   box/.style={
%     rectangle,
%     draw,
%     align=center,
%     rounded corners=4pt,
%     minimum width=5.5cm,
%     minimum height=1.5cm,
%     font=\scriptsize, % Slightly larger than tiny for readability
%     fill=white
%   },
%   labelbox/.style={
%     rectangle,
%     rounded corners=4pt,
%     fill=blue!20,
%     text width=2.5cm,
%     align=center,
%     font=\scriptsize\bfseries,
%     minimum height=0.8cm
%   },
%   labelbox1/.style={
%     rectangle,
%     rounded corners=4pt,
%     fill=blue!20,
%     text width=3cm,
%     align=center,
%     font=\scriptsize\bfseries,
%     minimum height=0.8cm
%   },
%   arrow/.style={-Latex, thick}
% ]

% % ==================== LABELS ====================
% \node[labelbox, rotate=90] (label1) at (-4,-0.9) {Identification};
% \node[labelbox1, rotate=90] (label2) at (-4,-4.1) {Screening};
% \node[labelbox, rotate=90] (label3) at (-4,-7.3) {Included};

% % ==================== IDENTIFICATION ====================
% \node[box] (idleft) at (-0.3,-0.4) {Records identified from:\\Databases (n = 271,100)};

% \node[box, right=12mm of idleft] (idright) {Records removed before screening:\\Extraction API Limits (n = 12,679)\\Duplicate records (n = 3,720)};

% % ==================== SCREENING ====================
% \node[box, below=12mm of idleft] (screenleft) {Records screened\\(n = 8,959)};

% \node[box, right=12mm of screenleft] (screenright) {Records excluded:\\Title screening (n = 17,534)};

% \node[box, below=5mm of screenleft] (assessleft) {Reports assessed for eligibility\\(n = 12,691)};

% \node[box, right=12mm of assessleft] (assessright) {Reports excluded:\\Abstract screening (n = 12,478)};

% % ==================== INCLUDED ====================
% \node[box, below=12mm of assessleft] (includedleft) {Included Articles\\(n = 213)};

% % ==================== ARROWS ====================
% % Vertical main flow arrows
% \draw[arrow] (idleft) -- (screenleft);
% \draw[arrow] (screenleft) -- (assessleft);
% \draw[arrow] (assessleft) -- (includedleft);

% % Horizontal exclusion arrows (Pointing OUTWARD to the right)
% \draw[arrow] (idleft.east) -- (idright.west);
% \draw[arrow] (screenleft.east) -- (screenright.west);
% \draw[arrow] (assessleft.east) -- (assessright.west);

% \end{tikzpicture}

% \end{figure}

\begin{figure}[t]
\centering

\caption{PRISMA flow diagram of the systematic literature review selection process}
\label{fig:fig_3}

\footnotesize
\begin{tikzpicture}[
  node distance=8mm and 12mm, 
  box/.style={
    rectangle,
    draw,
    align=center,
    rounded corners=4pt,
    minimum width=5.5cm,
    minimum height=1.5cm,
    font=\scriptsize, 
    fill=white
  },
  labelbox/.style={
    rectangle,
    rounded corners=4pt,
    fill=blue!20,
    text width=2.5cm,
    align=center,
    font=\scriptsize\bfseries,
    minimum height=0.8cm
  },
  labelbox1/.style={
    rectangle,
    rounded corners=4pt,
    fill=blue!20,
    text width=3cm,
    align=center,
    font=\scriptsize\bfseries,
    minimum height=0.8cm
  },
  arrow/.style={-Latex, thick}
]

% ==================== LABELS ====================
\node[labelbox, rotate=90] (label1) at (-4,-0.9) {Identification};
\node[labelbox1, rotate=90] (label2) at (-4,-4.1) {Screening};
\node[labelbox, rotate=90] (label3) at (-4,-7.3) {Included};

% ==================== IDENTIFICATION ====================
\node[box] (idleft) at (-0.3,-0.4) {Records identified from:\\Databases (n = 271,100)};

\node[box, right=12mm of idleft] (idright) {Records removed before screening:\\Unretrieved / API Limits (n = 258,421)\\Intra-database duplicates (n = 3,720)\\Cross-database duplicates (n = 1,408)};

% ==================== SCREENING ====================
\node[box, below=12mm of idleft] (screenleft) {Records screened\\(n = 7,551)};

\node[box, right=12mm of screenleft] (screenright) {Records excluded:\\Title screening (n = 6,145)};

\node[box, below=5mm of screenleft] (assessleft) {Reports assessed for eligibility\\(n = 1,406)};

\node[box, right=12mm of assessleft] (assessright) {Reports excluded:\\Abstract screening (n = 1,286)};

% ==================== INCLUDED ====================
\node[box, below=12mm of assessleft] (includedleft) {Included Articles\\(n = 120)};

% ==================== ARROWS ====================
% Vertical main flow arrows
\draw[arrow] (idleft) -- (screenleft);
\draw[arrow] (screenleft) -- (assessleft);
\draw[arrow] (assessleft) -- (includedleft);

% Horizontal exclusion arrows (Pointing OUTWARD to the right)
\draw[arrow] (idleft.east) -- (idright.west);
\draw[arrow] (screenleft.east) -- (screenright.west);
\draw[arrow] (assessleft.east) -- (assessright.west);

\end{tikzpicture}

\end{figure}

==> img/flow.tex <==
\begin{figure}[htbp]
    \centering
    % Scales the diagram to fit perfectly within the text width
    \resizebox{0.75\textwidth}{!}{
    \begin{tikzpicture}[
        % Define styles for the nodes to ensure uniformity
        mainnode/.style={
            circle, 
            draw=black, 
            thick, 
            fill=white, 
            minimum size=2.6cm, 
            align=center, 
            font=\sffamily\scriptsize, 
            inner sep=1pt
        },
        dashednode/.style={
            circle, 
            draw=black, 
            thick, 
            dashed, 
            fill=white, 
            minimum size=2.6cm, 
            align=center, 
            font=\sffamily\scriptsize, 
            inner sep=1pt
        },
        % Standard arrow style for node connections
        arr/.style={
            thick, 
            ->, 
            >=stealth
        },
        % Style for the parallel boundary arrows
        lblarrow/.style={
            <->, 
            thick, 
            blue!50
        },
        lbltext/.style={
            midway, 
            sloped, 
            above=2pt,
            font=\bfseries\sffamily\small, 
            text=blue!50
        },
        labeltext/.style={
            midway, 
            sloped, 
            below=2pt,
            font=\bfseries\sffamily\small, 
            text=blue!50
        }
    ]

    % =========================================================
    % 1. MAIN NODES (Solid Circles)
    % Placed along two parallel diagonal lanes (Upper and Lower)
    % =========================================================
    
    % Upper Lane Nodes
    \node[mainnode] (S1) at (1.0, 2.56) {\textbf{Step 1:}\\Set Research\\objectives};
    \node[mainnode] (S2) at (3.5, 4.11) {\textbf{Step 2:}\\Define\\Literature\\Scope};
    \node[mainnode] (S3) at (6.0, 5.66) {\textbf{Step 3:}\\Select\\Keywords};
    
    % Lower Lane Nodes
    \node[mainnode] (S4) at (7.0, 0.72) {\textbf{Step 4:}\\Formulate \&\\Execute\\Queries};
    \node[mainnode] (S5) at (9.5, 1.87) {\textbf{Step 5:}\\Article Section\\to be searched};
    \node[mainnode] (S6) at (12.0, 3.02) {\textbf{Step 6:}\\Apply Filters:\\- Inclusion\\- Exclusion};
    
    % Upper Lane Nodes (Continued)
    \node[mainnode] (S7) at (10.0, 7.83) {\textbf{Step 7:}\\Conduct\\synthesis on\\screened\\articles};
    \node[mainnode] (S8) at (12.3, 9.18) {\textbf{Step 8:}\\Conclude the\\findings};

    % =========================================================
    % 2. DASHED NODES (Sub-categories)
    % =========================================================
    
    \node[dashednode] (D1) at (1.5, 6.7) {
        \begin{tabular}{@{}l@{}}
            $\bullet$ Search\\ \ \ Engines\\
            $\bullet$ Publication\\ \ \ Tenure\\
            $\bullet$ Article Type
        \end{tabular}
    };
    
    \node[dashednode] (D2) at (4.0, 8.2) {
        \begin{tabular}{@{}l@{}}
            $\bullet$ Primary\\
            $\bullet$ Secondary
        \end{tabular}
    };
    
    % \node[dashednode] (D3) at (6.7, 8.8) {Select\\Operators\\for the Keywords\\based on retrieved\\results};
    
    % \node[dashednode] (D4) at (12.5, -0.1) {
    %     \begin{tabular}{@{}l@{}}
    %         - Language\\
    %         - Status\\
    %         - Access
    %     \end{tabular}
    % };

    % =========================================================
    % 3. CONNECTING ARROWS BETWEEN NODES
    % =========================================================
    
    \draw[arr] (S2) -- (D1);
    \draw[arr] (S3) -- (D2);

    % =========================================================
    % 4. DIAGONAL FOOTPRINT TRACK
    % Placed explicitly between the Upper and Lower Lanes
    % =========================================================
    
    \foreach \pos in {0.0, 0.1, 0.2, 0.3, 0.4, 0.5, 0.6, 0.7, 0.8, 0.9, 1.0} {
        % \faShoePrints natively points UP, rotating by -65 degrees aligns it with the 25-degree diagonal path.
        \node[rotate=25, text=black!85, font=\Large] at ($(1.5, 0.69)!\pos!(13.5, 6.21)$) {\faShoePrints};
    }

    % =========================================================
    % 5. PARALLEL TEXT ARROWS (Blue Boundaries)
    % =========================================================
    
    % Starting of Research (Bottom Left)
    \draw[lblarrow] (1.5, 0.09) -- (5.5, 1.9) node[labeltext] {Starting of Research};
    
    % Screening of Results (Middle, between footprints and upper lane)
    \draw[lblarrow] (4.5, 2.87) -- (9.5, 5.17) node[lbltext] {Screening of Results};
    
    % Systematic Review (Top Right)
    \draw[lblarrow] (10.50, 5.66) -- (14.0, 7.24) node[lbltext] {Systematic Review};

    \end{tikzpicture}
    }
    \caption{Eight steps of the search process followed for finding the related work.}
    \label{fig:search_process}
\end{figure}

==> img/rnn_architecture.tex <==
\begin{figure}[t]
    \centering
\usetikzlibrary{arrows.meta, calc}

\tikzset{
  node style/.style={circle, draw, minimum size=4mm, font=\small},
  hidden style/.style={rectangle, rounded corners=2pt, draw, minimum width=8mm, minimum height=6mm, fill=green!20, font=\small},
  arrow/.style={-Latex, thick}
}

\begin{tikzpicture}[>=Latex]

\def\xsep{1.8cm} 
\def\ysep{1.3cm}  

\node[hidden style] (rnn) at (-\xsep,0) {RNN};
\node[node style, fill=orange!60] (X_T) at ($(rnn)+(0,-\ysep)$) {$X_T$};
\node[node style, fill=blue!40]   (Y_T) at ($(rnn)+(0,\ysep)$)  {$Y_T$};

\node[hidden style] (h0) at (0,0)                  {$h_{T-n}$};
\node[hidden style] (h1) at (\xsep,0)              {$h_{t}$};
\node[hidden style] (h2) at (2*\xsep,0)            {$h_{T-1}$};

\node[node style, fill=orange!60] (x0) at (0,-\ysep)      {$x_{T-n}$};
\node[node style, fill=orange!60] (x1) at (\xsep,-\ysep)  {$x_{t}$};
\node[node style, fill=orange!60] (x2) at (2*\xsep,-\ysep){$x_{T-1}$};

\node[node style, fill=blue!40] (y0) at (0,\ysep)       {$y_{T-n}$};
\node[node style, fill=blue!40] (y1) at (\xsep,\ysep)   {$y_{t}$};
\node[node style, fill=blue!40] (y2) at (2*\xsep,\ysep) {$y_{T-1}$};

\draw[arrow] (X_T) -- (rnn);
\draw[arrow] (rnn) -- (Y_T);
\draw[arrow] (rnn.north west) .. controls +(-0.75,1.0) and +(-1.0,-0.50) .. (rnn.south west);

\node at ($(rnn.east)!0.5!(h0.west)$) {\Large $=$};

\draw[arrow] (x0) -- node[midway,right]  {$W_{xh}$} (h0);
\draw[arrow] (x1) -- node[midway,right]  {$W_{xh}$} (h1);
\draw[arrow] (x2) -- node[midway,right]  {$W_{xh}$} (h2);

\draw[arrow] (h0) -- node[midway,right] {$W_{hy}$} (y0);
\draw[arrow] (h1) -- node[midway,right] {$W_{hy}$} (y1);
\draw[arrow] (h2) -- node[midway,right] {$W_{hy}$} (y2);

\draw[arrow] (h0) -- node[midway,above] {$W_{hh}$} (h1);
\draw[arrow] (h1) -- node[midway,above] {$W_{hh}$} (h2);

\end{tikzpicture}
    \caption{RNN Architecture}
\end{figure}

==> old_reference_file.tex <==
@InProceedings{achiam2017constrained,
  title = 	 {Constrained Policy Optimization},
  author =       {Joshua Achiam and David Held and Aviv Tamar and Pieter Abbeel},
  booktitle = 	 {Proceedings of the 34th International Conference on Machine Learning},
  pages = 	 {22--31},
  year = 	 {2017},
  editor = 	 {Precup, Doina and Teh, Yee Whye},
  volume = 	 {70},
  series = 	 {Proceedings of Machine Learning Research},
  month = 	 {06--11 Aug},
  publisher =    {PMLR},
  url = 	 {https://proceedings.mlr.press/v70/achiam17a.html}
}


@inproceedings{ahn2024large,
    title = {Large Language Models for Mathematical Reasoning: Progresses and Challenges},
    author = {Ahn, Janice  and
      Verma, Rishu  and
      Lou, Renze  and
      Liu, Di  and
      Zhang, Rui  and
      Yin, Wenpeng},
    editor = {Falk, Neele  and
      Papi, Sara  and
      Zhang, Mike},
    booktitle = {Proceedings of the 18th Conference of the European Chapter of the Association for Computational Linguistics: Student Research Workshop},
    month = mar,
    year = {2024},
    address = {St. Julian{'}s, Malta},
    publisher = {Association for Computational Linguistics},
    url = {https://aclanthology.org/2024.eacl-srw.17/},
    doi = {10.18653/v1/2024.eacl-srw.17},
    pages = {225--237}
}

@article{ainslie2023gqa,
  title={Gqa: Training generalized multi-query transformer models from multi-head checkpoints},
  author={Ainslie, Joshua and Lee-Thorp, James and De Jong, Michiel and Zemlyanskiy, Yury and Lebr{\'o}n, Federico and Sanghai, Sumit},
  journal={arXiv preprint arXiv:2305.13245},
  year={2023}
}

@inbook{anton2025human,
author = {Anton, Jacqueline and Cosentino, Giulia and Sharma, Kshitij and Gelsomini, Mirko and Mok, Micah and Giannakos, Michail and Abrahamson, Dor},
title = {The Human Condition: Modal and Interactive Advantages of Teacher over AI Feedback on Children's Mathematical Performance},
year = {2025},
isbn = {9798400714733},
publisher = {Association for Computing Machinery},
address = {New York, NY, USA},
url = {https://doi.org/10.1145/3713043.3728863},
booktitle = {Proceedings of the 24th Interaction Design and Children},
pages = {183–203},
numpages = {21}
}

@misc{ausbrooks2003mathml,
  title={Mathematical Markup Language (MathML) Version 2.0},
  author={Ausbrooks, Ron and others},
  year={2003},
  publisher={W3C Recommendation},
  url={https://www.w3.org/TR/MathML2/}
}

@misc{azerbayev2023proofnet,
      title={ProofNet: Autoformalizing and Formally Proving Undergraduate-Level Mathematics}, 
      author={Zhangir Azerbayev and Bartosz Piotrowski and Hailey Schoelkopf and Edward W. Ayers and Dragomir Radev and Jeremy Avigad},
      year={2023},
      eprint={2302.12433},
      archivePrefix={arXiv},
      primaryClass={cs.CL},
      url={https://arxiv.org/abs/2302.12433}, 
}

@inproceedings{benedek2024prilora,
  title={PRILoRA: Pruned and Rank-Increasing Low-Rank Adaptation},
  author={Benedek, Nadav and Wolf, Lior},
  booktitle={Findings of the Association for Computational Linguistics: EACL 2024},
  pages={252--263},
  year={2024}
}

@inproceedings{bostrom2020byte,
    title = {Byte Pair Encoding is Suboptimal for Language Model Pretraining},
    author = {Bostrom, Kaj  and
      Durrett, Greg},
    editor = {Cohn, Trevor  and
      He, Yulan  and
      Liu, Yang},
    booktitle = {Findings of the Association for Computational Linguistics: EMNLP 2020},
    month = nov,
    year = {2020},
    address = {Online},
    publisher = {Association for Computational Linguistics},
    url = {https://aclanthology.org/2020.findings-emnlp.414/},
    doi = {10.18653/v1/2020.findings-emnlp.414},
    pages = {4617--4624}
}

@inproceedings{brown2020language,
 author = {Brown, Tom and Mann, Benjamin and Ryder, Nick and Subbiah, Melanie and Kaplan, Jared D and Dhariwal, Prafulla and Neelakantan, Arvind and Shyam, Pranav and Sastry, Girish and Askell, Amanda and Agarwal, Sandhini and Herbert-Voss, Ariel and others},
 booktitle = {Advances in Neural Information Processing Systems},
 pages = {1877--1901},
 publisher = {Curran Associates, Inc.},
 title = {Language Models are Few-Shot Learners},
 url = {https://proceedings.neurips.cc/paper_files/paper/2020/file/1457c0d6bfcb4967418bfb8ac142f64a-Paper.pdf},
 volume = {33},
 year = {2020}
}


@ARTICLE{cai2025survey,
  author={Cai, Weilin and Jiang, Juyong and Wang, Fan and Tang, Jing and Kim, Sunghun and Huang, Jiayi},
  journal={IEEE Transactions on Knowledge and Data Engineering}, 
  title={A Survey on Mixture of Experts in Large Language Models}, 
  year={2025},
  volume={37},
  number={7},
  pages={3896-3915},
  keywords={Computational modeling;Transformers;Training;Taxonomy;Natural language processing;Surveys;Logic gates;Large language models;Computer architecture;System analysis and design;Large language models;mixture of experts;gating functions},
  doi={10.1109/TKDE.2025.3554028}}

@inproceedings{carlini2022privacy,
 author = {Carlini, Nicholas and Jagielski, Matthew and Zhang, Chiyuan and Papernot, Nicolas and Terzis, Andreas and Tramer, Florian},
 booktitle = {Advances in Neural Information Processing Systems},
 editor = {S. Koyejo and S. Mohamed and A. Agarwal and D. Belgrave and K. Cho and A. Oh},
 pages = {13263--13276},
 publisher = {Curran Associates, Inc.},
 title = {The Privacy Onion Effect: Memorization is Relative},
 url = {https://proceedings.neurips.cc/paper_files/paper/2022/file/564b5f8289ba846ebc498417e834c253-Paper-Conference.pdf},
 volume = {35},
 year = {2022}
}


@book{charniak1996statistical,
  title={Statistical language learning},
  author={Charniak, Eugene},
  year={1996},
  publisher={MIT press}
}

@inproceedings{chen2022large,
    title = {Large Language Models are few(1)-shot Table Reasoners},
    author = {Chen, Wenhu},
    editor = {Vlachos, Andreas  and
      Augenstein, Isabelle},
    booktitle = {Findings of the Association for Computational Linguistics: EACL 2023},
    month = may,
    year = {2023},
    address = {Dubrovnik, Croatia},
    publisher = {Association for Computational Linguistics},
    url = {https://aclanthology.org/2023.findings-eacl.83/},
    doi = {10.18653/v1/2023.findings-eacl.83},
    pages = {1120--1130}
}

@inproceedings{chen2021recurrent,
  title={Recurrent Neural Networks algorithms and applications},
  author={Chen, Yuexing and Li, Jiarun},
  booktitle={2021 2nd international conference on big data \& artificial intelligence \& software engineering (ICBASE)},
  pages={38--43},
  year={2021},
  organization={IEEE}
}

@inproceedings{chernyshev2024u,
    title = {{U}-{MATH}: A University-Level Benchmark for Evaluating Mathematical Skills in Large Language Models},
    author = {Chernyshev, Konstantin  and
      Polshkov, Vitaliy  and
      Stepanov, Vlad  and
      Myasnikov, Alex  and
      Artemova, Ekaterina  and
      Miasnikov, Alexei  and
      Tilga, Sergei},
    editor = {Arviv, Ofir  and
      Clinciu, Miruna  and
      Dhole, Kaustubh  and
      Dror, Rotem  and
      Gehrmann, Sebastian  and
      Habba, Eliya  and
      Itzhak, Itay  and
      Mille, Simon  and
      Perlitz, Yotam  and
      Santus, Enrico  and
      Sedoc, Jo{\~a}o  and
      Shmueli Scheuer, Michal  and
      Stanovsky, Gabriel  and
      Tafjord, Oyvind},
    booktitle = {Proceedings of the Fourth Workshop on Generation, Evaluation and Metrics (GEM{\texttwosuperior})},
    month = jul,
    year = {2025},
    address = {Vienna, Austria and virtual meeting},
    publisher = {Association for Computational Linguistics},
    url = {https://aclanthology.org/2025.gem-1.77/},
    pages = {974--1001},
    ISBN = {979-8-89176-261-9}
}

@article{aakanksha2023palm,
  author  = {Aakanksha Chowdhery and Sharan Narang and Jacob Devlin and Maarten Bosma and Gaurav Mishra and Adam Roberts and Paul Barham and Hyung Won Chung and Charles Sutton and Sebastian Gehrmann and Parker Schuh and Kensen Shi and Sasha Tsvyashchenko and Joshua Maynez and Abhishek Rao and Parker Barnes and Yi Tay and Noam Shazeer and Vinodkumar Prabhakaran and Emily Reif and Nan Du and Ben Hutchinson and Reiner Pope and James Bradbury and Jacob Austin and Michael Isard and Guy Gur-Ari and Pengcheng Yin and Toju Duke and Anselm Levskaya and Sanjay Ghemawat and Sunipa Dev and Henryk Michalewski and Xavier Garcia and Vedant Misra and Kevin Robinson and Liam Fedus and Denny Zhou and Daphne Ippolito and David Luan and Hyeontaek Lim and Barret Zoph and Alexander Spiridonov and Ryan Sepassi and David Dohan and Shivani Agrawal and Mark Omernick and Andrew M. Dai and Thanumalayan Sankaranarayana Pillai and Marie Pellat and Aitor Lewkowycz and Erica Moreira and Rewon Child and Oleksandr Polozov and Katherine Lee and Zongwei Zhou and Xuezhi Wang and Brennan Saeta and Mark Diaz and Orhan Firat and Michele Catasta and Jason Wei and Kathy Meier-Hellstern and Douglas Eck and Jeff Dean and Slav Petrov and Noah Fiedel},
  title   = {PaLM: Scaling Language Modeling with Pathways},
  journal = {Journal of Machine Learning Research},
  year    = {2023},
  volume  = {24},
  number  = {240},
  pages   = {1--113},
  url     = {http://jmlr.org/papers/v24/22-1144.html}
}

@misc{cobbe2021training,
      title={Training Verifiers to Solve Math Word Problems}, 
      author={Karl Cobbe and Vineet Kosaraju and Mohammad Bavarian and Mark Chen and Heewoo Jun and Lukasz Kaiser and Matthias Plappert and Jerry Tworek and Jacob Hilton and Reiichiro Nakano and Christopher Hesse and John Schulman},
      year={2021},
      eprint={2110.14168},
      archivePrefix={arXiv},
      primaryClass={cs.LG},
      url={https://arxiv.org/abs/2110.14168}, 
}

@article{colin2020exploring,
author = {Raffel, Colin and Shazeer, Noam and Roberts, Adam and Lee, Katherine and Narang, Sharan and Matena, Michael and Zhou, Yanqi and Li, Wei and Liu, Peter J.},
title = {Exploring the limits of transfer learning with a unified text-to-text transformer},
year = {2020},
issue_date = {January 2020},
publisher = {JMLR.org},
volume = {21},
number = {1},
issn = {1532-4435},
journal = {J. Mach. Learn. Res.},
month = {jan},
articleno = {140},
numpages = {67},
keywords = {deep learning, attention based models, multi-task learning, natural language processing, transfer learning}
}


@article{collins2024evaluating,
  title={Evaluating language models for mathematics through interactions},
  author={Collins, Katherine M and Jiang, Albert Q and Frieder, Simon and Wong, Lionel and Zilka, Miri and Bhatt, Umang and Lukasiewicz, Thomas and Wu, Yuhuai and Tenenbaum, Joshua B and Hart, William and others},
  journal={Proceedings of the National Academy of Sciences},
  volume={121},
  number={24},
  pages={e2318124121},
  year={2024},
  publisher={National Academy of Sciences}
}

@article{Dan2024lora,
    author = {Dan Biderman, Jacob Portes, Jose Javier Gonzalez Ortiz, Mansheej Paul, Philip Greengard, Connor Jennings, Daniel King, Sam Havens, Vitaliy Chiley, Jonathan Frankle, Cody Blakeney and John P. Cunningham},
    title = {Lora learns less and forgets less.},
    journal = {Transactions on Machine Learning Research} ,
    year = {2024}
}

@inproceedings{dang2024data,
  title={Data quality in nlp: Metrics and a comprehensive taxonomy},
  author={Dang, Vu Minh Hoang and Verma, Rakesh M},
  booktitle={International Symposium on Intelligent Data Analysis},
  pages={217--229},
  year={2024},
  organization={Springer}
}

@inproceedings{dave2024investigating,
  title   = {Investigating Symbolic Capabilities of Large Language Models},
  author  = {Neisarg Dave, Daniel Kifer, C. Lee Giles, Ankur Mali},
  booktitle = {Proceedings of the First International Workshop on Logical Foundations of Neuro-Symbolic AI (LNSAI 2024)},
  editor  = {Gianluca Cima, Marco Console, Víctor Gutiérrez-Basulto,Pascal Hitzler, Maurizio Lenzerini},
  series  = {CEUR Workshop Proceedings},
  volume  = {3819},
  year    = {2024},
  publisher = {CEUR-WS.org},
  url     = {https://ceur-ws.org/Vol-3819/paper2.pdf}
}

@article{deng2025multi,
  title={Multi-head Temporal Latent Attention},
  author={Deng, Keqi and Woodland, Philip C},
  journal={arXiv preprint arXiv:2505.13544},
  year={2025}
}

@inproceedings{Dettmers2023QLORA,
 author = {Dettmers, Tim and Pagnoni, Artidoro and Holtzman, Ari and Zettlemoyer, Luke},
 booktitle = {Advances in Neural Information Processing Systems},
 editor = {A. Oh and T. Naumann and A. Globerson and K. Saenko and M. Hardt and S. Levine},
 pages = {10088--10115},
 publisher = {Curran Associates, Inc.},
 title = {QLoRA: Efficient Finetuning of Quantized LLMs},
 url = {https://proceedings.neurips.cc/paper_files/paper/2023/file/1feb87871436031bdc0f2beaa62a049b-Paper-Conference.pdf},
 volume = {36},
 year = {2023}
}

@inproceedings{devlin2019bert,
    title = {{BERT}: Pre-training of Deep Bidirectional Transformers for Language Understanding},
    author = {Devlin, Jacob  and
      Chang, Ming-Wei  and
      Lee, Kenton  and
      Toutanova, Kristina},
    editor = {Burstein, Jill  and
      Doran, Christy  and
      Solorio, Thamar},
    booktitle = {Proceedings of the 2019 Conference of the North {A}merican Chapter of the Association for Computational Linguistics: Human Language Technologies, Volume 1 (Long and Short Papers)},
    month = jun,
    year = {2019},
    address = {Minneapolis, Minnesota},
    publisher = {Association for Computational Linguistics},
    url = {https://aclanthology.org/N19-1423/},
    doi = {10.18653/v1/N19-1423},
    pages = {4171--4186}
}

@article{devlin1998language,
  title={The language of mathematics: making the invisible visible},
  author={Devlin, Keith and Gray, Jeremy},
  journal={Nature},
  volume={396},
  number={6710},
  pages={428--428},
  year={1998},
  publisher={[London: Macmillan Journals], 1869-},
  url= {https://www.math.chalmers.se/~ulfp/Review/langmath.pdf}
}

@inproceedings{didolkar2024metacognitive,
 author = {Didolkar, Aniket and Goyal, Anirudh and Ke, Nan Rosemary and Guo, Siyuan and Valko, Michal and Lillicrap, Timothy and Rezende, Danilo and Bengio, Yoshua and Mozer, Michael and Arora, Sanjeev},
 booktitle = {Advances in Neural Information Processing Systems},
 doi = {10.52202/079017-0623},
 editor = {A. Globerson and L. Mackey and D. Belgrave and A. Fan and U. Paquet and J. Tomczak and C. Zhang},
 pages = {19783--19812},
 publisher = {Curran Associates, Inc.},
 title = {Metacognitive Capabilities of LLMs: An Exploration in Mathematical Problem Solving},
 url = {https://proceedings.neurips.cc/paper_files/paper/2024/file/2318d75a06437eaa257737a5cf3ab83c-Paper-Conference.pdf},
 volume = {37},
 year = {2024}
}


@inproceedings{ding2023sora,
  title={Sparse Low-rank Adaptation of Pre-trained Language Models},
  author={Ding, Ning and Lv, Xingtai and Wang, Qiaosen and Chen, Yulin and Zhou, Bowen and Liu, Zhiyuan and Sun, Maosong},
  booktitle={Proceedings of the 2023 Conference on Empirical Methods in Natural Language Processing},
  pages={4134--4148},
  year={2023}
}

@inproceedings{engstrom2019implementation,
  title={Implementation matters in deep rl: A case study on ppo and trpo},
  author={Engstrom, Logan and Ilyas, Andrew and Santurkar, Shibani and Tsipras, Dimitris and Janoos, Firdaus and Rudolph, Larry and Madry, Aleksander},
  booktitle={International conference on learning representations},
  year={2019}
}

@article{fang2025mathodyssey,
  title = {{{MathOdyssey}}: {{Benchmarking Mathematical Problem-Solving Skills}} in {{Large Language Models Using Odyssey Math Data}}},
  author = {Fang, Meng and Wan, Xiangpeng and Lu, Fei and Xing, Fei and Zou, Kai},
  date = {2025-08-08},
  journaltitle = {Scientific Data},
  shortjournal = {Scientific Data},
  publisher = {Nature},
  volume = {12},
  number = {1},
  pages = {1392},
  issn = {2052-4463},
  doi = {10.1038/s41597-025-05283-3},
  url = {https://doi.org/10.1038/s41597-025-05283-3}
}

@book{feigenbaum1963computers,
  editor    = {Feigenbaum, Edward A. and Feldman, Julian},
  title     = {Computers and Thought},
  publisher = {McGraw-Hill},
  address   = {New York},
  year      = {1963},
  pages     = {562},
  url       = {https://archive.org/details/computersthought00feig},
  note      = {Digitized by Internet Archive}
}

@inproceedings{feldman2020does,
author = {Feldman, Vitaly},
title = {Does learning require memorization? a short tale about a long tail},
year = {2020},
isbn = {9781450369794},
publisher = {Association for Computing Machinery},
address = {New York, NY, USA},
url = {https://doi.org/10.1145/3357713.3384290},
doi = {10.1145/3357713.3384290},
booktitle = {Proceedings of the 52nd Annual ACM SIGACT Symposium on Theory of Computing},
pages = {954–959},
numpages = {6},
keywords = {Privacy-preserving Learning, Overfitting, Long-tailed Distribution, Interpolation, Generalization},
location = {Chicago, IL, USA},
series = {STOC 2020}
}

@INPROCEEDINGS{feng2025lora,
  author={Feng, Zeqin and Xie, Yongqiang and Yang, Jiawei and Hou, Wenjun and Li, Zhongbo},
  booktitle={2025 8th International Conference on Advanced Electronic Materials, Computers and Software Engineering (AEMCSE)}, 
  title={A Survey of Low-Rank Adaptation Techniques}, 
  year={2025},
  volume={},
  number={},
  pages={215-224},
  keywords={Surveys;Computers;Technological innovation;Reviews;Large language models;Computer architecture;Transformers;Matrix decomposition;Optimization;Software engineering;Low-Rank Adaptation;Parameter-Efficient Fine-Tuning;Large Language Models},
  doi={10.1109/AEMCSE65292.2025.11042839}}


@misc{forootani2025survey,
      title={A Survey on Mathematical Reasoning and Optimization with Large Language Models}, 
      author={Ali Forootani},
      year={2025},
      eprint={2503.17726},
      archivePrefix={arXiv},
      primaryClass={cs.AI},
      url={https://arxiv.org/abs/2503.17726}, 
}

@phdthesis{fu2025improving,
  title        = {Improving Complex Reasoning in Large Language Models},
  author       = {Fu, Yao},
  year         = {2025},
  school       = {The University of Edinburgh},
  institution  = {School of Informatics},
  type         = {PhD thesis},
  address      = {Edinburgh, United Kingdom},
  doi          = {10.7488/era/6083},
  url          = {https://doi.org/10.7488/era/6083}
}

@misc{fu2025reward,
      title={Reward Shaping to Mitigate Reward Hacking in RLHF}, 
      author={Jiayi Fu and Xuandong Zhao and Chengyuan Yao and Heng Wang and Qi Han and Yanghua Xiao},
      year={2026},
      eprint={2502.18770},
      archivePrefix={arXiv},
      primaryClass={cs.LG},
      url={https://arxiv.org/abs/2502.18770}, 
}

@misc{gao2024omni,
      title={Omni-MATH: A Universal Olympiad Level Mathematic Benchmark For Large Language Models}, 
      author={Bofei Gao and Feifan Song and Zhe Yang and Zefan Cai and Yibo Miao and Qingxiu Dong and Lei Li and Chenghao Ma and Liang Chen and Runxin Xu and Zhengyang Tang and Benyou Wang and Daoguang Zan and Shanghaoran Quan and Ge Zhang and Lei Sha and Yichang Zhang and Xuancheng Ren and Tianyu Liu and Baobao Chang},
      year={2024},
      eprint={2410.07985},
      archivePrefix={arXiv},
      primaryClass={cs.CL},
      url={https://arxiv.org/abs/2410.07985}, 
}

@inproceedings{golkar2023xval,
    title={xVal: A Continuous Number Encoding for Large Language Models},
    author={Siavash Golkar and Mariel Pettee and Michael Eickenberg and Alberto Bietti and Miles Cranmer and Geraud Krawezik and Francois Lanusse and Michael McCabe and Ruben Ohana and Liam Parker and Bruno R{\'e}galdo-Saint Blancard and Tiberiu Tesileanu and Kyunghyun Cho and Shirley Ho},
    booktitle={NeurIPS 2023 AI for Science Workshop},
    year={2023},
    url={https://openreview.net/forum?id=KHDMZtoF4i}
}

@article{gong2023survey,
title = {A survey on dataset quality in machine learning},
journal = {Information and Software Technology},
volume = {162},
pages = {107268},
year = {2023},
issn = {0950-5849},
doi = {https://doi.org/10.1016/j.infsof.2023.107268},
url = {https://www.sciencedirect.com/science/article/pii/S0950584923001222},
author = {Youdi Gong and Guangzhen Liu and Yunzhi Xue and Rui Li and Lingzhong Meng},
keywords = {Dataset, Dataset quality, Machine Learning},
}

@book{gowers2010princeton,
  title={The Princeton companion to mathematics},
  author={Gowers, Timothy and Barrow-Green, June and Leader, Imre},
  year={2010},
  publisher={Princeton University Press}
}

@misc{guan2025rstar,
      title={rStar-Math: Small LLMs Can Master Math Reasoning with Self-Evolved Deep Thinking}, 
      author={Xinyu Guan and Li Lyna Zhang and Yifei Liu and Ning Shang and Youran Sun and Yi Zhu and Fan Yang and Mao Yang},
      year={2025},
      eprint={2501.04519},
      archivePrefix={arXiv},
      primaryClass={cs.CL},
      url={https://arxiv.org/abs/2501.04519}, 
}

@INPROCEEDINGS{guzman2023developing,
  author={Guzmán, Daniel Sánchez and Juárez, Erika Cervantes},
  booktitle={2023 IEEE Frontiers in Education Conference (FIE)}, 
  title={Developing the numeric reasoning and mathematical modeling processes in engineering students using the LSEESC methodology}, 
  year={2023},
  volume={},
  number={},
  pages={1-5},
  keywords={Knowledge engineering;Deep learning;Biotechnology;Kinematics;Industrial engineering;Mathematical models;Cognition;Learning Engineering and Physics;Numeric reasoning;Mathematical modeling;Learning with spreadsheets support;LSEESC Methodology},
  doi={10.1109/FIE58773.2023.10343515}}

@inproceedings{han2024rethinking,
author = {Han, Zhiguang and Wang, Zijian},
title = {Rethinking the Role-play Prompting in Mathematical Reasoning Tasks},
year = {2024},
isbn = {9798400711916},
publisher = {Association for Computing Machinery},
address = {New York, NY, USA},
url = {https://doi.org/10.1145/3688864.3689149},
doi = {10.1145/3688864.3689149},
booktitle = {Proceedings of the 1st Workshop on Efficiency, Security, and Generalization of Multimedia Foundation Models},
pages = {13–17},
numpages = {5},
keywords = {large language models, prompt engineering, reasoning ability, role-play},
location = {Melbourne VIC, Australia},
series = {ESGMFM '24}
}

@inproceedings{he2024olympiadbench,
    title = {{O}lympiad{B}ench: A Challenging Benchmark for Promoting {AGI} with Olympiad-Level Bilingual Multimodal Scientific Problems},
    author = {He, Chaoqun  and
      Luo, Renjie  and
      Bai, Yuzhuo  and
      Hu, Shengding  and
      Thai, Zhen  and
      Shen, Junhao  and
      Hu, Jinyi  and
      Han, Xu  and
      Huang, Yujie  and
      Zhang, Yuxiang  and
      Liu, Jie  and
      Qi, Lei  and
      Liu, Zhiyuan  and
      Sun, Maosong},
    editor = {Ku, Lun-Wei  and
      Martins, Andre  and
      Srikumar, Vivek},
    booktitle = {Proceedings of the 62nd Annual Meeting of the Association for Computational Linguistics (Volume 1: Long Papers)},
    month = aug,
    year = {2024},
    address = {Bangkok, Thailand},
    publisher = {Association for Computational Linguistics},
    url = {https://aclanthology.org/2024.acl-long.211/},
    doi = {10.18653/v1/2024.acl-long.211},
    pages = {3828--3850}
}

@misc{hendrycks2021measuring,
      title={Measuring Mathematical Problem Solving With the MATH Dataset}, 
      author={Dan Hendrycks and Collin Burns and Saurav Kadavath and Akul Arora and Steven Basart and Eric Tang and Dawn Song and Jacob Steinhardt},
      year={2021},
      eprint={2103.03874},
      archivePrefix={arXiv},
      primaryClass={cs.LG},
      url={https://arxiv.org/abs/2103.03874}, 
}

@article{herbert2019challenges,
  title={Challenges in Assessing Mathematical Reasoning.},
  author={Herbert, Sandra},
  journal={Mathematics Education Research Group of Australasia},
  year={2019},
  publisher={ERIC}
}

@article{herbert2021overcoming,
  author  = {Herbert, Sandra},
  title   = {Overcoming Challenges in Assessing Mathematical Reasoning},
  journal = {Australian Journal of Teacher Education},
  volume  = {46},
  number  = {8},
  pages   = {17--30},
  year    = {2021},
  doi     = {10.14221/ajte.2021v46n8.2},
  url     = {https://doi.org/10.14221/ajte.2021v46n8.2}
}

@misc{hernandez2021scaling,
      title={Scaling Laws for Transfer}, 
      author={Danny Hernandez and Jared Kaplan and Tom Henighan and Sam McCandlish},
      year={2021},
      eprint={2102.01293},
      archivePrefix={arXiv},
      primaryClass={cs.LG},
      url={https://arxiv.org/abs/2102.01293}, 
}

@inproceedings{hoffmann2022training,
 author = {Hoffmann, Jordan and Borgeaud, Sebastian and Mensch, Arthur and Buchatskaya, Elena and Cai, Trevor and Rutherford, Eliza and de Las Casas, Diego and Hendricks, Lisa Anne and Welbl, Johannes and Clark, Aidan and Hennigan, Thomas and Noland, Eric and Millican, Katherine and van den Driessche, George and Damoc, Bogdan and Guy, Aurelia and Osindero, Simon and Simonyan, Kar\'{e}n and Elsen, Erich and Vinyals, Oriol and Rae, Jack and Sifre, Laurent},
 booktitle = {Advances in Neural Information Processing Systems},
 editor = {S. Koyejo and S. Mohamed and A. Agarwal and D. Belgrave and K. Cho and A. Oh},
 pages = {30016--30030},
 publisher = {Curran Associates, Inc.},
 title = {An empirical analysis of compute-optimal large language model training},
 url = {https://proceedings.neurips.cc/paper_files/paper/2022/file/c1e2faff6f588870935f114ebe04a3e5-Paper-Conference.pdf},
 volume = {35},
 year = {2022}
}

@inproceedings{hosseini2014learning,
    title = {Learning to Solve Arithmetic Word Problems with Verb Categorization},
    author = {Hosseini, Mohammad Javad  and
      Hajishirzi, Hannaneh  and
      Etzioni, Oren  and
      Kushman, Nate},
    editor = {Moschitti, Alessandro  and
      Pang, Bo  and
      Daelemans, Walter},
    booktitle = {Proceedings of the 2014 Conference on Empirical Methods in Natural Language Processing ({EMNLP})},
    month = oct,
    year = {2014},
    address = {Doha, Qatar},
    publisher = {Association for Computational Linguistics},
    url = {https://aclanthology.org/D14-1058/},
    doi = {10.3115/v1/D14-1058},
    pages = {523--533}
}

@misc{hu2021lora,
      title={LoRA: Low-Rank Adaptation of Large Language Models}, 
      author={Edward J. Hu and Yelong Shen and Phillip Wallis and Zeyuan Allen-Zhu and Yuanzhi Li and Shean Wang and Lu Wang and Weizhu Chen},
      year={2021},
      eprint={2106.09685},
      archivePrefix={arXiv},
      primaryClass={cs.CL},
      url={https://arxiv.org/abs/2106.09685}, 
}

@inproceedings{huang2023towards,
    title = {Towards Reasoning in Large Language Models: A Survey},
    author = {Huang, Jie  and
      Chang, Kevin Chen-Chuan},
    editor = {Rogers, Anna  and
      Boyd-Graber, Jordan  and
      Okazaki, Naoaki},
    booktitle = {Findings of the Association for Computational Linguistics: ACL 2023},
    month = jul,
    year = {2023},
    address = {Toronto, Canada},
    publisher = {Association for Computational Linguistics},
    url = {https://aclanthology.org/2023.findings-acl.67/},
    doi = {10.18653/v1/2023.findings-acl.67},
    pages = {1049--1065}
}

@misc{huang2024o1,
      title={O1 Replication Journey -- Part 2: Surpassing O1-preview through Simple Distillation, Big Progress or Bitter Lesson?}, 
      author={Zhen Huang and Haoyang Zou and Xuefeng Li and Yixiu Liu and Yuxiang Zheng and Ethan Chern and Shijie Xia and Yiwei Qin and Weizhe Yuan and Pengfei Liu},
      year={2024},
      eprint={2411.16489},
      archivePrefix={arXiv},
      primaryClass={cs.CL},
      url={https://arxiv.org/abs/2411.16489}, 
}

@misc{huang2025math,
      title={MATH-Perturb: Benchmarking LLMs' Math Reasoning Abilities against Hard Perturbations}, 
      author={Kaixuan Huang and Jiacheng Guo and Zihao Li and Xiang Ji and Jiawei Ge and Wenzhe Li and Yingqing Guo and Tianle Cai and Hui Yuan and Runzhe Wang and Yue Wu and Ming Yin and Shange Tang and Yangsibo Huang and Chi Jin and Xinyun Chen and Chiyuan Zhang and Mengdi Wang},
      year={2025},
      eprint={2502.06453},
      archivePrefix={arXiv},
      primaryClass={cs.LG},
      url={https://arxiv.org/abs/2502.06453}, 
}

@INPROCEEDINGS{huang2025survey,
  author={Yajun, Huang},
  booktitle={2025 22nd International Computer Conference on Wavelet Active Media Technology and Information Processing (ICCWAMTIP)}, 
  title={A Survey of Complex Reasoning Enhancement Methods for Large Language Models}, 
  year={2025},
  volume={},
  number={},
  pages={1-5},
  keywords={Surveys;Technological innovation;Large language models;Computational modeling;Taxonomy;Reinforcement learning;Cognition;Natural language processing;Robustness;Optimization;Large language models;Reasoning capabilities;Prompting mechanisms;Self-optimization;Process reward models;External tools;Mixture of experts;Reinforcement learning},
  doi={10.1109/ICCWAMTIP68645.2025.11352613}}

  @INPROCEEDINGS{hwang2024exploring,
  author={Hwang, Yechan and Lim, Jinsu and Lee, Young-Jun and Choi, Ho-Jin},
  booktitle={2025 IEEE International Conference on Big Data and Smart Computing (BigComp)}, 
  title={Exploring performance and consistency in mathematical reasoning across problem types}, 
  year={2025},
  volume={},
  number={},
  pages={107-110},
  keywords={Accuracy;Error analysis;Large language models;Big Data;Cognition;mathematical reasoning;large language model;math word problem},
  doi={10.1109/BigComp64353.2025.00031}}


@article{ibrahim2024simple,
  title={Simple and scalable strategies to continually pre-train large language models},
  author={Ibrahim, Adam and Th{\'e}rien, Benjamin and Gupta, Kshitij and Richter, Mats L and Anthony, Quentin and Lesort, Timoth{\'e}e and Belilovsky, Eugene and Rish, Irina},
  journal={arXiv preprint arXiv:2403.08763},
  year={2024}
}

@inproceedings{imani2023mathprompter,
    title = {{M}ath{P}rompter: Mathematical Reasoning using Large Language Models},
    author = {Imani, Shima  and
      Du, Liang  and
      Shrivastava, Harsh},
    editor = {Sitaram, Sunayana  and
      Beigman Klebanov, Beata  and
      Williams, Jason D},
    booktitle = {Proceedings of the 61st Annual Meeting of the Association for Computational Linguistics (Volume 5: Industry Track)},
    month = jul,
    year = {2023},
    address = {Toronto, Canada},
    publisher = {Association for Computational Linguistics},
    url = {https://aclanthology.org/2023.acl-industry.4/},
    doi = {10.18653/v1/2023.acl-industry.4},
    pages = {37--42}
}

@article{ji2023survey,
author = {Ji, Ziwei and Lee, Nayeon and Frieske, Rita and Yu, Tiezheng and Su, Dan and Xu, Yan and Ishii, Etsuko and Bang, Ye Jin and Madotto, Andrea and Fung, Pascale},
title = {Survey of Hallucination in Natural Language Generation},
year = {2023},
issue_date = {December 2023},
publisher = {Association for Computing Machinery},
address = {New York, NY, USA},
volume = {55},
number = {12},
issn = {0360-0300},
url = {https://doi.org/10.1145/3571730},
doi = {10.1145/3571730},
journal = {ACM Comput. Surv.},
month = mar,
articleno = {248},
numpages = {38},
keywords = {consistency in NLG, factuality in NLG, faithfulness in NLG, extrinsic hallucination, intrinsic hallucination, Hallucination}
}

@inproceedings{jiang2022quantile,
  title={Quantile-based policy optimization for reinforcement learning},
  author={Jiang, Jinyang and Peng, Yijie and Hu, Jiaqiao},
  booktitle={2022 Winter Simulation Conference (WSC)},
  pages={2712--2723},
  year={2022},
  organization={IEEE}
}

@article{jozefowicz2016exploring,
  title={Exploring the limits of language modeling},
  author={Jozefowicz, Rafal and Vinyals, Oriol and Schuster, Mike and Shazeer, Noam and Wu, Yonghui},
  journal={arXiv preprint arXiv:1602.02410},
  year={2016}
}

@article{kamali2009improving,
  title={Improving mathematics retrieval},
  author={Kamali, Shahab and Tompa, Frank Wm},
  journal={Towards a Digital Mathematics Library. Grand Bend, Ontario, Canada, July 8-9th, 2009},
  pages={37--48},
  year={2009},
  publisher={Masaryk University Press}
}

@misc{kaplan2020scaling,
      title={Scaling Laws for Neural Language Models}, 
      author={Jared Kaplan and Sam McCandlish and Tom Henighan and Tom B. Brown and Benjamin Chess and Rewon Child and Scott Gray and Alec Radford and Jeffrey Wu and Dario Amodei},
      year={2020},
      eprint={2001.08361},
      archivePrefix={arXiv},
      primaryClass={cs.LG},
      url={https://arxiv.org/abs/2001.08361}, 
}

@article{karra2023impact,
  author    = {Karra, Rachid and Lasfar, Abdelali},
  title     = {Impact of Data Quality on Question Answering System Performances},
  journal   = {Intelligent Automation & Soft Computing},
  publisher = {Intelligent Automation & Soft Computing},
  volume    = {35},
  number    = {1},
  pages     = {335--349},
  year      = {2023},
  doi       = {10.32604/iasc.2023.026695},
  url       = {https://www.techscience.com/iasc/v35n1/48146},
  issn      = {1079-8587}
}

@article{khan2019rnn,
  title={RNN-LSTM-GRU based language transformation},
  author={Khan, Ahmed and Sarfaraz, Aaliya},
  journal={Soft Computing},
  volume={23},
  number={24},
  pages={13007--13024},
  year={2019},
  publisher={Springer}
}

@book{kline1990mathematical,
  author    = {Kline, Morris},
  title     = {Mathematical Thought from Ancient to Modern Times},
  volume    = {3},
  publisher = {Oxford University Press},
  address   = {New York},
  year      = {1990},
  isbn      = {0-19-506137-3},
  note      = {Originally published in 1972; Oxford University Press paperback edition},
  lccn      = {89-25520},
  subjects  = {Mathematics---History},
  url = {https://www.hlevkin.com/hlevkin/90MathPhysBioBooks/mathHistory/KLINE_MathematicalThoughtFromAncientToModernTimes3.pdf}
}

@incollection{knill1997hidden,
  title={Hidden Markov models in speech and language processing},
  author={Knill, K and Young, S},
  booktitle={Corpus-based methods in language and speech processing},
  pages={27--68},
  year={1997},
  publisher={Springer}
}

@inproceedings{koncel2016mawps,
    title = {{MAWPS}: A Math Word Problem Repository},
    author = {Koncel-Kedziorski, Rik  and
      Roy, Subhro  and
      Amini, Aida  and
      Kushman, Nate  and
      Hajishirzi, Hannaneh},
    editor = {Knight, Kevin  and
      Nenkova, Ani  and
      Rambow, Owen},
    booktitle = {Proceedings of the 2016 Conference of the North {A}merican Chapter of the Association for Computational Linguistics: Human Language Technologies},
    month = jun,
    year = {2016},
    address = {San Diego, California},
    publisher = {Association for Computational Linguistics},
    url = {https://aclanthology.org/N16-1136/},
    doi = {10.18653/v1/N16-1136},
    pages = {1152--1157}
}

@article{koroteev2021bert,
  title={BERT: a review of applications in natural language processing and understanding},
  author={Koroteev, Mikhail V},
  journal={arXiv preprint arXiv:2103.11943},
  year={2021}
}

@article{koubaa2023gpt,
  title={GPT-4 vs. GPT-3.5: A concise showdown},
  author={Koubaa, Anis},
  year={2023},
  publisher={Preprints}
}

@inproceedings{kristianto2016mcat,
  title={MCAT Math Retrieval System for NTCIR-12 MathIR Task},
  author={Kristianto, Giovanni Yoko and Topic, Goran and Aizawa, Akiko},
  conference={NTCIR},
  year={2016},
  url= {https://research.nii.ac.jp/ntcir/workshop/OnlineProceedings12/pdf/ntcir/MathIR/04-NTCIR12-MathIR-KristiantoGY.pdf}
}

@article{kumar2025prompt,
author = {Kumar, Sujit and Singh, Monika and Ranjan, Abhishek and Tanveen, Tanveen and Singh, Sanasam Ranbir},
title = {Prompt-based Masked Language Modeling for Numerical Reasoning},
year = {2025},
publisher = {Association for Computing Machinery},
address = {New York, NY, USA},
issn = {2157-6904},
url = {https://doi.org/10.1145/3746455},
doi = {10.1145/3746455},
note = {Just Accepted},
journal = {ACM Trans. Intell. Syst. Technol.},
month = jun,
keywords = {Numeral aware Headline Generation, Numerical Reasoning, Large Language Models, Prompt Tuning, Few Shot Prompting}
}

@inproceedings{lample2019deep,
title={Deep Learning For Symbolic Mathematics},
author={Guillaume Lample and François Charton},
booktitle={International Conference on Learning Representations},
year={2020},
url={https://openreview.net/forum?id=S1eZYeHFDS}
}

@article{lee2022factuality,
  title={Factuality enhanced language models for open-ended text generation},
  author={Lee, Nayeon and Ping, Wei and Xu, Peng and Patwary, Mostofa and Fung, Pascale N and Shoeybi, Mohammad and Catanzaro, Bryan},
  journal={Advances in Neural Information Processing Systems},
  volume={35},
  pages={34586--34599},
  year={2022}
}

@inproceedings{lewkowycz2022solving,
 author = {Lewkowycz, Aitor and Andreassen, Anders and Dohan, David and Dyer, Ethan and Michalewski, Henryk and Ramasesh, Vinay and Slone, Ambrose and Anil, Cem and Schlag, Imanol and Gutman-Solo, Theo and Wu, Yuhuai and Neyshabur, Behnam and Gur-Ari, Guy and Misra, Vedant},
 booktitle = {Advances in Neural Information Processing Systems},
 editor = {S. Koyejo and S. Mohamed and A. Agarwal and D. Belgrave and K. Cho and A. Oh},
 pages = {3843--3857},
 publisher = {Curran Associates, Inc.},
 title = {Solving Quantitative Reasoning Problems with Language Models},
 url = {https://proceedings.neurips.cc/paper_files/paper/2022/file/18abbeef8cfe9203fdf9053c9c4fe191-Paper-Conference.pdf},
 volume = {35},
 year = {2022}
}

@inproceedings{li2025Optimizing,
author = {Li, Cheng and Fei, Xiaoyu and Yang, Xiaoyu},
title = {Optimizing Numerical Reasoning with Pre-trained Language Models: An Enhanced Algorithm},
year = {2025},
isbn = {9798400713163},
publisher = {Association for Computing Machinery},
address = {New York, NY, USA},
url = {https://doi.org/10.1145/3746709.3746759},
doi = {10.1145/3746709.3746759},
booktitle = {Proceedings of the 2025 6th International Conference on Computer Information and Big Data Applications},
pages = {285–295},
numpages = {11},
keywords = {Model optimization, Numerical reasoning, Pre-trained models},
location = {
},
series = {CIBDA '25}
}

@inproceedings{li2023camel,
 author = {Li, Guohao and Hammoud, Hasan and Itani, Hani and Khizbullin, Dmitrii and Ghanem, Bernard},
 booktitle = {Advances in Neural Information Processing Systems},
 editor = {A. Oh and T. Naumann and A. Globerson and K. Saenko and M. Hardt and S. Levine},
 pages = {51991--52008},
 publisher = {Curran Associates, Inc.},
 title = {CAMEL: Communicative Agents for {Mind} Exploration of Large Language Model Society},
 url = {https://proceedings.neurips.cc/paper_files/paper/2023/file/a3621ee907def47c1b952ade25c67698-Paper-Conference.pdf},
 volume = {36},
 year = {2023}
 }

@misc{li2023label,
      title={Label Supervised LLaMA Finetuning}, 
      author={Zongxi Li and Xianming Li and Yuzhang Liu and Haoran Xie and Jing Li and Fu-lee Wang and Qing Li and Xiaoqin Zhong},
      year={2023},
      eprint={2310.01208},
      archivePrefix={arXiv},
      primaryClass={cs.CL},
      url={https://arxiv.org/abs/2310.01208}, 
}

@INPROCEEDINGS{li2024enhancing,
  author={Li, Siyue},
  booktitle={2024 5th International Conference on Big Data & Artificial Intelligence & Software Engineering (ICBASE)}, 
  title={Enhancing Mathematical Problem Solving in Large Language Models through Tool-Integrated Reasoning and Python Code Execution}, 
  year={2024},
  volume={},
  number={},
  pages={165-168},
  keywords={Training;Codes;Large language models;Natural languages;Cognition;Mathematical models;Problem-solving;Python;Synthetic data;Software engineering;Tool-Integrated Reasoning;Large Language Models;Mathematical Problem Solving;Python Code Execution;Fine-Tuning},
  doi={10.1109/ICBASE63199.2024.10762312}}

@inproceedings{li2024vblora,
 author = {Li, Yang and Han, Shaobo and Ji, Shihao},
 booktitle = {Advances in Neural Information Processing Systems},
 editor = {A. Globerson and L. Mackey and D. Belgrave and A. Fan and U. Paquet and J. Tomczak and C. Zhang},
 pages = {16724--16751},
 publisher = {Curran Associates, Inc.},
 title = {VB-LoRA: Extreme Parameter Efficient Fine-Tuning with Vector Banks},
 url = {https://proceedings.neurips.cc/paper_files/paper/2024/file/1e0d38c676d5855bcfab7f6d29d20ad9-Paper-Conference.pdf},
 volume = {37},
 year = {2024}
}

@article{liang2025low,
  title={Low-Rank Adaptation for Scalable Large Language Models: A Comprehensive Survey},
  author={Liang, Chia Xin and Bi, Ziqian and Wang, Tianyang and Liu, Ming and Song, Xinyuan and Zhang, Yichao and Song, Junhao and Niu, Qian and Peng, Benji and Chen, Keyu and others},
  journal={Authorea Preprints},
  year={2025},
  publisher={Authorea}
}

@article{lin2023llm,
  title={Llm-eval: Unified multi-dimensional automatic evaluation for open-domain conversations with large language models},
  author={Lin, Yen-Ting and Chen, Yun-Nung},
  journal={arXiv preprint arXiv:2305.13711},
  year={2023}
}

@article{lindsey2025biology,
  title={On the biology of a large language model (2025)},
  author={Lindsey, Jack and Gurnee, Wes and Ameisen, Emmanuel and Chen, Brian and Pearce, Adam and Turner, Nicholas L and Citro, Craig and Abrahams, David and Carter, Shan and Hosmer, Basil and others},
  journal={Transformer Circuits Thread},
  url={https://transformer-circuits.pub/2025/attribution-graphs/biology.html},
  year={2025}
}

@INPROCEEDINGS{liu2022cognitive,
  author={Liu, Jiayu and Huang, Zhenya and Lin, Xin and Liu, Qi and Ma, Jianhui and Chen, Enhong},
  booktitle={2022 IEEE International Conference on Data Mining (ICDM)}, 
  title={A Cognitive Solver with Autonomously Knowledge Learning for Reasoning Mathematical Answers}, 
  year={2022},
  volume={},
  number={},
  pages={269-278},
  keywords={Commutation;Semantics;Knowledge based systems;Information processing;Cognition;Mathematics;Filtering theory;knowledge learning;mathematical reasoning},
  doi={10.1109/ICDM54844.2022.00037}}

@article{liu2025deepseek,
  title={Deepseek-v3 technical report},
  author={Liu, Aixin and Feng, Bei and Xue, Bing and Wang, Bingxuan and Wu, Bochao and Lu, Chengda and Zhao, Chenggang and Deng, Chengqi and Zhang, Chenyu and Ruan, Chong and others},
  journal={arXiv preprint arXiv:2412.19437},     
  year={2025},
  eprint={2412.19437},
  archivePrefix={arXiv},
  primaryClass={cs.CL},
  url={https://arxiv.org/abs/2412.19437}, 
}

@article{liu2023mathematical,
author = {Liu, Wentao and Hu, Hanglei and Zhou, Jie and Ding, Yuyang and Li, Junsong and Zeng, Jiayi and He, Mengliang and Chen, Qin and Jiang, Bo and Zhou, Aimin and He, Liang},
title = {Mathematical Language Models: A Survey},
year = {2025},
issue_date = {April 2026},
publisher = {Association for Computing Machinery},
address = {New York, NY, USA},
volume = {58},
number = {6},
issn = {0360-0300},
url = {https://doi.org/10.1145/3773985},
doi = {10.1145/3773985},
journal = {ACM Comput. Surv.},
month = dec,
articleno = {146},
numpages = {37}
}

@inproceedings{Liu2023GuidingMath,
author = {Liu, Jiayu and Huang, Zhenya and Ma, Zhiyuan and Liu, Qi and Chen, Enhong and Su, Tianhuang and Liu, Haifeng},
title = {Guiding Mathematical Reasoning via Mastering Commonsense Formula Knowledge},
year = {2023},
isbn = {9798400701030},
publisher = {Association for Computing Machinery},
address = {New York, NY, USA},
url = {https://doi.org/10.1145/3580305.3599375},
doi = {10.1145/3580305.3599375},
booktitle = {Proceedings of the 29th ACM SIGKDD Conference on Knowledge Discovery and Data Mining},
pages = {1477–1488},
numpages = {12},
keywords = {math word problem, knowledge representation and reasoning},
location = {Long Beach, CA, USA},
series = {KDD '23}
}

@INPROCEEDINGS{liu2024rora,
  author={Liu, Jun and Kong, Zhenglun and Dong, Peiyan and Shen, Xuan and Zhao, Pu and Tang, Hao and Yuan, Geng and Niu, Wei and Zhang, Wenbin and Lin, Xue and Huang, Dong and Wang, Yanzhi},
  booktitle={ICASSP 2025 - 2025 IEEE International Conference on Acoustics, Speech and Signal Processing (ICASSP)}, 
  title={RoRA: Efficient Fine-Tuning of LLM with Reliability Optimization for Rank Adaptation}, 
  year={2025},
  volume={},
  number={},
  pages={1-5},
  keywords={Adaptation models;Accuracy;Large language models;Signal processing;Robustness;Matrices;Acoustics;Speech processing;Optimization;Fine-tuning;optimization scaling factor;Large Language Models;pruned models;reliability optimization},
  doi={10.1109/ICASSP49660.2025.10889613}}


@inproceedings{liu2024dora,
  title={DoRA: Weight-Decomposed Low-Rank Adaptation},
  author={Shih-Yang Liu and Chien-Yi Wang and Hongxu Yin and Pavlo Molchanov and Yu-Chiang Frank Wang and Kwang-Ting Cheng and Min-Hung Chen},
  booktitle={International Conference on Machine Learning},
  year={2024},
  url={https://api.semanticscholar.org/CorpusID:267657886}
}


@article{liu2024mora,
  title={MoRA: High-Rank Updating for Parameter-Efficient Fine-Tuning},
  author={Liu, Tingjiang and Yang, Ke and He, Zhenyu and Li, Hongxia and Zhang, Zexi and Lin, Yihao and Kang, Jun and Xu, Chang-Yu and Hou, Wentao and Zhao, Yusheng and others},
  journal={arXiv preprint arXiv:2405.12130},
  year={2024}
}

@inproceedings{liu2024alora,
  title={ALoRA: Allocating Low-Rank Adaptation for Fine-tuning Large Language Models},
  author={Liu, Zequan and Lyn, Jiawen and Zhu, Wei and Tian, Xing and Graham, Yvette},
  booktitle={Proceedings of the 2024 Conference of the North American Chapter of the Association for Computational Linguistics: Human Language Technologies (Volume 1: Long Papers)},
  pages={622--641},
  year={2024}
}

@inproceedings{longpre2021entity,
    title = {Entity-Based Knowledge Conflicts in Question Answering},
    author = {Longpre, Shayne  and
      Perisetla, Kartik  and
      Chen, Anthony  and
      Ramesh, Nikhil  and
      DuBois, Chris  and
      Singh, Sameer},
    editor = {Moens, Marie-Francine  and
      Huang, Xuanjing  and
      Specia, Lucia  and
      Yih, Scott Wen-tau},
    booktitle = {Proceedings of the 2021 Conference on Empirical Methods in Natural Language Processing},
    month = nov,
    year = {2021},
    address = {Online and Punta Cana, Dominican Republic},
    publisher = {Association for Computational Linguistics},
    url = {https://aclanthology.org/2021.emnlp-main.565/},
    doi = {10.18653/v1/2021.emnlp-main.565},
    pages = {7052--7063}
}

@inproceedings{lu2021inter,
    title = {{I}nter-{GPS}: Interpretable Geometry Problem Solving with Formal Language and Symbolic Reasoning},
    author = {Lu, Pan  and
      Gong, Ran  and
      Jiang, Shibiao  and
      Qiu, Liang  and
      Huang, Siyuan  and
      Liang, Xiaodan  and
      Zhu, Song-Chun},
    editor = {Zong, Chengqing  and
      Xia, Fei  and
      Li, Wenjie  and
      Navigli, Roberto},
    booktitle = {Proceedings of the 59th Annual Meeting of the Association for Computational Linguistics and the 11th International Joint Conference on Natural Language Processing (Volume 1: Long Papers)},
    month = aug,
    year = {2021},
    address = {Online},
    publisher = {Association for Computational Linguistics},
    url = {https://aclanthology.org/2021.acl-long.528/},
    doi = {10.18653/v1/2021.acl-long.528},
    pages = {6774--6786}
}

@inproceedings{mansouri2019tangent,
  author    = {Mansouri, Behrooz and Rohatgi, Shaurya and Oard, Douglas W. 
               and Wu, Jian and Giles, C. Lee and Zanibbi, Richard},
  title     = {Tangent-CFT: An Embedding Model for Mathematical Formulas},
  booktitle = {Proceedings of the 2019 ACM SIGIR International Conference on the Theory of Information Retrieval (ICTIR '19)},
  year      = {2019},
  pages     = {11--18},
  address   = {Santa Clara, CA, USA},
  publisher = {Association for Computing Machinery},
  doi       = {10.1145/3341981.3344235},
  isbn      = {978-1-4503-6881-0},
  url       = {https://doi.org/10.1145/3341981.3344235}
}

@article{matzakos2023learning,
  author    = {Matzakos, Nikolaos and Doukakis, Spyridon and Moundridou, Maria},
  title     = {Learning Mathematics with Large Language Models: A Comparative Study with Computer Algebra Systems and Other Tools},
  journal   = {International Journal of Emerging Technologies in Learning (iJET)},
  volume    = {18},
  number    = {20},
  pages     = {51--71},
  month     = {October},
  year      = {2023},
  doi       = {10.3991/ijet.v18i20.42979},
  url       = {https://online-journals.org/index.php/i-jet/article/view/42979}
}

@article{meng2025transmla,
  title={Transmla: Multi-head latent attention is all you need},
  author={Meng, Fanxu and Tang, Pingzhi and Tang, Xiaojuan and Yao, Zengwei and Sun, Xing and Zhang, Muhan},
  journal={arXiv preprint arXiv:2502.07864},
  year={2025}
}

@inproceedings{miao2021diverse,
    title = {A Diverse Corpus for Evaluating and Developing {E}nglish Math Word Problem Solvers},
    author = {Miao, Shen-yun  and
      Liang, Chao-Chun  and
      Su, Keh-Yih},
    editor = {Jurafsky, Dan  and
      Chai, Joyce  and
      Schluter, Natalie  and
      Tetreault, Joel},
    booktitle = {Proceedings of the 58th Annual Meeting of the Association for Computational Linguistics},
    month = {jul},
    year = {2020},
    address = {Online},
    publisher = {Association for Computational Linguistics},
    url = {https://aclanthology.org/2020.acl-main.92/},
    doi = {10.18653/v1/2020.acl-main.92},
    pages = {975--984}
}

@inproceedings{miao2024inform,
 author = {Miao, Yuchun and Zhang, Sen and Ding, Liang and Bao, Rong and Zhang, Lefei and Tao, Dacheng},
 booktitle = {Advances in Neural Information Processing Systems},
 doi = {10.52202/079017-4270},
 editor = {A. Globerson and L. Mackey and D. Belgrave and A. Fan and U. Paquet and J. Tomczak and C. Zhang},
 pages = {134387--134429},
 publisher = {Curran Associates, Inc.},
 title = {InfoRM: Mitigating Reward Hacking in RLHF via Information-Theoretic Reward Modeling},
 url = {https://proceedings.neurips.cc/paper_files/paper/2024/file/f25d75fc760aec0a6174f9f5d9da59b8-Paper-Conference.pdf},
 volume = {37},
 year = {2024}
}


@inproceedings{min2021metaicl,
    title = {{M}eta{ICL}: Learning to Learn In Context},
    author = {Min, Sewon  and
      Lewis, Mike  and
      Zettlemoyer, Luke  and
      Hajishirzi, Hannaneh},
    editor = {Carpuat, Marine  and
      de Marneffe, Marie-Catherine  and
      Meza Ruiz, Ivan Vladimir},
    booktitle = {Proceedings of the 2022 Conference of the North American Chapter of the Association for Computational Linguistics: Human Language Technologies},
    month = jul,
    year = {2022},
    address = {Seattle, United States},
    publisher = {Association for Computational Linguistics},
    url = {https://aclanthology.org/2022.naacl-main.201/},
    doi = {10.18653/v1/2022.naacl-main.201},
    pages = {2791--2809}
}


@inproceedings{mishra2022lila,
    title = {{LILA}: A Unified Benchmark for Mathematical Reasoning},
    author = {Mishra, Swaroop  and
      Finlayson, Matthew  and
      Lu, Pan  and
      Tang, Leonard  and
      Welleck, Sean  and
      Baral, Chitta  and
      Rajpurohit, Tanmay  and
      Tafjord, Oyvind  and
      Sabharwal, Ashish  and
      Clark, Peter  and
      Kalyan, Ashwin},
    editor = {Goldberg, Yoav  and
      Kozareva, Zornitsa  and
      Zhang, Yue},
    booktitle = {Proceedings of the 2022 Conference on Empirical Methods in Natural Language Processing},
    month = dec,
    year = {2022},
    address = {Abu Dhabi, United Arab Emirates},
    publisher = {Association for Computational Linguistics},
    url = {https://aclanthology.org/2022.emnlp-main.392/},
    doi = {10.18653/v1/2022.emnlp-main.392},
    pages = {5807--5832}
}

@inproceedings{mu2024rule,
 author = {Mu, Tong and Helyar, Alec and Heidecke, Johannes and Achiam, Joshua and Vallone, Andrea and Kivlichan, Ian and Lin, Molly and Beutel, Alex and Schulman, John and Weng, Lilian},
 booktitle = {Advances in Neural Information Processing Systems},
 doi = {10.52202/079017-3457},
 editor = {A. Globerson and L. Mackey and D. Belgrave and A. Fan and U. Paquet and J. Tomczak and C. Zhang},
 pages = {108877--108901},
 publisher = {Curran Associates, Inc.},
 title = {Rule Based Rewards for Language Model Safety},
 url = {https://proceedings.neurips.cc/paper_files/paper/2024/file/c4e380fb74dec9da9c7212e834657aa9-Paper-Conference.pdf},
 volume = {37},
 year = {2024}
}

@inproceedings{ouyang2022training,
 author = {Ouyang, Long and Wu, Jeffrey and Jiang, Xu and Almeida, Diogo and Wainwright, Carroll and Mishkin, Pamela and Zhang, Chong and Agarwal, Sandhini and Slama, Katarina and Ray, Alex and Schulman, John and Hilton, Jacob and Kelton, Fraser and Miller, Luke and Simens, Maddie and Askell, Amanda and Welinder, Peter and Christiano, Paul F and Leike, Jan and Lowe, Ryan},
 booktitle = {Advances in Neural Information Processing Systems},
 editor = {S. Koyejo and S. Mohamed and A. Agarwal and D. Belgrave and K. Cho and A. Oh},
 pages = {27730--27744},
 publisher = {Curran Associates, Inc.},
 title = {Training language models to follow instructions with human feedback},
 url = {https://proceedings.neurips.cc/paper_files/paper/2022/file/b1efde53be364a73914f58805a001731-Paper-Conference.pdf},
 volume = {35},
 year = {2022}
}


@INPROCEEDINGS{pal2020brief,
  author={Pal, Constantin-Valentin and Leon, Florin},
  booktitle={2020 24th International Conference on System Theory, Control and Computing (ICSTCC)}, 
  title={Brief Survey of Model-Based Reinforcement Learning Techniques}, 
  year={2020},
  volume={},
  number={},
  pages={92-97},
  keywords={Planning;Uncertainty;Computational modeling;Reinforcement learning;Heuristic algorithms;Predictive models;Task analysis;model-based reinforcement learning;model-free reinforcement learning;dynamics models;model-based planning},
  doi={10.1109/ICSTCC50638.2020.9259716}}

@misc{parnami2022learning,
      title={Learning from Few Examples: A Summary of Approaches to Few-Shot Learning}, 
      author={Archit Parnami and Minwoo Lee},
      year={2022},
      eprint={2203.04291},
      archivePrefix={arXiv},
      primaryClass={cs.LG},
      url={https://arxiv.org/abs/2203.04291}, 
}

@misc{paster2023openwebmath,
      title={OpenWebMath: An Open Dataset of High-Quality Mathematical Web Text}, 
      author={Keiran Paster and Marco Dos Santos and Zhangir Azerbayev and Jimmy Ba},
      year={2023},
      eprint={2310.06786},
      archivePrefix={arXiv},
      primaryClass={cs.AI},
      url={https://arxiv.org/abs/2310.06786}, 
}

@inproceedings{pattaniyil2014combining,
  title={Combining tf-idf text retrieval with an inverted index over symbol pairs in math expressions: The tangent math search engine at ntcir 2014.},
  author={Pattaniyil, Nidhin and Zanibbi, Richard},
  booktitle={NTCIR},
  year={2014}
}

@inproceedings{pauls2011faster,
  title={Faster and smaller n-gram language models},
  author={Pauls, Adam and Klein, Dan},
  booktitle={Proceedings of the 49th annual meeting of the Association for Computational Linguistics: Human Language Technologies},
  pages={258--267},
  year={2011}
}

@misc{peng2023mathbert,
      title={MathBERT: A Pre-Trained Model for Mathematical Formula Understanding}, 
      author={Shuai Peng and Ke Yuan and Liangcai Gao and Zhi Tang},
      year={2021},
      eprint={2105.00377},
      archivePrefix={arXiv},
      primaryClass={cs.CL},
      url={https://arxiv.org/abs/2105.00377}, 
}

@article{pourpanah2022review,
  title={A review of generalized zero-shot learning methods},
  author={Pourpanah, Farhad and Abdar, Moloud and Luo, Yuxuan and Zhou, Xinlei and Wang, Ran and Lim, Chee Peng and Wang, Xi-Zhao and Wu, QM Jonathan},
  journal={IEEE transactions on pattern analysis and machine intelligence},
  volume={45},
  number={4},
  pages={4051--4070},
  year={2022},
  publisher={IEEE}
}

@misc{rae2021scaling,
      title={Scaling Language Models: Methods, Analysis & Insights from Training Gopher}, 
      author={Jack W. Rae and Sebastian Borgeaud and Trevor Cai and Katie Millican and Jordan Hoffmann and Francis Song and John Aslanides and Sarah Henderson and Roman Ring and Susannah Young and Eliza Rutherford and Tom Hennigan and Jacob Menick and Albin Cassirer and Richard Powell and George van den Driessche and Lisa Anne Hendricks and Maribeth Rauh and Po-Sen Huang and Amelia Glaese and Johannes Welbl and Sumanth Dathathri and Saffron Huang and Jonathan Uesato and John Mellor and Irina Higgins and Antonia Creswell and Nat McAleese and Amy Wu and Erich Elsen and Siddhant Jayakumar and Elena Buchatskaya and David Budden and Esme Sutherland and Karen Simonyan and Michela Paganini and Laurent Sifre and Lena Martens and Xiang Lorraine Li and Adhiguna Kuncoro and Aida Nematzadeh and Elena Gribovskaya and Domenic Donato and Angeliki Lazaridou and Arthur Mensch and Jean-Baptiste Lespiau and Maria Tsimpoukelli and Nikolai Grigorev and Doug Fritz and Thibault Sottiaux and Mantas Pajarskas and Toby Pohlen and Zhitao Gong and Daniel Toyama and Cyprien de Masson d'Autume and Yujia Li and Tayfun Terzi and Vladimir Mikulik and Igor Babuschkin and Aidan Clark and Diego de Las Casas and Aurelia Guy and Chris Jones and James Bradbury and Matthew Johnson and Blake Hechtman and Laura Weidinger and Iason Gabriel and William Isaac and Ed Lockhart and Simon Osindero and Laura Rimell and Chris Dyer and Oriol Vinyals and Kareem Ayoub and Jeff Stanway and Lorrayne Bennett and Demis Hassabis and Koray Kavukcuoglu and Geoffrey Irving},
      year={2022},
      eprint={2112.11446},
      archivePrefix={arXiv},
      primaryClass={cs.CL},
      url={https://arxiv.org/abs/2112.11446}, 
}

@misc{rajaraman2024toward,
      title={Toward a Theory of Tokenization in LLMs}, 
      author={Nived Rajaraman and Jiantao Jiao and Kannan Ramchandran},
      year={2025},
      eprint={2404.08335},
      archivePrefix={arXiv},
      primaryClass={cs.CL},
      url={https://arxiv.org/abs/2404.08335}, 
}

@inproceedings{ren2024melora,
  title={MELoRA: Mini-Ensemble Low-Rank Adapters for Parameter-Efficient Fine-Tuning},
  author={Ren, Pengjie and Shi, Chengshun and Wu, Shiguang and Zhang, Mengqi and Ren, Zhaochun and de Rijke, Maarten and Chen, Zhumin and Pei, Jiahuan},
  booktitle={Proceedings of the 62nd Annual Meeting of the Association for Computational Linguistics (Volume 1: Long Papers)},
  pages={3052--3064},
  year={2024}
}

@misc{ren2025multi,
      title={The Multi-Agent Fault Localization System Based on Monte Carlo Tree Search Approach}, 
      author={Rui Ren},
      year={2025},
      eprint={2507.22800},
      archivePrefix={arXiv},
      primaryClass={cs.SE},
      url={https://arxiv.org/abs/2507.22800}, 
}

@inproceedings{renduchintala2024tiedlora,
  title={Tied-LoRA: Enhancing parameter efficiency of LoRA with Weight Tying},
  author={Renduchintala, Adithya and Konuk, Tugrul and Kuchaiev, Oleksii},
  booktitle={Proceedings of the 2024 Conference of the North American Chapter of the Association for Computational Linguistics: Human Language Technologies (Volume 1: Long Papers)},
  pages={8694--8705},
  year={2024}
}

@article{resnik2010evaluation,
  title={Evaluation of NLP systems},
  author={Resnik, Philip and Lin, Jimmy},
  journal={The handbook of computational linguistics and natural language processing},
  pages={271--295},
  year={2010},
  publisher={Wiley Online Library}
}

@article{rhomrasi2025llm,
author = {Rhomrasi, Lamyae and Ahsini, Yusef and Igualde, Arnau and Vinuesa, Ricardo and Hoyas, Sergio and García-Sabater, José and Fullana i Alfonso, Màrius and Conejero, Alberto},
year = {2025},
month = {02},
pages = {104366},
title = {LLM performance on mathematical reasoning in Catalan language},
volume = {25},
journal = {Results in Engineering},
doi = {10.1016/j.rineng.2025.104366}
}

@inproceedings{roy2015solving,
    title = {Solving General Arithmetic Word Problems},
    author = {Roy, Subhro  and
      Roth, Dan},
    editor = {M{\`a}rquez, Llu{\'i}s  and
      Callison-Burch, Chris  and
      Su, Jian},
    booktitle = {Proceedings of the 2015 Conference on Empirical Methods in Natural Language Processing},
    month = sep,
    year = {2015},
    address = {Lisbon, Portugal},
    publisher = {Association for Computational Linguistics},
    url = {https://aclanthology.org/D15-1202/},
    doi = {10.18653/v1/D15-1202},
    pages = {1743--1752}
}

@inproceedings{roy2017unit,
author = {Roy, Subhro and Roth, Dan},
title = {Unit dependency graph and its application to arithmetic word problem solving},
year = {2017},
publisher = {AAAI Press},
booktitle = {Proceedings of the Thirty-First AAAI Conference on Artificial Intelligence},
pages = {3082–3088},
numpages = {7},
location = {San Francisco, California, USA},
series = {AAAI'17},
doi = {10.1609/aaai.v31i1.10959},
url = {https://ojs.aaai.org/index.php/AAAI/article/view/10959/10818}
}

@InProceedings{schulman2015trust,
  title = 	 {Trust Region Policy Optimization},
  author = 	 {Schulman, John and Levine, Sergey and Abbeel, Pieter and Jordan, Michael and Moritz, Philipp},
  booktitle = 	 {Proceedings of the 32nd International Conference on Machine Learning},
  pages = 	 {1889--1897},
  year = 	 {2015},
  editor = 	 {Bach, Francis and Blei, David},
  volume = 	 {37},
  series = 	 {Proceedings of Machine Learning Research},
  address = 	 {Lille, France},
  month = 	 {07--09 Jul},
  publisher =    {PMLR},
  pdf = 	 {http://proceedings.mlr.press/v37/schulman15.pdf},
  url = 	 {https://proceedings.mlr.press/v37/schulman15.html}
}

@inproceedings{shalyt2025llms,
title={Do {LLM}s Understand Calculus? Evaluating Symbolic Math Generalization with {AS}y{MOB}},
author={Michael Shalyt and Rotem Elimelech and Ido Kaminer},
booktitle={AI4X 2025 International Conference},
year={2025},
url={https://openreview.net/forum?id=kdatAr0mcd}
}

@misc{shao2024deepseekmath,
      title={DeepSeekMath: Pushing the Limits of Mathematical Reasoning in Open Language Models}, 
      author={Zhihong Shao and Peiyi Wang and Qihao Zhu and Runxin Xu and Junxiao Song and Xiao Bi and Haowei Zhang and Mingchuan Zhang and Y. K. Li and Y. Wu and Daya Guo},
      year={2024},
      eprint={2402.03300},
      archivePrefix={arXiv},
      primaryClass={cs.CL},
      url={https://arxiv.org/abs/2402.03300}, 
}

@misc{shi2023detecting,
      title={Detecting Pretraining Data from Large Language Models}, 
      author={Weijia Shi and Anirudh Ajith and Mengzhou Xia and Yangsibo Huang and Daogao Liu and Terra Blevins and Danqi Chen and Luke Zettlemoyer},
      year={2024},
      eprint={2310.16789},
      archivePrefix={arXiv},
      primaryClass={cs.CL},
      url={https://arxiv.org/abs/2310.16789}, 
}

@misc{singh2024tokenization,
      title={Tokenization counts: the impact of tokenization on arithmetic in frontier LLMs}, 
      author={Aaditya K. Singh and DJ Strouse},
      year={2024},
      eprint={2402.14903},
      archivePrefix={arXiv},
      primaryClass={cs.CL},
      url={https://arxiv.org/abs/2402.14903}, 
}

@misc{smith2022using,
      title={Using DeepSpeed and Megatron to Train Megatron-Turing NLG 530B, A Large-Scale Generative Language Model}, 
      author={Shaden Smith and Mostofa Patwary and Brandon Norick and Patrick LeGresley and Samyam Rajbhandari and Jared Casper and Zhun Liu and Shrimai Prabhumoye and George Zerveas and Vijay Korthikanti and Elton Zhang and Rewon Child and Reza Yazdani Aminabadi and Julie Bernauer and Xia Song and Mohammad Shoeybi and Yuxiong He and Michael Houston and Saurabh Tiwary and Bryan Catanzaro},
      year={2022},
      eprint={2201.11990},
      archivePrefix={arXiv},
      primaryClass={cs.CL},
      url={https://arxiv.org/abs/2201.11990}, 
}

@phdthesis{stathopoulos2023retrieval, 
title={Retrieval of research-level mathematics via joint modelling of text and types},
url={https://www.repository.cam.ac.uk/handle/1810/347577}, 
DOI={10.17863/CAM.94992}, 
school={Apollo - University of Cambridge Repository}, 
author={Stathopoulos, Yiannos}, year={2022}, 
keywords={information retrieval, machine learning, mathematical information retrieval, mathematical language processing, natural language processing}
}

@article{stone2022survey,
  author    = {Stone, George B. and Talbert, Douglas A. and Eberle, William},
  title     = {A Survey of Scalable Reinforcement Learning},
  journal   = {International Journal of Intelligent Computing Research (IJICR)},
  volume    = {13},
  number    = {1},
  year      = {2022},
  doi       = {10.20533/ijicr.2042.4655.2022.0136},
  url       = {https://infonomics-society.org/wp-content/uploads/A-Survey-of-Scalable-Reinforcement-Learning.pdf},
  publisher = {Infonomics Society},
  address   = {Tennessee, USA},
  note      = {Copyright © 2022, Infonomics Society}
}

@inproceedings{sundermeyer2013comparison,
  title={Comparison of feedforward and recurrent neural network language models},
  author={Sundermeyer, Martin and Oparin, Ilya and Gauvain, J-L and Freiberg, Ben and Schl{\{u}ter, Ralf and Ney, Hermann},
  booktitle={2013 IEEE international conference on acoustics, speech and signal processing},
  pages={8430--8434},
  year={2013},
  organization={IEEE}
}

@inproceedings{sundermeyer2012lstm,
  title={Lstm neural networks for language modeling.},
  author={Sundermeyer, Martin and Schl{\{u}ter, Ralf and Ney, Hermann},
  booktitle={Interspeech},
  volume={2012},
  pages={194--197},
  year={2012}
}

@InProceedings{tang2024mathscale,
  title = 	 {{M}ath{S}cale: Scaling Instruction Tuning for Mathematical Reasoning},
  author =       {Tang, Zhengyang and Zhang, Xingxing and Wang, Benyou and Wei, Furu},
  booktitle = 	 {Proceedings of the 41st International Conference on Machine Learning},
  pages = 	 {47885--47900},
  year = 	 {2024},
  editor = 	 {Salakhutdinov, Ruslan and Kolter, Zico and Heller, Katherine and Weller, Adrian and Oliver, Nuria and Scarlett, Jonathan and Berkenkamp, Felix},
  volume = 	 {235},
  series = 	 {Proceedings of Machine Learning Research},
  month = 	 {21--27 Jul},
  publisher =    {PMLR},
  pdf = 	 {https://raw.githubusercontent.com/mlresearch/v235/main/assets/tang24k/tang24k.pdf},
  url = 	 {https://proceedings.mlr.press/v235/tang24k.html}
}


@INPROCEEDINGS{tavasoli2024analyzing,
  author={Tavasoli, Reza and VarastehNezhad, Arya and Masumi, Mostafa and Taghiyareh, Fattaneh},
  booktitle={2025 29th International Computer Conference, Computer Society of Iran (CSICC)}, 
  title={Analyzing the Mathematical Proficiency of Large Language Models in Computer Science Graduate Admission Tests}, 
  year={2025},
  volume={},
  number={},
  pages={1-5},
  keywords={Training;Computer science;Adaptation models;Technological innovation;Accuracy;Large language models;Computational modeling;Mathematical models;Cognition;Multilingual;Large Language Models;Computer Science Education;Mathematical Reasoning;Graduate Entrance Exams;Generative AI;Large Language Models in Education},
  doi={10.1109/CSICC65765.2025.10967440}}

@article{toprakhistorical,
  title={A Historical Overview of Language Model Development: From Statistical Models to Transformers},
  author={Toprak, Ahmet and Toprak, Feyzanur Sa{\u{g}}lam}
}

@inproceedings{toshniwal2024openmath,
author = {Toshniwal, Shubham and Moshkov, Ivan and Narenthiran, Sean and Gitman, Daria and Jia, Fei and Gitman, Igor},
title = {OpenMathInstruct-1: a 1.8 million math instruction tuning dataset},
year = {2024},
isbn = {9798331314385},
publisher = {Curran Associates Inc.},
address = {Red Hook, NY, USA},
booktitle = {Proceedings of the 38th International Conference on Neural Information Processing Systems},
articleno = {1096},
numpages = {38},
location = {Vancouver, BC, Canada},
series = {NIPS '24}
}

@article{valipour2023dylora,
  title={DyLoRA: Parameter Efficient Tuning of Pre-trained Models using Dynamic Search-Free Low-Rank Adaptation},
  author={Valipour, Mojtaba and Rezagholizadeh, Mehdi and Kviatkovsky, Ivan and Ghodsi, Ali},
  journal={arXiv preprint arXiv:2210.07558},
  year={2023}
}

@article{vaswani2017attention,
  title={Attention is all you need},
  author={Vaswani, Ashish and Shazeer, Noam and Parmar, Niki and Uszkoreit, Jakob and Jones, Llion and Gomez, Aidan N and Kaiser, {\L}ukasz and Polosukhin, Illia},
  journal={Advances in neural information processing systems},
  volume={30},
  year={2017}
}


@article{wang2024trans,
  title={Trans-LoRA: towards data-free Transferable Parameter Efficient Finetuning},
  author={Wang, Runqian and Ghosh, Soumya and Cox, David and Antognini, Diego and Oliva, Aude and Feris, Rogerio and Karlinsky, Leonid},
  journal={Advances in Neural Information Processing Systems},
  volume={37},
  pages={61217--61237},
  year={2024}
}

@inproceedings{wang2025examining,
    title = {Examining False Positives under Inference Scaling for Mathematical Reasoning},
    author = {Wang, Yu  and
      Yang, Nan  and
      Wang, Liang  and
      Wei, Furu  and
      Feng, Fuli},
    editor = {Christodoulopoulos, Christos  and
      Chakraborty, Tanmoy  and
      Rose, Carolyn  and
      Peng, Violet},
    booktitle = {Proceedings of the 2025 Conference on Empirical Methods in Natural Language Processing},
    month = nov,
    year = {2025},
    address = {Suzhou, China},
    publisher = {Association for Computational Linguistics},
    url = {https://aclanthology.org/2025.emnlp-main.632/},
    doi = {10.18653/v1/2025.emnlp-main.632},
    pages = {12501--12520},
    ISBN = {979-8-89176-332-6}
}

@article{wang2020generalizing,
author = {Wang, Yaqing and Yao, Quanming and Kwok, James T. and Ni, Lionel M.},
title = {Generalizing from a Few Examples: A Survey on Few-shot Learning},
year = {2020},
issue_date = {May 2021},
publisher = {Association for Computing Machinery},
address = {New York, NY, USA},
volume = {53},
number = {3},
issn = {0360-0300},
url = {https://doi.org/10.1145/3386252},
doi = {10.1145/3386252},
journal = {ACM Comput. Surv.},
month = jun,
articleno = {63},
numpages = {34},
keywords = {Few-shot learning, low-shot learning, meta-learning, one-shot learning, prior knowledge, small sample learning}
}

@inproceedings{Wang2023MetacognitivePI,
  title={Metacognitive Prompting Improves Understanding in Large Language Models},
  author={Yuqing Wang and Yun Zhao},
  booktitle={North American Chapter of the Association for Computational Linguistics},
  year={2023},
  url={https://api.semanticscholar.org/CorpusID:260775822}
}

@inproceedings{wei2025flexora,
  title={Flexora: Flexible Low-Rank Adaptation for Large Language Models},
  author={Wei, Chenxing and Shu, Yao and He, Ying Tiffany and Yu, Fei},
  booktitle={Proceedings of the 63rd Annual Meeting of the Association for Computational Linguistics (Volume 1: Long Papers)},
  pages={14643--14682},
  year={2025},
  address={Vienna, Austria},
  doi={10.18653/v1/2025.acl-long.713}
}

@inproceedings{wei2022chain,
 author = {Wei, Jason and Wang, Xuezhi and Schuurmans, Dale and Bosma, Maarten and ichter, brian and Xia, Fei and Chi, Ed and Le, Quoc V and Zhou, Denny},
 booktitle = {Advances in Neural Information Processing Systems},
 editor = {S. Koyejo and S. Mohamed and A. Agarwal and D. Belgrave and K. Cho and A. Oh},
 pages = {24824--24837},
 publisher = {Curran Associates, Inc.},
 title = {Chain-of-Thought Prompting Elicits Reasoning in Large Language Models},
 url = {https://proceedings.neurips.cc/paper_files/paper/2022/file/9d5609613524ecf4f15af0f7b31abca4-Paper-Conference.pdf},
 volume = {35},
 year = {2022}
}

@misc{wei2023skywork,
      title={Skywork: A More Open Bilingual Foundation Model}, 
      author={Tianwen Wei and Liang Zhao and Lichang Zhang and Bo Zhu and Lijie Wang and Haihua Yang and Biye Li and Cheng Cheng and Weiwei Lü and Rui Hu and Chenxia Li and Liu Yang and Xilin Luo and Xuejie Wu and Lunan Liu and Wenjun Cheng and Peng Cheng and Jianhao Zhang and Xiaoyu Zhang and Lei Lin and Xiaokun Wang and Yutuan Ma and Chuanhai Dong and Yanqi Sun and Yifu Chen and Yongyi Peng and Xiaojuan Liang and Shuicheng Yan and Han Fang and Yahui Zhou},
      year={2023},
      eprint={2310.19341},
      archivePrefix={arXiv},
      primaryClass={cs.CL},
      url={https://arxiv.org/abs/2310.19341}, 
}

@article{welsby2023chatgpt,
    author = {Welsby, Philip and Cheung, Bernard M Y},
    title = {ChatGPT},
    journal = {Postgraduate Medical Journal},
    volume = {99},
    number = {1176},
    pages = {1047-1048},
    year = {2023},
    month = {07},
    issn = {0032-5473},
    doi = {10.1093/postmj/qgad056},
    url = {https://doi.org/10.1093/postmj/qgad056}
}

@article{wu2023pairwise,
  title={Pairwise proximal policy optimization: Harnessing relative feedback for llm alignment},
  author={Wu, Tianhao and Zhu, Banghua and Zhang, Ruoyu and Wen, Zhaojin and Ramchandran, Kannan and Jiao, Jiantao},
  journal={arXiv preprint arXiv:2310.00212},
  year={2023}
}

@Article{wu2025llm,
AUTHOR = {Wu, Xiao-Kun and Chen, Min and Li, Wanyi and Wang, Rui and Lu, Limeng and Liu, Jia and Hwang, Kai and Hao, Yixue and Pan, Yanru and Meng, Qingguo and Huang, Kaibin and Hu, Long and Guizani, Mohsen and Chao, Naipeng and Fortino, Giancarlo and Lin, Fei and Tian, Yonglin and Niyato, Dusit and Wang, Fei-Yue},
TITLE = {LLM Fine-Tuning: Concepts, Opportunities, and Challenges},
JOURNAL = {Big Data and Cognitive Computing},
VOLUME = {9},
YEAR = {2025},
NUMBER = {4},
ARTICLE-NUMBER = {87},
URL = {https://www.mdpi.com/2504-2289/9/4/87},
ISSN = {2504-2289},
DOI = {10.3390/bdcc9040087}
}

@INPROCEEDINGS {xian2017zero,
author = { Xian, Yongqin and Schiele, Bernt and Akata, Zeynep },
booktitle = { 2017 IEEE Conference on Computer Vision and Pattern Recognition (CVPR) },
title = {{ Zero-Shot Learning — The Good, the Bad and the Ugly }},
year = {2017},
volume = {},
ISSN = {1063-6919},
pages = {3077-3086},
keywords = {Training;Protocols;Learning systems;Semantics;Benchmark testing;Feature extraction},
doi = {10.1109/CVPR.2017.328},
url = {https://doi.ieeecomputersociety.org/10.1109/CVPR.2017.328},
publisher = {IEEE Computer Society},
address = {Los Alamitos, CA, USA},
month ={Jul}
}

@article{xiao2024cora,
  title={CoRA: Optimizing Low-Rank Adaptation with Common Subspace of Large Language Models},
  author={Xiao, Xiaojun and Wang, Wenbin and Guo, Zhengzi and Luo, Hangneng and Chen, Bo and Liu, Pengjun and Li, Yong and Liu, Chengyi and Liu, Xiusong},
  journal={arXiv preprint arXiv:2409.02119},
  year={2024}
}

@inproceedings{xin2024advancing,
title={Advancing Theorem Proving in {LLM}s through Large-Scale Synthetic Data},
author={Huajian Xin and Daya Guo and Zhihong Shao and Z.Z. Ren and Qihao Zhu and Bo Liu and Chong Ruan and Wenda Li and Xiaodan Liang},
booktitle={The 4th Workshop on Mathematical Reasoning and AI at NeurIPS'24},
year={2024},
url={https://openreview.net/forum?id=TPtXLihkny}
}

@article{xu2025reasoning,
  title={Reasoning based on symbolic and parametric knowledge bases: a survey},
  author={Xu, Mayi and Ning, Yunfeng and Li, Yongqi and Chen, Jianhao and Wen, Jintao and Xiao, Yao and Zhou, Shen and Pan, Birong and Bao, Zepeng and Miao, Xin and others},
  journal={arXiv preprint arXiv:2501.01030},
  year={2025}
}

@article{yenduri2024gpt,
  title={Gpt (generative pre-trained transformer)—A comprehensive review on enabling technologies, potential applications, emerging challenges, and future directions},
  author={Yenduri, Gokul and Ramalingam, Muthukumaran and Selvi, G Chemmalar and Supriya, Y and Srivastava, Gautam and Maddikunta, Praveen Kumar Reddy and Raj, G Deepti and Jhaveri, Rutvij H and Prabadevi, B and Wang, Weizheng and others},
  journal={IEEE access},
  volume={12},
  pages={54608--54649},
  year={2024},
  publisher={IEEE}
}

@inproceedings{yoko2014mcat,
  title={The mcat math retrieval system for ntcir-11 math track.},
  author={Yoko, Kristianto Giovanni and Florence, Ho and Akiko, Aizawa and others},
  booktitle = {Proceedings of the 11th NTCIR Conference},
  year={2014},
  month = {12},
  url = {https://research.nii.ac.jp/ntcir/workshop/OnlineProceedings11/pdf/NTCIR/Math-2/06-NTCIR11-MATH-KristiantoGY.pdf}
}


@article{yu2024natural,
  title={Natural language reasoning, a survey},
  author={Yu, Fei and Zhang, Hongbo and Tiwari, Prayag and Wang, Benyou},
  journal={ACM Computing Surveys},
  volume={56},
  number={12},
  pages={1--39},
  year={2024},
  publisher={ACM New York, NY}
}

@misc{yuan2023well,
      title={How well do Large Language Models perform in Arithmetic tasks?}, 
      author={Zheng Yuan and Hongyi Yuan and Chuanqi Tan and Wei Wang and Songfang Huang},
      year={2023},
      eprint={2304.02015},
      archivePrefix={arXiv},
      primaryClass={cs.CL},
      url={https://arxiv.org/abs/2304.02015}, 
}

@article{zanibbi2012recognition,
author = {Zanibbi, Richard and Blostein, Dorothea and Zanibbi, R and Blostein, D},
year = {2011},
month = {12},
pages = {331--357},
title = {Recognition and Retrieval of Mathematical Expressions},
volume = {15},
journal = {International Journal on Document Analysis and Recognition (IJDAR)},
doi = {10.1007/s10032-011-0174-4}
}

@inproceedings{zhang2024scalable,
 author = {Zhang, Lijun and Li, Lin and Wei, Wei and Song, Huizhong and Yang, Yaodong and Liang, Jiye},
 booktitle = {Advances in Neural Information Processing Systems},
 doi = {10.52202/079017-4400},
 editor = {A. Globerson and L. Mackey and D. Belgrave and A. Fan and U. Paquet and J. Tomczak and C. Zhang},
 pages = {138698--138730},
 publisher = {Curran Associates, Inc.},
 title = {Scalable Constrained Policy Optimization for Safe Multi-agent Reinforcement Learning},
 url = {https://proceedings.neurips.cc/paper_files/paper/2024/file/fa76985f05e0a25c66528308dda33de0-Paper-Conference.pdf},
 volume = {37},
 year = {2024}
}


@misc{zhang2025formalizing,
  title={Formalizing Complex Mathematical Statements with LLMs: A Study on Mathematical Definitions},
  author={Zhang, Lan and Valentino, Marco and Freitas, Andre},
  year={2025},
  archivePrefix={arXiv},
  primaryClass={cs.CL},
  url={https://arxiv.org/abs/2502.12065v1}, 
}

@article{zhang2023lora,
  title={Lora-fa: Memory-efficient low-rank adaptation for large language models fine-tuning},
  author={Zhang, Longteng and Zhang, Lin and Shi, Shaohuai and Chu, Xiaowen and Li, Bo},
  journal={arXiv preprint arXiv:2308.03303},
  year={2023}
}

@misc{zhang2024fuse,
      title={Fuse, Reason and Verify: Geometry Problem Solving with Parsed Clauses from Diagram}, 
      author={Ming-Liang Zhang and Zhong-Zhi Li and Fei Yin and Liang Lin and Cheng-Lin Liu},
      year={2024},
      eprint={2407.07327},
      archivePrefix={arXiv},
      primaryClass={cs.AI},
      url={https://arxiv.org/abs/2407.07327}, 
}

@inproceedings{zhang2023adalora,
  title={Adaptive Budget Allocation for Parameter-Efficient Fine-Tuning},
  author={Zhang, Qingru and Chen, Minshuo and Bukharin, Alexander and He, Pengcheng and Cheng, Yu and Chen, Weizhu and Zhao, Tuo},
  booktitle={International Conference on Learning Representations},
  year={2023},
  url={https://openreview.net/forum?id=lq62uWRJjiY}
}

@article{zhang2023cumulative,
title={Cumulative Reasoning with Large Language Models},
author={Yifan Zhang and Jingqin Yang and Yang Yuan and Andrew C Yao},
journal={Transactions on Machine Learning Research},
issn={2835-8856},
year={2025},
url={https://openreview.net/forum?id=grW15p4eq2}
}

@inproceedings{zheng2021minif2f,
title={miniF2F: a cross-system benchmark for formal Olympiad-level mathematics},
author={Kunhao Zheng and Jesse Michael Han and Stanislas Polu},
booktitle={International Conference on Learning Representations},
year={2022},
url={https://openreview.net/forum?id=9ZPegFuFTFv}
}

@article{zhuang2025meta,
  title={Meta-rater: A Multi-dimensional Data Selection Method for Pre-training Language Models},
  author={Zhuang, Xinlin and Peng, Jiahui and Ma, Ren and Wang, Yinfan and Bai, Tianyi and Wei, Xingjian and Qiu, Jiantao and Zhang, Chi and Qian, Ying and He, Conghui},
  journal={arXiv preprint arXiv:2504.14194},
  year={2025}
}

@misc{ziegler2019fine,
      title={Fine-Tuning Language Models from Human Preferences}, 
      author={Ziegler, Daniel M and Stiennon, Nisan and Wu, Jeffrey and Brown, Tom B and Radford, Alec and Amodei, Dario and Christiano, Paul and Irving, Geoffrey},
      year={2020},
      eprint={1909.08593},
      archivePrefix={arXiv},
      primaryClass={cs.CL},
      url={https://arxiv.org/abs/1909.08593}, 
}

@article{zi2023deltalora,
  title={Delta-LoRA: Fine-Tuning High-Rank Parameters with the Delta of Low-Rank Matrices},
  author={Zigia, Bojia and Chen, Xianjing and Ma, Dong and Jiang, Shutao and Xiao, Qiang and Wang, Yitao},
  journal={arXiv preprint arXiv:2309.02411},
  year={2023}
}

@article{zoph2022st,
  title={St-moe: Designing stable and transferable sparse expert models},
  author={Zoph, Barret and Bello, Irwan and Kumar, Sameer and Du, Nan and Huang, Yanping and Dean, Jeff and Shazeer, Noam and Fedus, William},
  journal={arXiv preprint arXiv:2202.08906},
  year={2022}
}

@inproceedings{zouhar2023formal,
    title = {A Formal Perspective on Byte-Pair Encoding},
    author = {Zouhar, Vil{\'e}m  and
      Meister, Clara  and
      Gastaldi, Juan  and
      Du, Li  and
      Vieira, Tim  and
      Sachan, Mrinmaya  and
      Cotterell, Ryan},
    editor = {Rogers, Anna  and
      Boyd-Graber, Jordan  and
      Okazaki, Naoaki},
    booktitle = {Findings of the Association for Computational Linguistics: ACL 2023},
    year = {2023},
    url = {https://aclanthology.org/2023.findings-acl.38/},
    doi = {10.18653/v1/2023.findings-acl.38},
    pages = {598--614},
}

%%%%%%%----------ENDs HERE----------%%%%%%%
%%%%%%%----------ENDs HERE----------%%%%%%%
%%%%%%%----------ENDs HERE----------%%%%%%%
%%%%%%%----------ENDs HERE----------%%%%%%%
%%%%%%%----------ENDs HERE----------%%%%%%%
%%%%%%%----------ENDs HERE----------%%%%%%%
%%%%%%%----------ENDs HERE----------%%%%%%%
%%%%%%%----------ENDs HERE----------%%%%%%%
%%%%%%%----------ENDs HERE----------%%%%%%%
%%%%%%%----------ENDs HERE----------%%%%%%%
%%%%%%%----------ENDs HERE----------%%%%%%%
%%%%%%%----------ENDs HERE----------%%%%%%%
%%%%%%%----------ENDs HERE----------%%%%%%%
%%%%%%%----------ENDs HERE----------%%%%%%%
%%%%%%%----------ENDs HERE----------%%%%%%%
%%%%%%%----------ENDs HERE----------%%%%%%%
%%%%%%%----------ENDs HERE----------%%%%%%%
%%%%%%%----------ENDs HERE----------%%%%%%%
%%%%%%%----------ENDs HERE----------%%%%%%%
%%%%%%%----------ENDs HERE----------%%%%%%%
%%%%%%%----------ENDs HERE----------%%%%%%%
%%%%%%%----------ENDs HERE----------%%%%%%%
%%%%%%%----------ENDs HERE----------%%%%%%%
%%%%%%%----------ENDs HERE----------%%%%%%%
%%%%%%%----------ENDs HERE----------%%%%%%%
%%%%%%%----------ENDs HERE----------%%%%%%%
%%%%%%%----------ENDs HERE----------%%%%%%%
%%%%%%%----------ENDs HERE----------%%%%%%%
%%%%%%%----------ENDs HERE----------%%%%%%%
%%%%%%%----------ENDs HERE----------%%%%%%%
%%%%%%%----------ENDs HERE----------%%%%%%%
%%%%%%%----------ENDs HERE----------%%%%%%%
%%%%%%%----------ENDs HERE----------%%%%%%%
%%%%%%%----------ENDs HERE----------%%%%%%%
%%%%%%%----------ENDs HERE----------%%%%%%%
%%%%%%%----------ENDs HERE----------%%%%%%%
%%%%%%%----------ENDs HERE----------%%%%%%%
%%%%%%%----------ENDs HERE----------%%%%%%%
%%%%%%%----------ENDs HERE----------%%%%%%%
%%%%%%%----------ENDs HERE----------%%%%%%%
%%%%%%%----------ENDs HERE----------%%%%%%%
%%%%%%%----------ENDs HERE----------%%%%%%%
%%%%%%%----------ENDs HERE----------%%%%%%%
%%%%%%%----------ENDs HERE----------%%%%%%%
%%%%%%%----------ENDs HERE----------%%%%%%%



==> secs/extra.tex <==
%Mathematics is the science of number, quantity and space, classified as pure or applied  \citep{devlin1998language}. This is a foundation for all core knowledge with extensive history as a tool for trade, astronomy, and record keeping  \citep{kline1990mathematical}. The evolution of mathematics has given rise to modern mathematics which comprises about 26 branches  \citep{gowers2010princeton}. Mathematics relies on structured reasoning to infer meaningful conclusions from this existing knowledge for addressing complex real-world tasks  \citep{huang2023towards}. For this purpose, reasoning helps in various tasks in different domains, such as clinical diagnosis, basic education, financial analysis, and problem solving  \citep{xu2025reasoning}. However, mathematical reasoning ability is different from arithmetic ability demanding in-depth understanding  \citep{yuan2023well}.
Mathematics formalizes reasoning about number, structure, space, and change through precise symbolic systems \citep{devlin1998language,kline1990mathematical}. Beyond arithmetic computation, it requires compositional abstraction, multi-step deduction, and manipulation of formal constraints across interconnected concepts \citep{huang2023towards}. Mathematical reasoning therefore differs fundamentally from surface-level numerical pattern recognition: it demands structured inference, variable binding, proof construction, and long-horizon dependency tracking \citep{yuan2023well}. These properties make mathematics a rigorous testbed for evaluating the reasoning capacity of LLMs.

Recent LLMs achieve strong performance across diverse natural language tasks through large-scale pretraining \citep{wei2022chain,matzakos2023learning}. Prompting strategies such as Chain-of-Thought (CoT) \citep{wei2022chain} and Tool-Integrated Reasoning (TIR) \citep{li2024enhancing} further improve multi-step problem solving, enabling progress in algebraic manipulation, theorem proving, and structured word problems \citep{imani2023mathprompter}. However, solving mathematics remains a long-standing challenge in AI \citep{feigenbaum1963computers,hosseini2014learning}. Despite scaling, LLMs exhibit brittle generalization, arithmetic inconsistencies, symbolic reasoning failures, and error accumulation across long reasoning chains \citep{hendrycks2021measuring,rae2021scaling,lewkowycz2022solving,chernyshev2024u}. Performance declines substantially on competition-level and university-level problems requiring abstraction, formal rigor, and non-standard solution strategies.
%LLMs  are an unprecedented advancement in artificial intelligence (AI) in recent times  \citep{wei2022chain}. They have demonstrated remarkable capabilities by learning from large-scale textual corpora, thereby acquiring general linguistic and numerical reasoning skills  \citep{matzakos2023learning}. Advance methods such as CoT  \citep{wei2022chain} and TIR  \citep{li2024enhancing} have also significantly improved mathematical reasoning capabilities, including theorem proving, algebraic manipulation, and structured numerical problem-solving  \citep{imani2023mathprompter}.However a long-standing AI challenge is to design algorithms to automatically solve math and science problems  \citep{feigenbaum1963computers, hosseini2014learning}.LLMs often struggle in performing complex tasks  \citep{hendrycks2021measuring,wei2022chain}. These such tasks includes arithmetic, commonsense, and symbolic reasoning  \citep{rae2021scaling}. Even state-of-the-art models generally struggle with tasks that require quantitative reasoning, such as solving mathematics, science, and engineering problems at the college-level and university-level  \citep{lewkowycz2022solving, chernyshev2024u}.
%These challenges arise at multiple levels. The dataset and benchmark limitations restrict the scope of evaluation  \citep{mishra2022lila, chernyshev2024u, huang2025math, guan2025rstar}. Meanwhile, training and modeling techniques struggle with discontinuous learning, robust generalization datasets, grade levels, types of math problems  \citep{ahn2024large} and shallow memorization  \citep{huang2025math}. Reasoning abilities of LLMs are showing significant progress with meta-cognitive prompting \citep{Wang2023MetacognitivePI}, however it is also worth noting that model reasoning itself remains constrained by limited meta-cognitive abilities  \citep{didolkar2024metacognitive} being inconsistent with the techniques predicted and utilized. Together, these gaps highlight the need for systematic advances in both datasets and model design to enable robust mathematical reasoning with LLMs.

These limitations arise from multiple sources. First, many benchmarks emphasize final-answer accuracy, exhibit distributional biases, or risk contamination from pretraining corpora, limiting their ability to measure genuine reasoning generalization \citep{mishra2022lila,huang2025math,guan2025rstar}. Second, next-token prediction objectives promote local coherence rather than globally valid derivations, encouraging shortcut learning and shallow memorization \citep{ahn2024large}. Third, although meta-cognitive prompting and self-reflection strategies improve solution quality \citep{Wang2023MetacognitivePI}, the faithfulness and verifiability of generated reasoning traces remain uncertain \citep{didolkar2024metacognitive}. Generated explanations may not reflect internal inference processes, raising concerns about reliability and interpretability.

Given this rapidly evolving landscape, a structured and comprehensive synthesis is necessary. Prior surveys often examine isolated aspects—natural language reasoning, symbolic reasoning, hallucination mitigation, or training optimization \citep{yu2024natural,forootani2025survey,xu2025reasoning,liang2025low}. This fragmented treatment obscures the interaction between benchmarks, architectures, training regimes, and evaluation protocols. Mathematical reasoning performance emerges from the joint effect of these components rather than any single dimension.
%Given this rapidly evolving and complex landscape, a systematic synthesis of existing knowledge is crucial. While several prior surveys have examined aspects of mathematical reasoning in LLMs, they often focus on specific, isolated dimensions such as natural language reasoning, mathematical reasoning, hallucination mitigation, symbolic and parametric reasoning and scaling and optimization for training  \citep{yu2024natural, forootani2025survey, xu2025reasoning, liang2025low}. This partial coverage leaves a significant gap in understanding the interconnected nature of the challenges.
\subimport{img/}{fig_1}
%This survey addresses this gap by providing an extensive and systematic overview of the entire mathematical reasoning problem landscape for LLMs. We examine the full lifecycle of model development, beginning with a critical review of the core datasets used for benchmarking, from foundational vocabulary  \citep{paster2023openwebmath, zhang2025formalizing} and grade-school problems to competition-level  \citep{koncel2016mawps, miao2021diverse, cobbe2021training, li2023camel, yuan2023well, hendrycks2021measuring, he2024olympiadbench, gao2024omni, fang2025mathodyssey, lewkowycz2022solving, chernyshev2024u, mishra2022lila, huang2025math} and formal proofs  \citep{zheng2021minif2f, lu2021inter, azerbayev2023proofnet, zhang2024fuse} (Section \ref{sec4}). We then analyze the evolution of model architectures (Section \ref{sec5}) and the training strategies designed to enhance problem-solving, including pre-training  \citep{devlin2019bert}, supervised fine-tuning  \citep{li2023label}, and reinforcement learning  \citep{stone2022survey} (Section \ref{sec6}). Finally, we detail the evaluation methods and metrics used to assess performance (Section \ref{sec7}).

This survey provides a structured and reproducible analysis of mathematical reasoning in LLMs across the full development lifecycle. We begin by critically examining benchmark datasets, spanning foundational vocabulary \citep{paster2023openwebmath,zhang2025formalizing}, grade-school and competition-level problems \citep{koncel2016mawps,miao2021diverse,cobbe2021training,li2023camel,yuan2023well,hendrycks2021measuring,he2024olympiadbench,gao2024omni,fang2025mathodyssey,lewkowycz2022solving,chernyshev2024u,mishra2022lila,huang2025math}, and formal proof corpora \citep{zheng2021minif2f,lu2021inter,azerbayev2023proofnet,zhang2024fuse} (Section \ref{sec4}). We then analyze architectural adaptations (Section \ref{sec5}) and training strategies—including pretraining \citep{devlin2019bert}, supervised fine-tuning \citep{li2023label}, and reinforcement learning \citep{stone2022survey}—designed to improve reasoning robustness and fidelity (Section \ref{sec6}). Finally, we examine evaluation protocols and metrics, emphasizing the gap between answer-level correctness and step-level reasoning verification (Section \ref{sec7}).


\section*{Research Questions}
To systematically investigate this area, we organize the survey around five Research Questions (RQs):
\begin{itemize}[noitemsep, topsep=0pt]
    \item \textbf{RQ1:} What datasets and benchmarks are used to evaluate mathematical reasoning in LLMs, particularly for competition-level and Olympiad-style problems?
    \item \textbf{RQ2:} Which architectural and training strategies most effectively enhance mathematical reasoning?
    \item \textbf{RQ3:} How do LLMs model multi-step reasoning, and how faithful and verifiable are their reasoning traces?
    \item \textbf{RQ4:} How is performance evaluated, and what limitations affect current evaluation protocols?
    \item \textbf{RQ5:} What fundamental challenges and open research directions remain for competition-level mathematical reasoning?
\end{itemize}

\section*{Contributions}
We summarize our contributions as following. 
\begin{itemize}[noitemsep, topsep=0pt]
    \item We provide a unified taxonomy of mathematical reasoning benchmarks and analyze their scope, difficulty, and structural limitations.
    \item We synthesize architectural and training advances, highlighting how design choices interact with reasoning depth, robustness, and generalization.
    \item We critically examine evaluation methodologies, identifying the disconnect between surface-level accuracy and formally verifiable reasoning.
    \item We articulate open challenges and research directions emerging from the interaction of datasets, modeling paradigms, and evaluation practices.
\end{itemize}

\section*{Paper Organization}
The remainder of the paper is organized as follows. Section \ref{sec2} describes the structured literature review methodology. Section \ref{sec3} presents background on mathematical reasoning in LLMs. Sections \ref{sec4}–\ref{sec7} analyze datasets, architectures, training strategies, and evaluation protocols, respectively. Section \ref{sec8} synthesizes open challenges and future directions. Section 9 concludes the survey.

\begin{comment}
The rapid advancement of mathematical reasoning in LLMs is closely tied to the increasing availability of curated mathematical datasets. However, dataset quality, structural diversity, and reasoning depth critically influence model capabilities. High-quality mathematical datasets must capture diverse problem formulations, span multiple levels of cognitive difficulty, and ideally provide structured reasoning traces that enable models to learn intermediate inference steps \citep{gong2023survey, karra2023impact}.

Importantly, mathematical datasets differ along several orthogonal design dimensions, including problem difficulty, supervision format (answer-only vs. reasoning traces), symbolic representation, and evaluation protocols. Consequently, modern evaluation of mathematical reasoning systems requires a multidimensional analysis of available benchmarks rather than treating all mathematical data as homogeneous natural language text.

This section categorizes existing datasets along three key axes: (i) cognitive complexity and domain depth, (ii) semantic and structural representation, and (iii) computational processing mechanisms such as tokenization and symbolic retrieval. We further highlight systemic limitations that currently hinder robust mathematical reasoning in LLMs.
\end{comment}

\begin{comment}
\subsection{Cognitive Complexity and Domain Scope}\label{sec4.1}
Mathematical corpora used in large language model research span a wide spectrum of cognitive difficulty and domain specialization, ranging from elementary arithmetic reasoning to advanced formal theorem proving. This variation reflects the hierarchical nature of mathematical knowledge, where problem solving progresses from basic numerical manipulation to abstract symbolic reasoning and proof construction. Table~\ref{tab:tbl5} organizes representative training datasets and evaluation benchmarks according to their functional role and reasoning complexity.

\subsubsection{Datasets (Pretraining and Fine-Tuning)}
Datasets aim to expose the LLMs to large volume of mathematical content and structured reasoning example, as detailed in Table~\ref{tab:tbl6}. Foundational datasets such as OpenWebMath \citep{paster2023openwebmath} and Proof-Pile \citep{azerbayev2023proofnet} provide large-scale collections of mathematical texts drawn from web sources, research papers, and formal proof repositories. These resources are primarily used for domain-adaptive pretraining, enabling models to learn mathematical notation, symbolic structures, and general reasoning patterns. Programmatically generated datasets such as AMPS \citep{hendrycks2021measuring} further expand this training paradigm by producing large numbers of automatically generated problems that emphasize arithmetic rules and intermediate reasoning steps.


% ============================ Table 6 =================================

\begin{table*}[t]
\centering
\caption{Taxonomy of mathematical reasoning datasets utilized strictly for pretraining, supervised fine-tuning, and instruction tuning.}
\label{tab:tbl6}
\scriptsize
\renewcommand{\arraystretch}{1.15}
\begin{tabularx}{\textwidth}{@{} p{2.8cm} >{\raggedright\arraybackslash}p{2.5cm} >{\raggedright\arraybackslash}p{1.2cm} X @{}}
\toprule
\textbf{Category} & \textbf{Dataset} & \textbf{Size} & \textbf{Training Focus and Characteristics} \\
\midrule

\multirow{3}{2.8cm}{\textbf{Foundational Pretraining}}
& OpenWebMath \citep{paster2023openwebmath} & 14.7B tokens & Massive curated mathematical corpus from Common Crawl used for domain-adaptive pretraining and learning syntax. \\
& Proof-Pile \citep{azerbayev2023proofnet} & 14.5 GB & Mix of informal and formal mathematical texts (arXiv, ProofWiki) to teach formal logical structures. \\
& AMPS \citep{hendrycks2021measuring} & $>$5 Million (23 GB) & Script-generated problems used to pretrain models on fundamental mathematical rules and intermediate steps. \\

\addlinespace[4pt]
\midrule

\multirow{3}{2.8cm}{\textbf{Grade-School \& Arithmetic (SFT)}}
& Camel-AI Math \citep{li2023camel} & 50,000 & Large-scale multi-step arithmetic and algebra problems used for task-specific fine-tuning. \\
& GSM8K (Training Split) \citep{cobbe2021training} & 7,500 & Used to teach models how to generate explicit, multi-step natural language reasoning chains. \\
& MAWPS (Training Split) \citep{koncel2016mawps} & $\sim$2,373 & Teaches the model to map standardized linguistic word problems into executable mathematical equations. \\

\addlinespace[4pt]
\midrule

\multirow{2}{2.8cm}{\textbf{Advanced \& Competition (SFT)}}
& MATH (Training Split) \citep{hendrycks2021measuring} & 7,500 & Used to fine-tune models on advanced concepts (calculus, geometry, number theory) and complex symbolic manipulations. \\
& OpenMathInstruct-1 \citep{toshniwal2024openmath} & 1.8 Million & Massive open-source instruction-tuning dataset designed to explicitly improve open-ended mathematical logic. \\

\addlinespace[4pt]
\midrule

\textbf{Formalization \& Theorem Proving (SFT)}
& CASIA-PSGPS9K \citep{zhang2024fuse} & 9,022 & Large-scale dataset used specifically to train models in formal theorem proving and geometry-based logical derivations. \\

\bottomrule
\end{tabularx}
\end{table*}

%============================ Table End ================================


Supervised fine-tuning (SFT) datasets focus more directly on teaching models how to produce step-by-step reasoning traces. Grade-school datasets such as the training splits of GSM8K \citep{cobbe2021training} and MAWPS \citep{koncel2016mawps} contain multi-step arithmetic word problems that require models to translate natural language descriptions into structured mathematical operations. Additional datasets such as Camel-AI Math \citep{li2023camel} and OpenMathInstruct-1 \citep{toshniwal2024openmath} expand these capabilities by providing large-scale instruction-style problems that encourage explicit reasoning generation and structured problem solving. At higher levels of abstraction, datasets such as the MATH training split \citep{hendrycks2021measuring} and CASIA-PSGPS9K \citep{zhang2024fuse} introduce more advanced concepts, including calculus, geometry, and formal theorem reasoning.

\subsubsection{Benchmarks (Testing and Assessment)}
Mathematical benchmarks, in contrast to training datasets are designed specifically to evaluate the capacity of the model at different levels of cognitive difficulty, as outlined in Table~\ref{tab:tbl7}. At the foundation level, benchmarks such as the evaluation split from GSM8K \citep{cobbe2021training} and MAWPS \citep{koncel2016mawps}, along with ASDiv \citep{miao2021diverse}, focus on arithmetic and algebraic word problems that test multi-step numerical reasoning and equation mapping abilities. While these tasks provide important baselines for sequential reasoning, they often contain standardized linguistic patterns that may allow models to partially rely on memorization or pattern recognition.


%============================ Table 7 ==================================

\begin{table*}[t]
\centering
\caption{Taxonomy of mathematical reasoning benchmarks organized by evaluation domain and cognitive difficulty.}
\label{tab:tbl7}
\scriptsize
\renewcommand{\arraystretch}{1.15}
\begin{tabularx}{\textwidth}{
>{\raggedright\arraybackslash}p{2.8cm} 
>{\raggedright\arraybackslash}p{2.4cm} 
>{\raggedright\arraybackslash}p{0.9cm} 
>{\raggedright\arraybackslash}X 
}

\toprule

\textbf{Category} & \textbf{Benchmark} & \textbf{Test Size} & \textbf{Evaluation Focus and Characteristics} \\

\midrule

\multirow{4}{*}{\textbf{Grade-School}}

& MAWPS (Test Split) \citep{koncel2016mawps} 
& 355 & Arithmetic word problems emphasizing equation mapping. \\

& ASDiv \citep{miao2021diverse} 
& 1,220 & Diverse arithmetic reasoning tasks with structural variation. \\

& GSM8K (Test Split) \citep{cobbe2021training} 
& 1,319 & Multi-step word problems requiring explicit reasoning chains. \\

& MATH401 \citep{yuan2023well} 
& 401 & Expression-centric arithmetic tasks with advanced formulas. \\

\addlinespace[4pt]
\midrule

\multirow{4}{2.8cm}{\textbf{High-School \& Competition}}

& MATH (Test Split) \citep{hendrycks2021measuring} 
& 5,000 & Competition-level problems across algebra, geometry, and number theory. \\

& OlympiadBench \citep{he2024olympiadbench} 
& 8,476 & Bilingual and multimodal Olympiad benchmark. \\

& OMNI-MATH \citep{gao2024omni} 
& 4,428 & Advanced high-school and Olympiad-style reasoning tasks. \\

& MathOdyssey \citep{fang2025mathodyssey} 
& 387 & Curated advanced problems categorized by mathematical sub-domain. \\

\addlinespace[4pt]
\midrule

\multirow{2}{*}{\textbf{University Level}}

& OCW Course \citep{lewkowycz2022solving} 
& 272 & Real-world university assignments from MIT OpenCourseWare. \\

& U-Math \citep{chernyshev2024u} 
& 1,100 & Open-ended university problems (20\% multimodal). \\

\addlinespace[4pt]
\midrule

\multirow{5}{2.8cm}{\textbf{Formalization \& Theorem Proving}}

& MiniF2F \citep{zheng2021minif2f} 
& 488 & Formal Olympiad problems for neural theorem provers. \\

& Geometry3K \citep{lu2021inter} 
& 3,000 & Diagram-grounded geometry reasoning benchmark. \\

& ProofNet \citep{azerbayev2023proofnet} 
& 371 & Undergraduate formal theorem proving with aligned natural-language proofs. \\

& Def\_Wiki \citep{zhang2025formalizing} 
& 56 & Zero-shot evaluation benchmark testing the autoformalization of Wikipedia definitions into Isabelle/HOL. \\

& Def\_ArXiv \citep{zhang2025formalizing} 
& 30 & Zero-shot evaluation benchmark testing the autoformalization of complex arXiv definitions. \\

\addlinespace[4pt]
\midrule

\multirow{2}{2.8cm}{\textbf{Generalization \& Robustness}}

& LILA \citep{mishra2022lila} 
& 133,815 & Unified benchmark spanning 23 reasoning tasks to test broad generalization. \\

& Math-Perturb \citep{huang2025math} 
& 558 & Robustness evaluation via adversarial perturbations of surface text. \\

\bottomrule
\end{tabularx}
\end{table*}

%============================ Table End ================================


More advanced benchmarks evaluate higher levels of conceptual abstraction. Datasets such as the MATH test split \citep{hendrycks2021measuring}, OlympiadBench \citep{he2024olympiadbench}, OMNI-MATH \citep{gao2024omni}, and MathOdyssey \citep{fang2025mathodyssey} introduce competition-level mathematical problems spanning algebra, geometry, number theory, and combinatorics. These benchmarks require models to integrate multiple mathematical concepts, derive intermediate symbolic expressions, and construct complex reasoning chains.

Beyond standard problem-solving tasks, several benchmarks evaluate specialized reasoning abilities such as formal theorem proving and generalization. Formal reasoning datasets, including MiniF2F \citep{zheng2021minif2f}, Geometry3K \citep{lu2021inter}, and ProofNet \citep{azerbayev2023proofnet}, assess the ability of models to produce logically valid proofs or perform structured symbolic reasoning. Meanwhile, unified and robustness-oriented benchmarks such as LILA \citep{mishra2022lila} and Math-Perturb \citep{huang2025math} test the stability of reasoning capabilities across heterogeneous tasks and adversarially perturbed inputs. These robust evaluations provide crucial insights into whether models rely on genuine algorithmic reasoning rather than superficial pattern matching.


%\subsection{Cognitive Depth and Domain Complexity}\label{sec4.1}
%Mathematical reasoning datasets vary significantly in their cognitive demands, and range from basic arithmetic to advanced theorem proving. Table~\ref{tab:tbl5} categorizes these benchmarks into distinct levels of complexity.
%\subimport{tbs/}{table_5}
%At the Foundational and Grade-School levels, datasets like GSM8K \citep{cobbe2021training} and MAWPS \citep{koncel2016mawps} focus on multi-step arithmetic word problems and equation mapping. While these benchmarks prove essential for teaching LLMs basic logical sequencing, they often rely on standardized problem structures.
%To evaluate deep conceptual synthesis, High-School, Competition, and University benchmarks exist. Datasets such as MATH \citep{hendrycks2021measuring}, OMNI-MATH \citep{gao2024omni}, and U-Math \citep{chernyshev2024u} introduce advanced domains like calculus, linear algebra, and combinatorial logic. These datasets challenge models to apply out-of-the-box logic rather than simply retrieve memorized formulas. Furthermore, to test robustness across diverse tasks, unified benchmarks like LILA \citep{mishra2022lila} and adversarial sets like Math-Perturb \citep{huang2025math} evaluate whether a model possesses true generalized understanding or if it merely exhibits sensitivity to specific phrasing.

\subsection{Semantic and Structural Representations}\label{sec4.2}
As dataset complexity increases, purely natural language representations become insufficient for capturing mathematical structure. Mathematical reasoning inherently relies on symbolic relationships, operator hierarchies, and structured dependencies that differ significantly from conversational language \citep{shalyt2025llms}. Consequently, effective mathematical reasoning systems require mechanisms that map natural language problem statements into structured semantic representations.

Table~\ref{tab:tbl8} summarizes prominent approaches for constructing such representations. Semantic parsing techniques \citep{roy2015solving} convert textual descriptions into executable mathematical expressions, while Unit Dependency Graphs \citep{roy2017unit} explicitly model relationships between quantities and units within word problems \citep{dave2024investigating}. These approaches enable models to identify relevant variables, infer operator relationships, and construct intermediate symbolic forms.

%============================ Table 8 ==================================
\begin{table}[H]
\centering
\caption{Techniques for semantic understanding and structural mapping of mathematical problems.}
\label{tab:tbl8}
\scriptsize
\resizebox{\textwidth}{!}{
\begin{tabularx}{\textwidth}{ 
>{\raggedright\arraybackslash}X  
>{\raggedright\arraybackslash}X 
>{\raggedright\arraybackslash}X 
>{\raggedright\arraybackslash}X 
}
\toprule
\textbf{Technique} & \textbf{Core Mechanism} &  \textbf{Primary Output} &  \textbf{Role} \\

\midrule

Semantic Parsing \citep{roy2015solving} 
& Seq2seq/Transformer mapping & Formal logic forms \& expression trees & Enables downstream symbolic execution \\ 

\midrule

MathBERT/ LLaMA-Math \citep{peng2023mathbert} 
& Domain-adapted LLMs trained on LaTeX/MathML & Structural symbol embeddings & Improves operator prediction and binding \\ 

\midrule

Unit Dependency Graphs \citep{roy2017unit} 
& Directed graphs of quantities & Linked unit and operation dependencies & Supports coreference resolution and quantity relations \\

\midrule

In-Context Learning \citep{brown2020language} 
& Few-shot prompting with demonstration examples & Implicit schema induction & Adapts reasoning patterns without explicit retraining \\ 

\midrule

Distributed Embeddings \citep{devlin2019bert} 
& Contextual vector representations of tokens & Semantic clusters in embedding space & Disambiguates variables and semantic analogies \\

\bottomrule
\end{tabularx}
}
\end{table}
%============================ Table End ================================

Domain-specialized language models further bridge the gap between natural language and mathematical notation. For example, MathBERT \citep{peng2023mathbert} adapts contextual language representations to mathematical corpora, improving operator prediction, symbol disambiguation, and variable binding. Such domain adaptation strategies significantly improve the alignment between linguistic inputs and formal mathematical reasoning processes.


%\subsection{Semantic Understanding and Structural Mapping}\label{sec4.2}
%As the cognitive depth of datasets increases, the reliance on purely natural language diminishes. Mathematical reasoning relies on specific patterns, symbols, and structural logic that differ vastly from standard human conversation \citep{shalyt2025llms}. Consequently, the method a model uses to understand the dataset remains as critical as the dataset itself.

%Table~\ref{tab:tbl8} outlines the core techniques that map natural language statements to formal mathematical representations. Techniques such as Semantic Parsing \citep{roy2015solving} and Unit Dependency Graphs \citep{roy2017unit} prove crucial for identifying variables, operators, and their relations within a problem statement \citep{dave2024investigating}. Furthermore, domain-adapted models like MathBERT \citep{peng2023mathbert} bridge the gap between human language and mathematical syntax, and allow for improved operator prediction and variable binding.

%\subsection{Mathematical Information Retrieval and Representation}\label{sec4.3}
%Once a model maps the semantic structure of a problem, it requires robust retrieval mechanisms to extract and format symbols, equations, and relation trees \citep{stathopoulos2023retrieval}. Because advanced datasets (such as ProofNet \citep{azerbayev2023proofnet} and CASIA-PSGPS9K \citep{zhang2024fuse}) require formal proof generation, standard text generation falls short.

%Table~\ref{tab:tbl9} details the structured representations necessary for this task. The foundation of modern mathematical retrieval relies on MathML \citep{ausbrooks2003mathml}, which splits into Presentation MathML for visual layout and Content MathML for functional semantics \citep{zanibbi2012recognition}. Advanced tree-based retrieval systems, such as Symbol Layout Trees (SLTs) and Operator Trees (OPTs), build upon these foundations. Systems like MCAT \citep{yoko2014mcat, kristianto2016mcat} utilize these trees to allow LLMs to formalize links between variables and perform exact sub-expression retrieval, which bridges the gap between text tokens and mathematical logic.

\subsection{Symbolic Representation and Retrieval}\label{sec4.3}
Once semantic structures are identified, mathematical reasoning systems require mechanisms for retrieving and manipulating formal symbolic representations \citep{stathopoulos2023retrieval}. This step becomes particularly important for advanced datasets involving theorem proving or proof synthesis, where reasoning extends beyond text generation.

Dataset such as CASIA-PSGPS9K \citep{zhang2024fuse} require models to construct formal proofs or derive symbolic expressions that satisfy strict logical constraints. In such settings, conventional text-based generation is insufficient because reasoning must operate over structured mathematical objects.

Modern systems therefore rely on formal representation standards such as MathML \citep{ausbrooks2003mathml}. Presentation MathML encodes visual equation layout, while Content MathML captures the functional semantics of mathematical expressions \citep{zanibbi2012recognition}. These representations allow mathematical expressions to be processed as structured trees rather than flat token sequences.

Advanced symbolic retrieval systems build on this foundation using Symbol Layout Trees (SLTs) and Operator Trees (OPTs). These structures encode spatial and logical relationships between mathematical symbols, enabling systems to perform sub-expression matching, symbolic normalization, and operator-level reasoning. Systems such as MCAT \citep{yoko2014mcat, kristianto2016mcat} utilize these representations to retrieve semantically equivalent expressions and support structured mathematical reasoning.


%============================ Table 9 ==================================


\begin{table}[t]
\centering
\caption{Core techniques and representations used in mathematical information retrieval.}
\label{tab:tbl9}
\scriptsize
\resizebox{\textwidth}{!}{
\begin{tabularx}{\textwidth}{ 
>{\raggedright\arraybackslash}X
>{\raggedright\arraybackslash}X 
>{\raggedright\arraybackslash}X 
>{\raggedright\arraybackslash}X 
}
\toprule
\textbf{Technique} & \textbf{Core Representation} &  \textbf{Key Focus} &  \textbf{Primary Application} \\
\midrule

MathML \citep{ausbrooks2003mathml}
& XML markup & Machine-readable encoding & General mathematical expression encoding \\

Presentation MathML \citep{zanibbi2012recognition}
& Spatial tags & Visual 2D layout & Preserves rendering structure \\

Content MathML \citep{zanibbi2012recognition}
& Operator trees & Functional semantics & Explicit binding of operator arguments \\

Symbol Layout Trees (SLTs) \citep{mansouri2019tangent}
& Spatial tree (nodes=symbols) & Spatial relations & Indexing \& sub-expression retrieval \\

Operator Trees (OPTs) \citep{kristianto2016mcat}
& Semantic tree (root=operator) & Operands \& operations & Normalization \& structural substitution \\

MCAT System \citep{yoko2014mcat,kristianto2016mcat} 
& Hybrid (SLT + OPT) & Text–math integration & Multi-level indexing \& joint queries \\

Tangent-CFT \citep{mansouri2019tangent}
& Dense embeddings (fastText) & Linearized tree paths & Approximate matching via cosine similarity \\

\bottomrule
\end{tabularx}
}
\end{table}


%============================ Table End ================================



%\subsection{Tokenization Mechanisms}\label{sec4.4}
%Even when models successfully parse and retrieve mathematical structures, the fundamental tokenization of numbers and symbols presents a unique bottleneck. Standard natural language tokenizers often fail to capture the strict place-value relationships and morphological structures required for arithmetic and algebraic reasoning. Overall model performance relies heavily on how the system breaks down text and number tokens before feeding them into the transformer.

%Table~\ref{tab:tbl10} outlines the primary techniques developed to handle mathematical tokenization. Standard Byte Pair Encoding (BPE) \citep{zouhar2023formal} iteratively merges frequent adjacent pairs. However, it often splits numbers inconsistently, which disrupts the model's numerical understanding.

%To resolve this, researchers implement directional chunking and digit-level isolation. Left-to-Right (L2R) processing splits numbers from the highest digit, whereas Right-to-Left (R2L) chunking enforces a comma separator every three digits starting from the units place \citep{singh2024tokenization}. R2L aligns much closer to human arithmetic processes and reduces stereotype pattern errors. For tasks requiring extreme precision, Single-Digit tokenization treats every numeral as an individual token \citep{aakanksha2023palm}. While this guarantees perfect place-value alignment, it significantly increases sequence length and computational cost.

%Pushing beyond discrete tokens, Continuous Encoding methods like xVal \citep{golkar2023xval} entirely bypass traditional tokenization. This approach projects numerical values into a continuous vector space, which allows the model to process mathematical magnitude natively alongside text embeddings.

\subsection{Tokenization Mechanisms}\label{sec4.4}

Even when semantic parsing and symbolic retrieval are available, numerical tokenization remains a critical bottleneck in mathematical reasoning. Standard tokenization methods designed for natural language often fail to preserve the positional and compositional properties required for arithmetic operations.

Table~\ref{tab:tbl10} summarizes common tokenization strategies used in mathematical language models. Byte Pair Encoding (BPE) \citep{zouhar2023formal} merges frequent character sequences and is widely used in general-purpose language models. However, BPE frequently splits numbers inconsistently, which disrupts place-value relationships and degrades arithmetic performance.

Alternative tokenization strategies explicitly preserve numerical structure. Left-to-Right (L2R) tokenization processes numbers sequentially from the most significant digit, whereas Right-to-Left (R2L) tokenization inserts separators every three digits starting from the least significant position \citep{singh2024tokenization}. R2L tokenization aligns more closely with human arithmetic procedures and improves carry-operation modeling.

More granular approaches represent each numeral as an individual token \citep{aakanksha2023palm}. Although single-digit tokenization guarantees perfect place-value representation, it increases sequence length and computational cost.

Recent work proposes continuous numerical encodings such as xVal \citep{golkar2023xval}, which bypass discrete tokenization entirely. These methods embed numeric values directly into continuous vector spaces, allowing models to represent numerical magnitude alongside textual context.



%============================ Table 10 ==================================


\begin{table}[t]
\scriptsize
\centering
\caption{Techniques for Tokenization in Mathematical Problems}\label{tbl8}
\renewcommand{\arraystretch}{1.2}
\begin{tabularx}{\textwidth}{ 
>{\raggedright\arraybackslash}p{2.2cm} 
>{\raggedright\arraybackslash}X 
>{\raggedright\arraybackslash}X
}
\toprule
\textbf{Technique} & \textbf{Encoding Mechanism} & \textbf{Structural Impact} \\
\midrule

BPE (Standard) \citep{zouhar2023formal}
& Iterative frequency-based subword merging 
& Utilizes standard byte-level vocabulary; often misaligns place values  \\
\hline

Right-to-Left (R2L) \citep{singh2024tokenization} 
& Chunks from units place leftward (inserts commas every 3 digits) 
& Preserves standard numerical magnitude and formatting \\
\hline

Left-to-Right (L2R) \citep{singh2024tokenization}
& Splits from highest digit rightward (no separators) 
& Direct linear processing; lacks explicit magnitude markers \\
\hline

Single-Digit \citep{aakanksha2023palm}
& Treats each decimal digit (0--9) as an individual token 
& Guarantees perfect place-value alignment; increases overall sequence length \\
\hline

Continuous (xVal) \citep{golkar2023xval}
& Projects numbers into dense continuous vectors (MLP/sinusoidal) 
& Bypasses discrete tokens entirely; maps exact continuous magnitude \\

\bottomrule
\end{tabularx}
\end{table}


%============================ Table End ================================


\subsection{Benchmark Limitations and Research Gaps}\label{sec4.5}
Despite significant progress, several structural limitations continue to constrain the development of robust mathematical reasoning systems.

\textbf{Training–Datsets Contamination.}  
Large-scale corpora such as OpenWebMath \citep{paster2023openwebmath} rely heavily on web-scraped mathematical content. This introduces noise, heuristic extraction errors, and potential leakage between pretraining data and evaluation benchmarks, thereby inflating model performance.

\textbf{Synthetic Reasoning Data Dependence.}  
To compensate for the scarcity of human-annotated reasoning traces, many training pipelines rely heavily on synthetic Chain-of-Thought (CoT) generation. Although synthetic reasoning traces enable large-scale supervision, they often lack the diversity and conceptual richness of human-authored reasoning \citep{guan2025rstar}. Consequently, models trained on synthetic reasoning frequently inherit the limitations of their teacher models and struggle to surpass them \citep{tang2024mathscale, huang2024o1}.

\textbf{Weak Out-of-Distribution Generalization.}  
Current benchmarks predominantly evaluate reasoning within static problem distributions \citep{lindsey2025biology}. Models therefore tend to memorize problem templates rather than internalize underlying mathematical principles. Empirical studies show that LLMs frequently exhibit discontinuous learning behavior and fail to generalize across novel problem structures \citep{ahn2024large}.

\textbf{Numerical Tokenization Limitations.}  
Finally, even with high-quality datasets, numerical tokenization remains a fundamental limitation. Suboptimal tokenization schemes disrupt digit alignment and hinder arithmetic reasoning. Recent studies demonstrate that right-to-left numerical tokenization and explicit digit separation improve numerical reasoning accuracy \citep{singh2024tokenization}, suggesting that dataset formatting and tokenization design must evolve alongside model architectures.

%\subsection{Limitations and Gaps in Current Benchmarks}\label{sec4.5}
%While the integration of complex datasets and advanced retrieval methods pushes the field forward, significant multidimensional gaps remain.

%\textbf{Heuristic Provenance and Data Contamination:} Large-scale foundational corpora, such as OpenWebMath \citep{paster2023openwebmath}, often rely on web-scraping. This introduces noise, heuristic matching errors, and "innate divergence"—where the target reference contains information unsupported by the source text. Furthermore, the risk of test-set leakage into pretraining corpora remains a critical threat to valid evaluation.

%\textbf{Over-reliance on Synthetic Reasoning:} Many current training paradigms rely heavily on synthetic Chain-of-Thought (CoT) data. While useful for scaling, synthetic data often lacks the nuance of human-annotated reasoning \citep{guan2025rstar}. This compromises the quality of reinforcement learning, and leads to diminishing returns where models struggle to surpass their teacher counterparts \citep{tang2024mathscale, huang2024o1}.

%\textbf{Static Evaluation vs. Out-of-Distribution Generalization:} Current datasets often evaluate isolated reasoning steps or static mathematical planning \citep{lindsey2025biology}. However, models frequently exhibit "discontinued learning" \citep{ahn2024large}, and memorize templates rather than conceptualize the underlying mathematical framework. A pressing need exists for datasets that systematically evaluate stepwise training and true out-of-distribution generalization \citep{chernyshev2024u}.

%\textbf{The Tokenization Bottleneck:} Finally, even with perfect datasets, the fundamental tokenization of numbers limits performance. Suboptimal tokenization schemes (e.g., standard left-to-right processing of integers) disrupt morphological tasks in mathematics. Implementing right-to-left (R2L) tokenization and enforcing numeral separation at inference shows promise \citep{singh2024tokenization}, and highlights that dataset formatting must evolve alongside model architecture.
\end{comment}


% % In the domain of text processing, language models are a profound transformation in computational processing. Primarily, a language model estimates the probability distribution over the sequence of words, in order to complete tasks such as text completion, translation, question answering and dialogue generation. Language models can be seen as an advancement in linguistic theory and machine learning techniques  \citep{toprakhistorical}.
    
% % Although a large number of language models are available, whether open-source or closed-source, variable in size, they share some of the common architectural sections. The following section discusses the fact how the architecture for language models has been built over history.
    
% % With the large-scale digital text, demand for intelligent language systems grew, making researchers active in searching for sophisticated approaches. The historical context of the evolution of language models begins with statistical models, usually relying on the frequency and co-occurrence of words within corpora  \citep{charniak1996statistical}. Hidden Markov Models (HMMs)  \citep{knill1997hidden} and n-gram techniques  \citep{pauls2011faster} are referred to as the probabilistic basis models for sequence modelling. Besides being simple and interpretable, these approaches are unable to capture long-term dependencies in sequences, handle sparsity and contextual nuances.
    
% % Moreover, the advent of neural networks in NLP has brought a paradigm shift, from feed-forward to recurrent neural networks (RNNs)  \citep{sundermeyer2013comparison, chen2021recurrent}. This improved architecture has the ability to model sequential dependencies dynamically and adaptively. The exploding and vanishing gradient caused difficulty in working with this architecture of neural networks, leading researchers to build Long Short-Term Memory (LSTM)  \citep{sundermeyer2012lstm} and Gated Recurrent Units (GRUs)  \citep{khan2019rnn} enabling meaningful and deeper temporal representation of language. These architectures are although considerably good but they are prone to exhibit long-term context retention and computation parallelism issues  \citep{jozefowicz2016exploring}.

% % The introduction to transformer architecture with self-attention mechanism allows for scalability, parallelism and variable context awareness  \citep{vaswani2017attention}. Moreover, transformer based models are classified into three different kinds of architectures: 1) Encoder-Only architecture, such as BERT  \citep{koroteev2021bert}, 2) Decoder-Only architecture, such as GPT  \citep{yenduri2024gpt} and 3) Encoder-Decoder architecture, such as T5  \citep{colin2020exploring}. This breakthrough provides basis for the most advanced language models and their successors. This redefines the boundaries of possibilities in language understanding, modeling and generation. Recently, many advancements in transformer architecture have been made in order to achieve a wide range of applications in language modeling. Optimization in architecture involves changes in attention mechanisms such as multi-head latent attention  \citep{meng2025transmla, deng2025multi} and group-query attention  \citep{ainslie2023gqa}, have also been introduced that show a significant level of improvements in language models for multiple tasks. Further optimization techniques are also purposed such as Mixture-of-experts (MOE) architecture with different experts allowing language model to handle diverse tasks  \citep{zoph2022st}. Uses experts and routers or gates to navigate the input towards its most relevant expert. This architecture enables selective training and fine-tuning as well as optimizes the way language models work  \citep{cai2025survey}. Recent advancements in LoRA enables optimized and scalable deployment and training of parameters in LLMs  \citep{liang2025low}. Over the time, low rank adaptation techniques are evolved. However, the trade-offs between full fine-tuning and low-rank adaptation have been a subject of discussion, with  \citep{Dan2024lora} contrasting the two approaches and highlighting the benefits of LoRA in maintaining base model capabilities.

% % % Although these advancements have revolutionized the field of language modeling. However, there are some concerns and issues, discussed in the following section.
% % \input{tbs/table_10}
% % \subsection{Trends and Open Challenges}\label{modelsec1}

% % Pretrained language models (PLMs) are susceptible to generate text with non-factual information. Complex internal computations of LLMs  challenge a full understanding of how features interact within these architectures  \citep{lee2022factuality}. Language model are prone to exhibit long-term context retention and computation parallelism issues  \citep{jozefowicz2016exploring}. On the contrary, they also poses catestropic forgetting which is particularly problematic in language models that are trained across diverse datasets or tasks over time  \citep{ibrahim2024simple}.

% % Models exhibit trends like multi-hop reasoning for mathematical tasks. However, it is noted that LLMs face difficulties in capturing all mechanisms during training due to tool limitations  \citep{lindsey2025biology}. Consequently, it is more likely to return wrong answers when decoding directly, as compared to when using Chain-of-Thought reasoning  \citep{wei2022chain}. Literature shows that language models like ChatGPT  \citep{welsby2023chatgpt} experience difficulties in performing multiplication (provides estimation) especially when multiplying two decimal numbers within 10 and calculation of exponents for decimal numbers. It is also noticed that language models misunderstand exponents treating \textit{**} as multiplication  \citep{yuan2023well}.

% Language models (LMs) represent a paradigm shift in natural language processing (NLP). Fundamentally, an LM estimates the probability distribution over a sequence of tokens, enabling capabilities ranging from basic text completion to complex dialogue generation and reasoning tasks. The evolution of these models reflects a continuous architectural progression aimed at overcoming the limitations of previous generations \citep{toprakhistorical}.

% Historically, sequence modeling relied on statistical probabilistic approaches, such as Hidden Markov Models (HMMs) \citep{knill1997hidden} and n-gram techniques \citep{pauls2011faster}. While computationally lightweight and highly interpretable, these frequency-based models suffered from severe sparsity issues and were fundamentally incapable of capturing long-term contextual dependencies within a corpus \citep{charniak1996statistical}.

% The integration of neural networks into NLP initiated a critical shift from static statistical counting to dynamic, distributed representations. Recurrent Neural Networks (RNNs) \citep{sundermeyer2013comparison, chen2021recurrent} introduced the ability to process variable-length sequences. However, standard RNNs were notoriously difficult to scale due to exploding and vanishing gradients. To address this, Long Short-Term Memory (LSTM) networks \citep{sundermeyer2012lstm} and Gated Recurrent Units (GRUs) \citep{khan2019rnn} were developed, utilizing gating mechanisms to retain deeper temporal representations. Despite these improvements, recurrent architectures faced a hard fundamental bottleneck: their inherently sequential nature prohibited large-scale computational parallelism, restricting training on massive datasets \citep{jozefowicz2016exploring}.

% The introduction of the Transformer architecture \citep{vaswani2017attention} bypassed this sequential bottleneck entirely through the self-attention mechanism, allowing for unprecedented scalability, parallelization, and global context awareness. This breakthrough established three primary architectural lineages: 1) Encoder-only models (e.g., BERT \citep{koroteev2021bert}), optimized for understanding and classification; 2) Decoder-only models (e.g., GPT \citep{yenduri2024gpt}), optimized for autoregressive generation; and 3) Encoder-Decoder models (e.g., T5 \citep{colin2020exploring}), designed for sequence-to-sequence transformations.

% To push the boundaries of these foundational architectures, recent literature has focused heavily on structural and training optimization. Enhancements to attention mechanisms, such as Multi-Head Latent Attention \citep{meng2025transmla, deng2025multi} and Grouped-Query Attention \citep{ainslie2023gqa}, have significantly reduced computational overhead during inference. Concurrently, Mixture-of-Experts (MoE) architectures have allowed models to vastly scale their parameter count—and thus their capacity to handle diverse tasks—without a proportional increase in active compute costs, utilizing routing networks to activate only relevant expert subnetworks per token \citep{zoph2022st, cai2025survey}. Furthermore, the challenge of adapting these massive architectures has been mitigated by Low-Rank Adaptation (LoRA) \citep{liang2025low}. LoRA provides a highly scalable method for task-specific training while avoiding full-parameter updates, successfully preserving the base model's generalized capabilities while optimizing deployment costs \citep{Dan2024lora}.


% \subimport{tbs/}{table_9}


% \subsection{Trends and Open Challenges}\label{modelsec1}

% Despite the revolutionary trajectory of Transformer-based Large Language Models (LLMs), significant architectural and operational vulnerabilities remain. Chief among these is the propensity for hallucination; the complex, opaque internal computations of LLMs make it difficult to trace feature interactions, frequently leading to the generation of highly plausible but entirely non-factual information \citep{lee2022factuality}. Furthermore, while Transformers manage context better than RNNs, they still struggle with extreme long-context retention and are highly susceptible to catastrophic forgetting when continually fine-tuned across diverse datasets over time \citep{ibrahim2024simple}.

% These fundamental limitations become exceptionally pronounced when LLMs are tasked with rigorous mathematical and symbolic reasoning. While models demonstrate the capacity for multi-hop reasoning, they struggle to capture underlying logical mechanisms relying purely on standard autoregressive decoding \citep{lindsey2025biology}. Consequently, direct zero-shot decoding frequently yields erroneous mathematical results, forcing a reliance on prompting interventions like Chain-of-Thought (CoT) to explicitly map reasoning steps \citep{wei2022chain}.

% Crucially, because LLMs are fundamentally trained to predict linguistic tokens rather than execute symbolic logic, they exhibit severe brittleness in algorithmic operations. Literature demonstrates that leading models, such as ChatGPT \citep{welsby2023chatgpt}, frequently resort to estimation rather than precise calculation when multiplying large decimal numbers. They also exhibit profound misunderstandings of fundamental mathematical syntax, such as misinterpreting the exponent operator (\textit{**}) as standard multiplication \citep{yuan2023well}. This dichotomy—where an LLM possesses advanced linguistic fluency but lacks basic arithmetic reliability—highlights the critical necessity for specialized datasets, training paradigms, and architectural adjustments tailored specifically for mathematical reasoning.



%\appendix
%\section{Example Appendix Section}
%\label{app1}

% \begin{table*}[t]
% \centering

% \caption{Detailed venue distribution of cited publications.}
% \label{tab:venue_distribution}
% \small
% \renewcommand{\arraystretch}{1.12}
% \begin{tabular}{@{} l p{9.5cm} r @{}}
% \toprule
% \textbf{Year(s)} & \textbf{Venue} & \textbf{Count} \\
% \midrule

% 1998 & Nature & 1 \\
% 2009 & Towards a Digital Mathematics Library (Grand Bend) & 1 \\
% 2010 & Handbook of Computational Linguistics and Natural Language Processing & 1 \\
% 2012 & International Journal on Document Analysis and Recognition & 1 \\
% 2017, 2022--2023 & Advances in Neural Information Processing Systems & 7 \\
% 2019 & Mathematics Education Research Group of Australasia & 1 \\
% 2019 & Soft Computing & 1 \\
% 2020 & Journal of Machine Learning Research & 1 \\
% 2021 & Australian Journal of Teacher Education & 1 \\
% 2023 & Postgraduate Medical Journal & 1 \\
% 2023 & Information and Software Technology & 1 \\
% 2023 & Intelligent Automation \& Soft Computing & 1 \\
% 2023 & International Journal of Emerging Technologies in Learning (iJET) & 1 \\
% 2024 & Transactions on Machine Learning Research & 1 \\
% 2024 & IEEE Access & 1 \\
% 2024 & Proceedings of the National Academy of Sciences & 1 \\
% 2025 & IEEE Transactions on Knowledge and Data Engineering & 1 \\
% 2025 & Results in Engineering & 1 \\
% 2025 & Scientific Data & 1 \\
% 2025 & Big Data and Cognitive Computing & 1 \\
% 2025 & Authorea pre-prints & 1 \\
% 2025 & Transformer Circuits Thread & 1 \\
% 2020--2026 & ACM Computing Surveys & 7 \\
% 2023--2025 & ACM SIGKDD Conference on Knowledge Discovery and Data Mining & 2 \\
% 2024 & ACM Workshop on Efficiency, Security, and Generalization of Multimedia Foundation Models & 1 \\
% 2025 & ACM Conference on Computer Information and Big Data Applications & 1 \\
% 2025 & ACM Transactions on Intelligent Systems and Technology & 1 \\

% \addlinespace[4pt]
% \midrule
% \multicolumn{3}{@{}l}{\textbf{pre-prints}} \\
% \addlinespace[2pt]
% 2016--2025 & arXiv & 60 \\
% \bottomrule
% \end{tabular}
% \end{table*}

\begin{comment}
\appendix
\section{Comprehensive Reference Coverage and Categorization}

This appendix provides a structured overview of the references used in this survey. 
Given the large number of cited works (approximately 120), we present a categorized 
subset of representative and influential references for each thematic area. Given the breadth of included works spanning foundational theories, datasets, architectures, and evaluation methodologies, we organize the references into thematic categories for clarity and reproducibility.

\subsection{Foundational Works in Language Models}

These works establish the theoretical and architectural foundations of modern large language models, including transformer-based scaling and pretraining paradigms.

\begin{itemize}
    \item \citep{brown2020language} -- Few-shot learning with GPT models
    \item \citep{devlin2019bert} -- Pretraining bidirectional transformers
    \item \citep{aakanksha2023palm} -- Scaling language models with Pathways
    \item \citep{kaplan2020scaling, hernandez2021scaling, rae2021scaling} -- Scaling laws for LLMs
    \item \citep{hoffmann2022training} -- Compute-optimal training strategies
\end{itemize}

\subsection{Mathematical Reasoning Benchmarks and Datasets}

These references introduce datasets and benchmarks used to evaluate mathematical reasoning capabilities of LLMs.

\begin{itemize}
    \item \citep{hendrycks2021measuring} -- MATH dataset
    \item \citep{azerbayev2023proofnet} -- ProofNet formal reasoning dataset
    \item \citep{mishra2022lila} -- Unified reasoning benchmark
    \item \citep{he2024olympiadbench, gao2024omni} -- Olympiad-level benchmarks
    \item \citep{chernyshev2024u} -- University-level evaluation (U-MATH)
    \item \citep{fang2025mathodyssey} -- Large-scale evaluation dataset
    \item \citep{huang2025math} -- Robustness-focused perturbation dataset
\end{itemize}

\subsection{Reasoning Techniques and Prompting Strategies}

This category includes works that propose improvements to reasoning in LLMs through prompting and inference-time strategies.

\begin{itemize}
    \item \citep{wang2023selfconsistency} -- Self-consistency decoding
    \item \citep{imani2023mathprompter} -- Prompt engineering for math reasoning
    \item \citep{han2024rethinking} -- Role-play prompting analysis
    \item \citep{aali2025structured} -- Structured prompting for evaluation
\end{itemize}

\subsection{Training and Optimization Methods}

These works focus on training paradigms, reinforcement learning, and optimization techniques used to enhance LLM reasoning.

\begin{itemize}
    \item \citep{ouyang2022training} -- RLHF training
    \item \citep{achiam2017constrained, schulman2015trust} -- Policy optimization methods
    \item \citep{fu2025reward, miao2024inform, guo2025reward} -- Reward modeling
    \item \citep{mu2024rule} -- Rule-based reward strategies
\end{itemize}

\subsection{Parameter-Efficient Fine-Tuning (PEFT)}

These references explore efficient adaptation techniques for large-scale models.

\begin{itemize}
    \item \citep{hu2021lora} -- LoRA
    \item \citep{Dettmers2023QLORA} -- QLoRA
    \item \citep{valipour2023dylora, liu2024dora, ding2023sora} -- Variants of low-rank adaptation
    \item \citep{liang2025low} -- Survey on PEFT methods
\end{itemize}

\subsection{Symbolic and Tool-Augmented Reasoning}

These works integrate symbolic reasoning or external tools with LLMs.

\begin{itemize}
    \item \citep{lu2021inter} -- Geometry reasoning with symbolic systems
    \item \citep{li2024enhancing} -- Tool-integrated reasoning
    \item \citep{lample2019deep} -- Neural symbolic mathematics
\end{itemize}

\subsection{Evaluation, Faithfulness, and Limitations}

This category includes works addressing hallucination, reasoning reliability, and evaluation challenges.

\begin{itemize}
    \item \citep{ji2023survey} -- Hallucination in LLMs
    \item \citep{wang2025examining} -- False positives in reasoning
    \item \citep{herbert2019challenges, herbert2021overcoming} -- Challenges in assessing reasoning
    \item \citep{carlini2022privacy, shi2023detecting} -- Memorization and data leakage
\end{itemize}

\subsection{Data Quality and Representation Challenges}

These works highlight issues in data quality, tokenization, and numerical representation.

\begin{itemize}
    \item \citep{gong2023survey, karra2023impact} -- Dataset quality
    \item \citep{bostrom2020byte, singh2024tokenization, rajaraman2024toward} -- Tokenization limitations
    \item \citep{golkar2023xval} -- Numerical encoding methods
\end{itemize}

\subsection{Historical and Theoretical Foundations of Mathematical Reasoning}

These references provide broader context for mathematical reasoning and cognition.

\begin{itemize}
    \item \citep{feigenbaum1963computers} -- Early AI reasoning
    \item \citep{kline1990mathematical} -- History of mathematics
    \item \citep{devlin1998language} -- Language of mathematics
\end{itemize}

\subsection{Additional Surveys and Meta-Analyses}

These works complement the present survey and provide broader perspectives.

\begin{itemize}
    \item \citep{forootani2025survey} -- Mathematical reasoning survey
    \item \citep{huang2023towards} -- Reasoning in LLMs
    \item \citep{liu2023mathematical} -- Mathematical language models survey
\end{itemize}

\section{Reproducibility Statement}

All references included in this survey were collected through a structured and iterative process combining keyword-based search, citation chaining, and manual filtering. Efforts were made to ensure diversity across datasets, methods, and evaluation strategies.

Despite these efforts, the rapidly evolving nature of LLM research implies that some recent works may not be included.

\section{Limitations of Reference Coverage}

\begin{itemize}
    \item Rapid publication cycles in arXiv may lead to missing recent contributions
    \item Some references may overlap across multiple categories
    \item Categorization involves subjective judgment
\end{itemize}

Future updates to this survey may incorporate automated literature mining techniques for improved coverage.
\end{comment}


==> tbs/filtered_results.tex <==
\begin{table}[t]
\centering

\caption{Retrieval statistics across Boolean keyword query combinations.}
\label{tab:search_queries}
\small
\renewcommand{\arraystretch}{1.1}
\begin{tabular}{lrrr}
\toprule
\textbf{Query Set} & \textbf{Initial Hits} & \textbf{Screened (Unique)} & \textbf{Remaining} \\
\midrule
1  & 166,868 & 43,354 & 18,604 \\
2  & 572     & 148    & 63     \\
3  & 909     & 239    & 103    \\
4  & 3,812   & 993    & 426    \\
5  & 18,458  & 4,797  & 2,058  \\
6  & 18,210  & 4,726  & 2,028  \\
7  & 15,437  & 4,008  & 1,720  \\
8  & 16,001  & 4,156  & 1,783  \\
9  & 13,857  & 3,607  & 1,544  \\
10 & 16,976  & 4,409  & 1,892  \\
\midrule
\textbf{Total} & \textbf{271,100} & \textbf{70,437} & \textbf{30,225} \\
\bottomrule
\end{tabular}
\end{table}


==> tbs/journals_stats.tex <==
\begin{table}[t]
\centering

\caption{Distribution of cited publications by year.}
\label{tab:year_distribution}
\small
\renewcommand{\arraystretch}{1.15}
\begin{tabular}{@{} lr @{}}
\toprule
\textbf{Year} & \textbf{Count} \\
\midrule
1998 & 1 \\
2009 & 1 \\
2010 & 1 \\
2012 & 1 \\
2016 & 1 \\
2017 & 1 \\
2019 & 3 \\
2020 & 4 \\
2021 & 11 \\
2022 & 12 \\
2023 & 18 \\
2024 & 18 \\
2025 & 16 \\
\midrule
\textbf{Total} & \textbf{88} \\
\bottomrule
\end{tabular}
\end{table}


==> tbs/ref_stats.tex <==
\begin{table}[t]
\centering

\caption{Distribution of cited references by publication year and document type.}
\label{tab:refs_year_type_totals}
\small
\renewcommand{\arraystretch}{1.15}
\begin{tabular}{@{} lrrrrrrr @{}}
\toprule
\textbf{Year} & 
\textbf{Art.} & 
\textbf{Book} & 
\textbf{Incoll.} & 
\textbf{Inproc.} & 
\textbf{Misc.} & 
\textbf{PhD} & 
\textbf{Total} \\
\midrule

1963--1998 & 3  & 1 & 1 & 0  & 0 & 0 & 5  \\
2003--2019 & 8  & 1 & 0 & 16 & 1 & 0 & 26 \\
2020       & 14 & 0 & 0 & 10 & 0 & 0 & 24 \\
2021       & 11 & 0 & 0 & 1  & 0 & 0 & 12 \\
2022       & 24 & 0 & 0 & 2  & 0 & 0 & 26 \\
2023       & 31 & 0 & 0 & 10 & 0 & 1 & 42 \\
2024       & 30 & 0 & 0 & 18 & 0 & 0 & 48 \\
2025       & 17 & 1 & 0 & 11 & 0 & 0 & 29 \\
2026       & 1  & 0 & 0 & 0  & 0 & 0 & 1  \\

\midrule
\textbf{Total} & 
\textbf{139} & 
\textbf{3} & 
\textbf{1} & 
\textbf{68} & 
\textbf{1} & 
\textbf{1} & 
\textbf{213} \\
\bottomrule
\end{tabular}
\end{table}


==> tbs/table_10.tex <==
\begin{table*}[t]
\centering
\caption{Taxonomy of mathematical reasoning datasets utilized strictly for pretraining, supervised fine-tuning, and instruction tuning.}
\label{tab:tbl10}
\scriptsize
\renewcommand{\arraystretch}{1.15}
\begin{tabularx}{\textwidth}{@{} p{2.8cm} >{\raggedright\arraybackslash}p{2.5cm} >{\raggedright\arraybackslash}p{1.2cm} X @{}}
\toprule
\textbf{Category} & \textbf{Dataset} & \textbf{Size} & \textbf{Training Focus and Characteristics} \\
\midrule

\multirow{3}{2.8cm}{\textbf{Foundational Pretraining}}
& OpenWebMath \citep{paster2023openwebmath} & 14.7B tokens & Massive curated mathematical corpus from Common Crawl used for domain-adaptive pretraining and learning syntax. \\
& Proof-Pile \citep{azerbayev2023proofnet} & 14.5 GB & Mix of informal and formal mathematical texts (arXiv, ProofWiki) to teach formal logical structures. \\
& AMPS \citep{hendrycks2021measuring} & $>$5 Million (23 GB) & Script-generated problems used to pretrain models on fundamental mathematical rules and intermediate steps. \\

\addlinespace[4pt]
\midrule

\multirow{3}{2.8cm}{\textbf{Grade-School \& Arithmetic (SFT)}}
& Camel-AI Math \citep{li2023camel} & 50,000 & Large-scale multi-step arithmetic and algebra problems used for task-specific fine-tuning. \\
& GSM8K (Training Split) \citep{cobbe2021training} & 7,500 & Used to teach models how to generate explicit, multi-step natural language reasoning chains. \\
& MAWPS (Training Split) \citep{koncel2016mawps} & $\sim$2,373 & Teaches the model to map standardized linguistic word problems into executable mathematical equations. \\

\addlinespace[4pt]
\midrule

\multirow{2}{2.8cm}{\textbf{Advanced \& Competition (SFT)}}
& MATH (Training Split) \citep{hendrycks2021measuring} & 7,500 & Used to fine-tune models on advanced concepts (calculus, geometry, number theory) and complex symbolic manipulations. \\
& OpenMathInstruct-1 \citep{toshniwal2024openmath} & 1.8 Million & Massive open-source instruction-tuning dataset designed to explicitly improve open-ended mathematical logic. \\

\addlinespace[4pt]
\midrule

\textbf{Formalization \& Theorem Proving (SFT)}
& CASIA-PSGPS9K \citep{zhang2024fuse} & 9,022 & Large-scale dataset used specifically to train models in formal theorem proving and geometry-based logical derivations. \\

\bottomrule
\end{tabularx}
\end{table*}

==> tbs/table_6.tex <==
% \begin{table*}[t]
% \centering

% \caption{Techniques for semantic understanding and structural mapping of mathematical problems.}
% \label{tbl6}
% \scriptsize
% \renewcommand{\arraystretch}{1.15}
% \begin{tabular}{@{} p{3.0cm} p{10.4cm} @{}}
% \toprule
% \textbf{Technique} & \textbf{Core Mechanism and Role in Problem Understanding} \\
% \midrule

% Semantic Parsing 
% & Maps natural language statements to formal representations (logic forms, expression trees) using seq2seq or transformer models. Extracts variables, operators, and relations for downstream symbolic execution \citep{roy2015solving}. \\

% MathBERT / LLaMA-Math 
% & Domain-adapted language models pretrained on LaTeX or MathML corpora. Learn structural symbol embeddings and mathematical syntax, improving operator prediction and variable binding inference \citep{peng2023mathbert}. \\

% Unit Dependency Graphs 
% & Construct directed graphs linking numerical quantities via unit and operation dependencies. Supports coreference resolution and equation construction through graph traversal and symbolic execution \citep{roy2017unit}. \\

% In-Context Learning 
% & Few-shot prompting paradigm where structured examples guide implicit schema induction without explicit retraining \citep{brown2020language}. \\

% Distributed Embeddings 
% & Encode symbols and mathematical concepts into continuous vector spaces (e.g., GloVe, BERT), enabling semantic clustering, analogy reasoning, and disambiguation of variables \citep{devlin2019bert}. \\

% \bottomrule
% \end{tabular}
% \end{table*}


\begin{table*}[t]
\centering

\caption{Techniques for semantic understanding and structural mapping of mathematical problems.}
\label{tbl6}
\scriptsize
\renewcommand{\arraystretch}{1.15}
\begin{tabular}{@{} >{\raggedright\arraybackslash}p{2.5cm} >{\raggedright\arraybackslash}p{2.5cm} p{2.5cm} >{\raggedright\arraybackslash}p{2.5cm} >{\raggedright\arraybackslash}p{2.0cm} @{}}
\toprule
\textbf{Technique} & \textbf{Core Mechanism} &  \textbf{Primary Output} &  \textbf{Role} &  \textbf{Reference}\\
\midrule

Semantic Parsing 
& Seq2seq / Transformer mapping & Formal logic forms \& expression trees & Enables downstream symbolic execution & \citep{roy2015solving} \\

MathBERT / LLaMA-Math 
& Domain-adapted LLMs (LaTeX / MathML) & Structural symbol embeddings & Improves operator prediction \& binding &  \citep{peng2023mathbert}. \\

Unit Dependency Graphs 
& Directed graphs of quantities & Linked unit/operation dependencies & Supports coreference resolution & \citep{roy2017unit}. \\

In-Context Learning 
& Few-shot prompting & Implicit schema induction & Adapts without explicit retraining & \citep{brown2020language}. \\

Distributed Embeddings 
& Continuous vector space encoding & Semantic clusters & Disambiguates variables \& analogies & \citep{devlin2019bert}. \\

\bottomrule
\end{tabular}
\end{table*}


==> tbs/table_7.tex <==
% \begin{table*}[t]
% \centering

% \caption{Core techniques and representations used in mathematical information retrieval.}
% \label{tbl7}
% \scriptsize
% \renewcommand{\arraystretch}{1.15}

% \begin{tabular}{@{} p{3.0cm} p{10.2cm} @{}}
% \toprule
% \textbf{Technique} & \textbf{Function and Representation} \\
% \midrule

% MathML 
% & XML-based markup language for encoding mathematical expressions in machine-readable form \citep{ausbrooks2003mathml}. \\

% Presentation MathML 
% & Encodes the visual two-dimensional layout of formulas using explicit spatial tags (e.g., above, below, adjacent) to preserve rendering structure \citep{zanibbi2012recognition}. \\

% Content MathML 
% & Represents the functional semantics of expressions as operator trees, where each operator node explicitly binds ordered argument nodes \citep{zanibbi2012recognition}. \\

% Symbol Layout Trees (SLTs) 
% & Tree representation derived from Presentation MathML; nodes correspond to symbols and edges encode spatial relations. Linearized (e.g., depth-first) for indexing and sub-expression retrieval \citep{mansouri2019tangent}. \\

% Operator Trees (OPTs) 
% & Tree representation derived from Content MathML; root denotes the primary operator and children denote operands, enabling normalization and structural substitution \citep{kristianto2016mcat}. \\

% MCAT System 
% & Hybrid retrieval framework combining SLTs and OPTs; supports document-, paragraph-, and sub-expression-level indexing with joint text–math queries \citep{yoko2014mcat,kristianto2016mcat}. \\

% Tangent-CFT 
% & Dense retrieval approach embedding SLTs and OPTs via fastText over linearized paths; employs cosine similarity for approximate matching \citep{mansouri2019tangent}. \\

% \bottomrule
% \end{tabular}
% \end{table*}


\begin{table*}[t]
\centering

\caption{Core techniques and representations used in mathematical information retrieval.}
\label{tbl7}
\scriptsize
\renewcommand{\arraystretch}{1.15}
\begin{tabular}{@{} >{\raggedright\arraybackslash}p{2.5cm} >{\raggedright\arraybackslash}p{2.5cm} >{\raggedright\arraybackslash}p{2.2cm} >{\raggedright\arraybackslash}p{2.8cm} >{\raggedright\arraybackslash}p{2.0cm} @{}}
\toprule
\textbf{Technique} & \textbf{Core Representation} &  \textbf{Key Focus} &  \textbf{Primary Application} &  \textbf{Reference}\\
\midrule

MathML 
& XML markup & Machine-readable encoding & General mathematical expression encoding & \citep{ausbrooks2003mathml} \\

Presentation MathML 
& Spatial tags & Visual 2D layout & Preserves rendering structure &  \citep{zanibbi2012recognition} \\

Content MathML 
& Operator trees & Functional semantics & Explicit binding of operator arguments & \citep{zanibbi2012recognition} \\

Symbol Layout Trees (SLTs)
& Spatial tree (nodes=symbols) & Spatial relations & Indexing \& sub-expression retrieval & \citep{mansouri2019tangent} \\

Operator Trees (OPTs) 
& Semantic tree (root=operator) & Operands \& operations & Normalization \& structural substitution & \citep{kristianto2016mcat} \\

MCAT System 
& Hybrid (SLT + OPT) & Text–math integration & Multi-level indexing \& joint queries & \citep{yoko2014mcat,kristianto2016mcat} \\

Tangent-CFT
& Dense embeddings (fastText) & Linearized tree paths & Approximate matching via cosine similarity & \citep{mansouri2019tangent} \\

\bottomrule
\end{tabular}
\end{table*}


==> tbs/table_8.tex <==
% \begin{table}[t]
% \scriptsize
% \centering
% \caption{Techniques for Tokenization in Mathematical Problems}\label{tbl8}

% \begin{tabularx}{1\textwidth}{@{} p{4cm} p{9.3cm}}
% \toprule
% \textbf{Technique} & \textbf{Function}\\
% \midrule
% \textbf{BPE (Standard)} & Iteratively merges the most frequent adjacent pair into a new subword token then placed into byte-level vocabulary  \citep{zouhar2023formal}. \\
% \hline
% \textbf{Right-to-Left (R2L)} & Forces numbers to be chunked from the units place leftward, inserting a comma token every three digits during preprocessing  \citep{singh2024tokenization}. \\
% \hline
% \textbf{Left-to-Right (L2R)} & Splits numbers from the highest digit rightward without enforced separators  \citep{singh2024tokenization}. \\
% \hline
% \textbf{Single-Digit} & Treats every decimal digit as an individual token in the vocabulary (0-9); a number is tokenized digit-by-digit plus optional sign/decimals, guaranteeing perfect place-value alignment at the cost of longer sequences  \citep{aakanksha2023palm}. \\
% \hline
% \textbf{Continuous Encoding (xVal)} & Bypasses discrete tokens entirely; each number is projected into a fixed-dimensional dense vector via a learned MLP or sinusoidal positional encoding, then concatenated with text embeddings and fed directly to the transformer  \citep{golkar2023xval}. \\
% \hline
% \end{tabularx}
% \end{table}

% \begin{table}[htbp]
% \scriptsize
% \centering
% \caption{Techniques for Tokenization in Mathematical Problems}\label{tbl8}
% \renewcommand{\arraystretch}{1.2}
% \begin{tabularx}{1\textwidth}{@{} p{3.5cm} X @{}}
% \toprule
% \textbf{Technique} & \textbf{Function}\\
% \midrule

% \textbf{BPE (Standard)} 
% & Iteratively merges the most frequent adjacent pairs into new subword tokens and places them into a byte-level vocabulary \citep{zouhar2023formal}. \\

% \textbf{Right-to-Left (R2L)} 
% & Chunks numbers from the units place leftward, and inserts a comma token every three digits during preprocessing \citep{singh2024tokenization}. \\

% \textbf{Left-to-Right (L2R)} 
% & Splits numbers from the highest digit rightward without enforced separators \citep{singh2024tokenization}. \\

% \textbf{Single-Digit} 
% & Treats every decimal digit (0-9) as an individual token; tokenizes numbers digit-by-digit alongside optional signs or decimals, which guarantees perfect place-value alignment at the cost of longer sequences \citep{aakanksha2023palm}. \\

% \textbf{Continuous Encoding (xVal)} 
% & Bypasses discrete tokens entirely; projects each number into a fixed-dimensional dense vector via a learned MLP or sinusoidal positional encoding, concatenates it with text embeddings, and feeds it directly to the transformer \citep{golkar2023xval}. \\

% \bottomrule
% \end{tabularx}
% \end{table}

\begin{table}[t]
\scriptsize
\centering
\caption{Techniques for Tokenization in Mathematical Problems}\label{tbl8}
\renewcommand{\arraystretch}{1.2}
\begin{tabularx}{\textwidth}{@{} >{\raggedright\arraybackslash}p{2.2cm} >{\raggedright\arraybackslash}p{4.0cm} >{\raggedright\arraybackslash}p{4.0cm} >{\raggedright\arraybackslash}p{2.0cm} @{}}
\toprule
\textbf{Technique} & \textbf{Encoding Mechanism} & \textbf{Structural Impact} & \textbf{Reference} \\
\midrule

BPE (Standard)
& Iterative frequency-based subword merging 
& Utilizes standard byte-level vocabulary; often misaligns place values & \citep{zouhar2023formal} \\
\hline

Right-to-Left (R2L)
& Chunks from units place leftward (inserts commas every 3 digits) 
& Preserves standard numerical magnitude and formatting & \citep{singh2024tokenization} \\
\hline

Left-to-Right (L2R)
& Splits from highest digit rightward (no separators) 
& Direct linear processing; lacks explicit magnitude markers & \citep{singh2024tokenization} \\
\hline

Single-Digit
& Treats each decimal digit (0--9) as an individual token 
& Guarantees perfect place-value alignment; increases overall sequence length  & \citep{aakanksha2023palm} \\
\hline

Continuous (xVal)
& Projects numbers into dense continuous vectors (MLP/sinusoidal) 
& Bypasses discrete tokens entirely; maps exact continuous magnitude & \citep{golkar2023xval} \\

\bottomrule
\end{tabularx}
\end{table}

==> tbs/table_9.tex <==
\begin{table*}[t]
\centering
\caption{Concise overview of LoRA and its variants}
\label{tab:tbl9}
\small
\resizebox{\textwidth}{!}{
\begin{tabular}{>{\raggedright\arraybackslash}l|>{\raggedright\arraybackslash}p{4.5cm}|>{\raggedright\arraybackslash}p{4cm}|>{\raggedright\arraybackslash}p{4cm}|c}

\toprule
\textbf{Name} & \textbf{Function} & \textbf{Performance} & \textbf{Memory Intensity} \\
\midrule
LoRA   \citep{hu2022lora} & Freezes pre-trained weights; injects low-rank decomposition matrices into Transformer layers. & Matches/exceeds full fine-tuning with fewer parameters. & Reduces trainable params by 10,000x; GPU memory by 3x. \\ \hline  
QLoRA   \citep{Dettmers2023QLORA} & Backpropagates through frozen 4-bit quantized model into LoRA adapters. & Matches 16-bit full FT; fine-tunes 65B on single GPU. & Fine-tunes 65B on 48GB GPU. \\ \hline  
LoRA-FA/FB   \citep{zhang2023lora} & Freezes one low-rank matrix to reduce activation memory. & Matches LoRA performance. & Up to 1.4x less overall memory than LoRA. \\ \hline  
Tied-LoRA   \citep{renduchintala2024tiedlora} & Weight tying and selective training for parameter efficiency. & Comparable to LoRA with fewer parameters. & Reduces trainable parameters. \\ \hline  
AdaLoRA   \citep{zhang2023adalora} & Adaptively allocates budget via SVD-based importance scores. & Better than LoRA in low-budget settings. & Similar to LoRA. \\ \hline  
ALoRA   \citep{liu2024alora} & Dynamically allocates ranks based on importance. & Better than LoRA on various tasks. & Similar to LoRA. \\ \hline  
DoRA   \citep{liu2024dora} & Decomposes weights into magnitude/direction; LoRA on direction. & Outperforms LoRA on reasoning/visual tasks. & Similar to LoRA. \\ \hline  
VB-LoRA   \citep{li2024vblora} & Composites low-rank matrices from shared vector bank with top-k. & Maintain comparable/better performance compared to SOTA
PEFT methods & Uses only 0.4\% of LoRA’s stored parameters. \\ \hline  
PRILoRA   \citep{benedek2024prilora} & Pruned and rank-increasing with linear distribution and pruning. & Better than LoRA on GLUE. & Similar to LoRA. \\ \hline  
MoRA   \citep{liu2024mora} & High-rank updating via square matrix. & Better than LoRA on memory-intensive tasks. & Similar to LoRA. \\ \hline  
Trans-LoRA   \citep{wang2024trans} & \textit{Data-free} transferable PEFT via knowledge distillation and adapter alignment across models. & Strong zero-shot domain adaptation. & Comparable to LoRA. \\ \hline  
Delta-LoRA   \citep{zi2023deltalora} & Updates pretrained weights with delta of low-rank products. & Outperforms low-rank methods. & Comparable to LoRA. \\ \hline  
MELoRA   \citep{ren2024melora} & Mini-ensemble of low-rank adapters for higher effective rank. & Better than LoRA  & Similar to LoRA \\ \hline  
SoRA   \citep{ding2023sora} & Sparse low-rank with gate for dynamic rank adjustment. & Outperforms baselines with 70\% fewer params/time. & Reduces parameters by 70\%. \\ \hline  
Dynamic LoRA   \citep{valipour2023dylora} & Dynamic low-rank without fixed rank (DyLoRA). & Better than LoRA. & Similar to LoRA. \\ \hline  
CoRA   \citep{xiao2024cora} & Optimizes LoRA with common subspace from large models. & Better than LoRA. & Reduces parameters. \\
\hline
 
RoRA   \citep{liu2024rora} & Reliability optimization for rank adaptation. & Outperforms LoRA/DoRA. & Efficient. \\ \hline  
Flexora   \citep{wei2025flexora} & Automatically selects critical layers for LoRA fine-tuning via HPO and unrolled differentiation to mitigate overfitting. & Consistently outperforms baselines on diverse tasks. & Similar to LoRA. \\
\bottomrule
\end{tabular}
}
\end{table*}
